Understanding Interactions Between Chip Architecture and Uncertainties in Semiconductor Supply and Demand

Mitigating losses from supply and demand volatility in the semiconductor supply chain and market has traditionally been cast as a logistics and forecasting problem. We investigate how the architecture of a family of chips influences how it is affected by supply and demand uncertainties. We observe that semiconductor supply chains become fragile, in part, due to single demand paths, where one chip can satisfy only one demand. Chip architects can enable multiple paths to satisfy a chip demand, which improves supply chain resilience. Based on this observation, we study composition and adaptation as architectural strategies to improve resilience to volatility and also introduce a third strategy of dispersion. These strategies allow multiple paths to satisfy a given chip demand. We develop a model to analyze the impact of these architectural techniques on supply chain costs under different regimes of uncertainties and evaluate what happens when they are combined. We present several interesting and even counterintuitive observations about the product configurations and market conditions where these interventions are impactful and where they are not. In all, we show that product redesign supported by architectural changes can mitigate nearly half of the losses caused by supply and demand volatility. As far as we know, this is the first such investigation concerning chip architecture.

==> Interventions.tex <==
\subsection{Composition}
Composition is the process in which final demand goods are produced 
by combining a set of input goods. 
In this way, the supply and the demand chains are not tightly coupled/linked, 
rather "de-linked" to some extent with the goal to improve the overall 
resilience of the supply chain.
Mathematically, composition can be treated as many-to-one mapping 
problem as shown in Figure~\ref{fig:composition}-a. 

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{./images/composition.png}
    \caption{Caption}
    \label{fig:composition}
\end{figure}
A hypothetical example for composition is shown in figure~\ref{fig:composition}-a. 
Where demand goods are labeled as D1, D2 and D3; and supplied goods are
labeled as S1, S2, S3 and S4. 
The arrows connecting the supplied goods to demand goods show the mapping 
required to build the demand goods by the specific combination of supplied goods.
As shown in figure~\ref{fig:composition}-a the demanded product D1 can be made 
by combining the supplied goods S1, S2 and S3. 
And product D3 can be made by combining a different subset of supplied goods 
(S2, S3 and S4 in this hypothetical example). 
Different supplied goods can also be used to different demand products e.g. in this 
example S4 is used to build D2 and D3. 
Mathematically this can be treated as many-to-one mapping problem with 
selective optimization targets that may improve the resilience of the 
supply chain.

In the context of semiconductor hardware, the composition can be defined, 
as the process in which instead of building bigger monolithic integrated circuits (chips),
we build a set of smaller integrated circuits (chiplets) and combine them
together, using interconnects, to build the final product. 
Composing a system from a set of smaller chiplets instead of a single monolithic 
chip can help in improving the overall yield of the semiconductor manufacturing 
due to multiple reasons 

As discussed in section~\ref{sec:uncertainity}, 
uncertainties in the overall yield is a critical component that 
introduces uncertainty in semiconductor supply chain. 
The semiconductor products have short life cycles~\ref{sec:lifecycles}, 
newer products and processes are continuously introduced to meet the 
competition of the market.
As yield is at its worst for newer products/processes, 
due to developing science of the newer processes and short debugging/learning time.
The composition can help in decoupling the process and final demand products.  

Moreover, building larger area monolithic systems would require cutting edge process nodes
as it might not be possible to use older technology 
nodes to build large area monolithic systems due to the reticle limit~\cite{}.
As discussed earlier, the cutting edge process nodes are usually in the 
early stages of development and are not resilient.
Building the large systems as a combination of 
smaller chiplets will allow us to use mixed/older technology nodes, which have established 
science and are more resilient.
This will not only improve the overall yield but also increase
the overall flexibility and adaptability 
of the semiconductor supply chain 
as there are more choices for the technology node to pick from. 

The cost/mm2 of the semiconductor dies is increasing as newer 
technology nodes are being introduced. 
The cost of $250mm^2$ die on 7nm process is $\approx 4\times$
the cost on 45nm process and it's expected to continue to increases with 
newer/smaller technology nodes.
Hence building larger monolithic chiplets is increasingly becoming 
less economical. 
Breaking down monolithic systems to smaller chiplets considerably increases 
the yield with minimum area penalty 
($>2\times$ increase in yield when a $360mm^2$ die is 
broken down to 4-chiplet design with only $\approx 10\%$ area penalty ~\cite{}).
~\cite{}~\cite{} claim that 
if critical processor components are partitioned into separate chiplets
and integrated on highperformance interconnects
it will not cause significant performance
degradation (<5\%) compared to large area monolithic SoCs.

As the cost negatively impacts the resilience of the supply chain, 
the chiplet based designs will improve the 
resilience of semiconductor supply chain with minimum performance degradation. 

In summary, the composition strategy 
can make the semiconductor supply chain 
more flexible, more adaptable and more economical, 
as discussed in section ~\ref{sec:} these are some of the key characteristics 
to improve the resilience of the supply chain.
And smart decisions made by 
architects for building heterogeneous end products 
by smart combination of chiplets can 
directly impact the resilience of the semiconductor 
supply chain. 


\subsection{Adaptation}

The adaptation is the process in which the supplied goods 
can be adapted to meet the requirements of several demanded goods.
Like composition, adaptation also decouples the supplied goods from 
demanded goods with the potential to improve the overall 
resilience of the supply chain.
Mathematically, adaptation can be treated as one-to-many mapping 
problem from supply to demand, as shown in Figure~\ref{fig:composition}-b. 

A hypothetical example for adaptation is shown in figure~\ref{fig:composition}-b. 
Where demand goods are labeled as D1 and D2; and the supplied goods are
labeled as S1 and S2.
The arrows connecting the 
supplied goods to the demanded goods show the adaptation capability of the 
supplied goods. 
As shown in figure~\ref{fig:composition}-b 
the supplied good S1 can be adapted to 
meet the demands of D1, D2 and D3 and 
the supplied good S2 can be adapted to 
meet the demands of D4 and D5.
Mathematically this can be treated as one-to-many mapping problem that can be 
optimized with the goal to improve the overall resilience of the 
supply chain. 

In the context of semiconductor hardware, the adaptation can be defined, 
as the process in which
the supplied hardware can be adapted to target the specifications 
of more than one demand products. 
One way to achieve adaptation is to use the programmable or 
reconfigurable hardware, 
instead of fixed function hardware. 
If the we consider our demand as applications, we can either design 
application specific integrated circuits (ASICS)
to target those applications or use programmable 
such as FPGA (Field Programmable Gate Arrays) and 
programmable network devices (Switches, smart NICs) hardware.
Designing programmable hardware that can adapt to 
different demand requirements can improve the flexibility of the 
semiconductor supply chain and makes the supply chain less prune to disruptions, which 
will make the semiconductor supply chain more resilient to disruptions. 
Moreover, the programmable hardware can be mass produces as commodity 
product, which reduces the cost of hardware and in tern make the 
supoply chain more resilient. 

Adaptation in the semiconductor supply chain can also be achieved by binning
the hardware. 
Binning is the the process of categorizing the hardware components
by their quality and performance. 
The semiconductor components, such as microprocessors, GPUs, CPUs, RAMs etc,
are designed for certain performance specifications but sometimes they fall short 
to meet those specifications due to the complexities of the 
semiconductor manufacturing process.
One example of binning can be, if a four core Intel i5 processor fails to meet the 
required power specifications, they might disable two of it's cores and 
bin it as two core i3 processor ~\cite{binexample}. 
Adaptation of the hardware that doesn't meet the strict specification 
of higher end products by binning to lower end products 
can reduce the effective overall cost 
and improve the effective overall yield. 
The lower cost and higher yield translate to improvement in the 
resilience of the semiconductor supply chain. 
Architects can also use voltage/frequency scaling (VFS) to design adaptable hardware. 
Demand hardware may have varying performance and energy efficiency requirements based on the workloads that 
its supposed to target.  
Architects can use voltage/frequency scaling (VFS)
techniques to adapt the supplied hardware according to the performance 
and energy efficiency requirements of the demand hardware~\cite{onlineVFS}.
This will introduce flexibility in the supply chain and intern make it more resilient. 

Rebadging/rebranding and refreshing
techniques 
can also be used to make the hardware more adaptable. 
In semiconductor hardware context rebadging/rebranding 
is the process of taking the older products, preferably from previous
generations, and selling them by changing their names. 
In rebadging/rebranding
process, certain hardware features can be enabled or disabled or clock 
speed changes may be applied but the core architecture and the 
chip remain the same. 
E.g. Apple's A12Z Bionic Chip (2020-iPad-Pro) is a rebadged 
A12X Bionic with an enabled GPU core. 
Whereas, a "refresh" is 
the techniques in which minor enhancements are 
applied to improve the performance and/or efficiency of the chip.
E.g. the AMD Radeon-RX-500 series is a refresh of the older 
AMD Radeon-RX-400 series where both series use Polaris GPU 
architecture~\ref{refreshlist}.
Rebadging/rebranding and refresh may make the hardware adapt to 
different demand requirements. 

If architects design the hardware to be adaptable then, 
in the case of a disruptive event if the manufacturing of certain low-end hardware product is 
affected, then certain features of high-end hardware can be disabled to make it meet the 
specifications of the disruptive low-end product. Industry commonly uses rebadging to sell hardware 
under different product specifications, many examples of rebadging are presented in Table~\ref{tab:rebadging}.
%\input{./texFiles/rebadgingTable}
Rebadging usually cuts the 
overall cost of the semiconductor product and increase its life-cycle, 
as new chip design and architecture cost money, resources and time.
Lower cost and improved life-cycle of the product aid in 
improving the resilience of the semiconductor supply chain.
which improves the resilience of the semiconductor supply chain.
Rebadging increases the flexibility of the semiconductor supply chain, which improves 
the resilience of the supply chain.


\subsection{Commoditization}

The commoditization is the process in which final demand goods are produced 
by combining a set of commodity supplied goods. 
Commoditization also decouples the supply and demand 
to some extent with the goal to improve the overall 
resilience of the supply chain.
Mathematically, commoditization can be treated as 
one-to-many mapping from demand to supply.
A hypothetical example for commoditization is shown in figure~\ref{fig:composition}-c. 
Where demand goods are labeled as D1 and D2; and 
commodity supplied goods are
labeled as S1, S2, S3 and S4. 
The arrows connecting the demand goods to the commodity supplied goods show the mapping 
required to build the demand goods by the specific combination of commodity goods.
As shown in figure~\ref{fig:composition}-c the demand D1 can be met 
by the commodity products S1, S2 and S3.
And the demand D2 can be met 
by the commodity products S2 and S3.
Mathematically this can be treated as one-to-many mapping problem from demand to supply 
with selective optimization targets that may improve the resilience of the 
supply chain.

In the context of semiconductor hardware, the commoditization can be defined, 
as the process in which
the final demand architecture is build by 
selecting commodity products and connecting them together 
according to the demand specifications. 
The commodity products can be commercial chiplets that are mass produced 
by commodity firms and can be connected using interconnects to meet the 
final specifications of the demand architecture. 
Building an architecture by connecting a set of commodity chiplets 
can improve the resilience of the semiconductor supply chain in many ways. 

Architects have the choice to pick mixed process nodes, instead of only using the 
cutting edge process nodes to build the final demand architecture. 
Cutting edge process nodes usually have lower yield and have 
higher cost/mm2 ~\ref{sec:composition}. 

Older process nodes usually have higher yield and lower cost/mm2 and 
architects can quantify the PPA (performance, power and area) penalties 
of different architectural choices.
Architects can do a design space exploration to study the impacts 
of picking different mixed process based commodity chiplets on the overall 
cost and yield, with the goal to find the sweet spots that meet the 
specifications of the demand architecture with minimum cost and maximum yield. 
As discussed in section~\ref{sec:} the cost minimization and yield maximization 
can make the supply chain more resilient. 

There are many commodity firms that mass produce commodity 
chiplets for DRAM and flash memory, which are usually build 
using well established older technology nodes and have high yields. 
Architects can 
design memory heavy demand architectures to maximize the use of these commodity
memory chiplets. Such architectural decisions can maximize the yield, minimize the 
cost and improve the resilience of the semiconductor supply chain. 

Commoditization creates redundancy 
in terms of supplied goods 
as a large redundant inventory of commodity supplied goods 
can be procured 
from different commodity firms. 
The redundancy, created by commoditization, can 
make supply chain more resilient to disruptive event e.g. if a 
disruptive event ceases the operation of one or two manufacturing firm 
1) either redundant inventory can be used to respond 
to this disruptive event and/or 2) 

Commoditization promotes 
supply chain collaboration 
by providing many potential suppliers
as there are many commodity firms. 
As discussed in section~\ref{sec:} supply chain collaboration 
makes the supply chain more resilient to disruptive events. 
E.g. when a disruptive event causes some manufacturing unit to cease operations 
the collaboration approach gives the supply chain the flexibility 
to respond to the disruptive event by picking a different commodity supplier.  

Commoditization also improves the flexibility and overall adaptability
of the supply chain due to the availability of the large number of choices for 
commodity suppliers and commodity goods.

\color{black}

\let\comment\undefined


==> base_analysis.tex <==

\iffalse
\section{Basic Analysis}


This model discusses the factors of supply and demand as they relate to the
profit a firm producing chips experiences. It is unique from standard
architectural considerations in that there is the possibility of supply and
demand uncertainty. These uncertainties can render a good plan inferior, and
can completely change the best course of action for an architect. Additionally,
there are some real-world design techniques that can mitigate the impact of
supply and demand uncertainty present within the model.



\nathan{
Composition, adaptation, and dispersion can all increase the resilience of
a chip design when presented with market uncertainties as they enable new
paths to meet consumer chip demands.
}



%\subsection{Decoupling Supply and Demand}

%\textbf{Proposition 1a.} Decoupling supply and demand increases profit when components can be shared across architectures.

%In the deterministic case where supply and demand are coupled, every architecture is a monolith with its own NRE and per-unit costs. Decoupling supply and demand,

%\subsection{Uncertainty Changes Optimal Choice}
\nathan{
As one may expect, introduction of supply uncertainties or demand uncertainties
can change the optimal chip order policies, as can be demonstrated
by existential proofs showing parameter regimes in which this is the case
(proofs not presented) and via experimental verification of the same
(Section~\ref{sec:results}).
}

% \subsubsection{Supply Uncertainty}
% \textbf{Proposition 1.} There exists a scenario in which the optimal production
% strategy to minimize total cost changes once supply uncertainty is introduced.
% 
% \textbf{Proof}
% Define the scenario such that there are two possible mappings $M_{opt}$ and
% $M_{alt}$. For the certain case the best choice of mapping by the architect is
% given by $M_{opt}$ with cost function $CM_{opt}$. An alternative mapping is
% given by $M_{alt}$ with cost function $CM_{alt}$. $M_{alt}$ uses exclusively
% inputs unused by $M_{opt}$ i.e. if $M_{opt}$ produces one chip for every three
% of chiplet A and chiplet B, $M_{alt}$ does nothing with chiplets $A$ and $B$.
% 
% We can write this assumption as
% 
% \begin{equation}
%     M^{-1}_{opt}(\alpha) \neq M^{-1}(\beta) \forall \alpha, \beta
% \end{equation}
% 
% Additionally, assume that these functions are linear with respect to their inputs.
% 
% Now assume there is some supply uncertainty for the input components to
% $M_{opt}$. This can be modeled as weighted coin flip: with probability $1-p$ we
% receive the ordered quantity less those lost to yield, and with probability $p$
% the supply fails entirely due to some unforeseeable issue.  Such an issue could
% be a design flaw, geopolitical or environmental effects harming the foundry, or
% a shortage of the raw materials needed to make the components. In this case,
% there is probability $1-p$ of receiving the same profit we would in the
% deterministic case and probability $p$ of paying for production only to get no
% sales. The change in total cost is given by
% 
% \begin{equation}
%     \Delta TC(p) = p(\vec{Z_{d}}\cdot(\vec{g}+\vec{r}) - \Gamma_{opt}(\vec{x}\vec{y}))
% \end{equation}
% 
% We know that this term is positive as otherwise the cost of making chips in the
% best case would be greater than the value of selling them. This would mean the
% firm's best option is to close up and find a new market.
% 
% If the difference in total cost between $M_{alt}$ and $M_{opt}$ is less than
% $\Delta TC(P)$ for some $p<1$ then $M_{alt}$ becomes a superior choice to
% $M_{opt}$ for supply uncertainty greater or equal to $p$. 
% 
% \subsubsection{Demand Uncertainty}
% 
% \textbf{Proposition 2.} There exists a scenario in which the optimal production
% strategy to minimize total cost changes once demand uncertainty is introduced.
% 
% \textbf{Proof}
% We start again with a simple, single product case.  For the case of certain
% supply and demand, the optimal mapping is $M_{opt}$. For some demand $Z_{d2} <
% Z_{d1}$, the best mapping function is $M_{alt} \neq M_{opt}$. Assume mapping
% functions and cost of mapping functions are linear w.r.t. their inputs.
% 
% %float showing the means on a number-line. 
% %may do a follow-up with slope shown for different p's
% 
% Now assume there is uncertainty in demand from the initial (assumed) value of $Z_{d1}$. With probability $p$ the real demand is actually less than expected with a value of $Z_{d2}$ and with probability $1-p$ the demand remains $Z_{d1}$.
% 
% \begin{equation}
%     Z_d = \begin{cases} Z_{d1} & \text{probability} (1-p) \\ Z_{d2} & \text{probability} (p) \end{cases}
% \end{equation}
% 
% To determine what is worth producing we can look to the change in total cost
% when we make one more processor. Denote the production cost of making one more
% processor $\delta TC_{prod}$ which must be constant as $M$ and $CM$ are linear.
% 
% In the range $(0,Z_{d2})$, our change in total cost per processor made is given by 
% 
% \begin{equation}
%     \delta TC = \delta TC_{prod} - (g+r)
% \end{equation}
% 
% which is both constant and negative provided it is worth making any processors whatsoever.
% 
% In the range $(Z_{d2},Z_{d1})$, our change in total cost per processor created is given by 
% 
% \begin{equation}
%     \delta TC = \delta TC_{prod} - p \cdot h - (1-p) \cdot (g+r)
% \end{equation}
% 
% which for sufficiently large $p$ will be positive.
% 
% Thus there is a sufficient level of uncertainty such that $M_{opt}$ becomes inferior to $M_{alt}$.

\subsection{Tools to Mitigate Uncertainty}
Since uncertainty can impact order policy choices, a good question would be to
ask what choices help to mitigate the impact of uncertainty. Two good tools
which operate directly at opposite ends of the model are composition and
adaptation. Composition involves composing processors from chiplets and can
mitigate the effects of supply uncertainty directly. Adaptation involves
building processors which can be adapted to the different customer demands and
can mitigate demand uncertainty.

\subsubsection{Adaptation Mitigates Demand Uncertainty}

%\textbf{Proposition 3.}
There exists scenarios in which adaptation reduces total cost when demand
uncertainty is introduced.  Consider the following example, which uses simplifying
assumptions for clarity:

Consider a market in which there are two demands, $D_a$ and $D_b$.
These demands can be met by $P_a$ and $P_b$, respectively.  Further,
assume that shortage costs are high, so that profit maximization will mean
ordering sufficient quantities of $P_a$ and $P_b$ to guarantee that there
are no shortages for $D_a$ and $D_b$.

Now assume there is uncertainty in the demand for the two demands.
Specifically, the total is known to be $Z_{d} = Z_{D_a} + Z_{D_b}$ is known,
but $Z_{D_a}$ and $Z_{D_b}$ themselves are unknown.

In this case, orders for $P_a$ and $P_b$ are made so that $Z_{d}$ of each
are produced.

Consider the same scenario, but with an \textit{adaptable} produced good,
$P_c$, which can meet demand for both $D_a$ and $D_b$.  Further, suppose
that the NRE of $P_c$ is less than the sum of the NREs for $P_a$ and $P_b$,
and the unit cost of $P_c$ is less than the sum of the unit costs of $P_a$ and
$P_b$.  With the addition of $P_c$, the profit maximizing policy is to order
\textit{only} $P_c$ in order to meet demand $Z_{D}$.

%next step, introduce a (1+a) multiple to the right-hand-side of the equation


\subsubsection{Composition Helps Supply Uncertainty}

%\textbf{Proposition 4.} 

Increasing the number of possible architectures to meet a demand via
composition can decrease total cost under supply uncertainty.  Once again,
consider this simple example:

Assume there is an optimal architecture $A_{opt}$ produced by $M_{opt}$ and an
alternative architecture $A_{alt}$. Both are composed of one common chiplet and
one distinct chiplet i.e. $A_{opt}$ is composed of chiplets $C_1$ and $C_2$
whereas $A_{alt}$ is composed of $C_1$ and $C_3$.  Further, assume that
shortage costs are high.

Assume one of $C_2 , C_3$ has a major supply disruption and thus fails to be
supplied. For a demand of $Z_d$, ordering $Z_d$ of each chiplet still
guarantees the demand can be met and is therefore the optimal strategy.

Addition of further architectures can additionally reduce total cost under a
major supply disruption, assuming each new architecture reduces the set of
shared chiplets.


\subsection{Dispersion}

Unlike the previous two tools which rely on the mapping from supply to demand,
one can also consider the possibilities for demand mapping onto supply. Consider
the number of mappings that can meet a demand. If this number is multiple, we
say the demand has been dispersed. This can correspond to a redundancy in
supply chains or generalization of designs which can meet demand. Dispersion
moves in the opposite direction of general trends towards singular, specific
hardware. Additionally, it can help with supply uncertainty concerns.

\subsubsection{Dispersion and Supply Uncertainty}

There exists a scenario in which dispersion to two
supplies reduces total cost under uncertainty.

Assume the option of either a specific supplier or two commodity suppliers to
meet a customer's needs. Both cases meet the customer's requirements, and both
have equivalent per-unit costs, yields and NRE cost. In the certain supply case
both are equivalent, though managing a single supply line will almost certainly
be easier.

Now assume there is some uncertainty in the supply chain, represented by a
probability $p$ of the supply chain completely failing for a given supplier.
All three supplies are independent and identically distributed in this way. The
single supply case would have expected shortage cost $pZ_{d}(g+r)$ adding onto
the total cost.

If one purchases $Z_{d}/2 + \epsilon$ units from both suppliers instead, the
expected shortage becomes

\begin{equation}
\begin{split}
    \mathbb{E}[Z_{d}-M(\vec{x}\vec{y})]^{+} & = p^{2}Z_{d} + p(1-p)(Z_{d}-2\epsilon) \\
    & = pZ_{d} - p(1-p)2\epsilon
\end{split}
\end{equation}

Thus the shortage cost decreases as a function of $p$ and $\epsilon$. The
commodity goods are worth producing when their impact on shortage cost is
greater than the additional order cost, or by the inequality

\begin{equation}
p(1-p)(g+r) > \vec{s} \cdot \vec{c} + \Gamma(\vec{s}\vec{y})
\end{equation}

Where $\vec{s}$ is the order quantities needed to produce one good from each
supplier.

% \textbf{Proposition 6.} There is a general strategy for $k$ supply lines which
% will have lower total cost than a single supply line when a simple inequality
% of costs, benefits and probability of failure is true. This inequality is given
% by $\frac{g+r}{c} > \frac{1}{(1-p)-(1-p)^{k}}$, where the left term represents
% the ratio of marginal benefit to marginal cost and the right term is a function
% of the number of supply lines and probability of supply line failure.
% 
% 
% \textbf{Proof}
% Assume we have the choice between one and $n$ suppliers. In either case, all
% suppliers have an independent chance of failure $p$ where none of what is
% ordered arrives. 
% 
% In the case of a single supplier, expected shortage is $pZ_{d}$ units as there
% is probability $p$ of all $Z_{d}$ units being short.
% 
% In the case of $n$ suppliers, we can order $\frac{Z_{d}}{k-1}$ units from each.
% This means that if zero or one of the suppliers fail, there is no shortage.
% 
% Calculating expected shortage gives
% 
% \[
% \begin{split}
%     \frac{Z_{d}}{k-1}\mathbb{E}[[\text{failures}-1]^{+}] &= \frac{Z_{d}}{k-1}(kp-P(failures \geq 1))\\
%     &=\frac{Z_{d}}{k-1}(kp-(1-(1-p)^{k}))\\
%     &=pZ_{d} + \frac{Z_{d}((1-p)^{k}-(1-p))}{k-1}
% \end{split}
% \]
% 
% This is less than the shortage in the single-supply case by 
% 
% \begin{equation}
%     \frac{Z_{d}}{k-1}((1-p)-(1-p)^{k})
% \end{equation}
% 
% Assuming there is a marginal benefit from one more sale given by $g+r$ and a marginal cost to an extra unit ordered given by $c$, the $n$ suppliers are superior when the following inequality holds
% 
% \begin{equation}
%    ((1-p)-(1-p)^{k})(g+r) > c
% \end{equation}
% 
% Rearranging to get the per-unit benefit-to-cost ratio on the lefthand side gives the inequality
% 
% \begin{equation}
%     \frac{g+r}{c} > \frac{1}{(1-p)-(1-p)^{k}}
% \end{equation}
% 
% Assuming there is an NRE component $\omega$ which is paid once for each supplier. Then the inequality becomes 
% 
% \begin{equation}
%     c + \frac{\omega (k-1)^2}{Z_{d}} < ((1-p)-(1-p)^{k})(g+r)
% \end{equation}

\fi


==> costmodel.tex <==
%\label{sec:cost-model}
%We used table 


\iffalse
\begin{table}[]
\begin{tabular}{@{}ccc@{}}
%\label{tab:parameters}
\toprule
Parameter             & Value                                    &  \\ \midrule
Wafer Diameter        & 300mm                                    &  \\
n                     & 13 (1 layer of devices, 12 metal layers) &  \\
$Frac_{crit}$ (wire)  & 0.2625                                   &  \\
$Frac_{crit}$ (logic) & 0.75                                     &  \\
$\alpha$              & 1                                        &  \\ \bottomrule
\end{tabular}
\label{tab:parameters}
\caption{Parameters for cost model.}
\end{table}
\fi

We performed several case studies centered around \SI{22}{\nano\meter} 16, 8,
and 4-core dies. To estimate their area, we scaled the area for a 32-core
monolithic-chip from~\cite{amdnext} based on the number of cores and then
scaled it further to \SI{22}{\nano\meter}.
%For 16-core monolithic-chip we assumed the chip area to be half the 32-core
%monolithic-chip area and for 8-core monolithic-chip we assumed the chip area
%to be one fourth the 32-core monolithic-chip area. All the area numbers are
%scaled to 22nm technology node. 
%\nathan{
%A model is only as good as the data it relies on.  %Thus, 
%}
To estimate the yield of these dies, we used the model in a previous study from AMD~\cite{amdpaper}
($Yield = (1+(D_0/n \cdot A_{crit}) / \alpha)^{-\alpha}$) assuming a
\SI{300}{\nano\meter} wafer, 12 metal layers,  $Frac_{crit}$ (wire)  of 0.2625,
$Frac_{crit}$ (logic) of 0.75, and clustering factor $\alpha$ of 1.
\iffalse
First we calculate the total number of possible dies on a given wafer using the
formula~\cite{ndies}
\begin{equation}
    N_{total} = \pi * (R - \sqrt{A})^2 / A
\end{equation}
Where \(R\) is the radius of wafer, \(R = 150mm\) in our 
case as we did our analysis for $300mm$ wafer. 
We calculated the yield using the analytical yield
model from~\cite{amdpaper}. 
\begin{equation}
Yield = (1+(D_0/n * A_{crit}) / \alpha)^{-\alpha}
\end{equation}

where $D_0$ is the defect density (defects per $m^2$), 
n is the number of vulnerable layers, we 
performed our analysis for n=13 where we assume one 
layer of devices and 12 metal layers as suggested by~\cite{amdpaper}, 
Acrit is the total vulnerable area which is the 
product of die area and $Frac_crit$, which models the 
fact that the yield loss doesn not occur for where there 
are no devices. 
$\alpha$ is the clustering factor 
it models the fact
that defects are typically not perfectly uniformly distributed on the wafer. 
The parameters used for yield calculation are presented in 
Table~\ref{tab:parameters}.
\fi
%\textcolor{red}{
To estimate the unit cost of the dies, we first estimate the 
%number of possible dies on a given wafer using the formula $N_{dies} = (\pi/A_{die})*(W_r - 
%\sqrt{A_{die}})^2$ where $A_{die}$ is the area of the chip scaled to \SI{22}{\nano\meter}
%technology node.
%$W_r$ is the radius of wafer (we used $150mm$ wafer %for our evaluations).
%We then estimated the 
recurring engineering (RE) cost for a given order as 
$RE\_cost = (order/N_{dies})*RE\_wafer\_cost\_logic$, where $RE\_wafer\_cost\_logic = 2.43$ was taken 
from~\cite{tvlsi} (Table IV).  their cost estimates (normalized w.r.t \SI{45}{\nano\meter} wafer cost) are largely based on published industrial data. 
%for \SI{22}{\nano\meter} node (
%All the cost numbers in \cite{tvlsi}(Table IV) are 
%For our cost estimates, we do not differentiate between logic and SRAM, we assume that the entire
%die is made of logic.
To estimate the NRE cost, we again used cost numbers 
from~\cite{tvlsi} (Table IV). NRE cost has two parts, 1) area dependent NRE design cost and 2) area independent NRE mask set cost. We scale the design cost with our core area and add one mask set 
cost per design to estimate the total NRE cost. 
Once we have estimated the RE and NRE costs, we calculate the unit cost of the die using the formula 
$unit\_cost = 2\cdot(RE\_cost + NRE\_cost) / order$.
Using the above methodology, our unit cost estimates are $0.12$, $0.05$ and $0.024$ respectively for 16, 8 and 4 core dies for 
the order of 100M each. 
The unit cost numbers are normalized w.r.t \SI{45}{\nano\meter} wafer cost.
%}
\iffalse
presents the 
NRE design cost per mm2 of silicon area, 
NRE mask set cost, 
Recurring wafer cost per wafer 
and area dependant integration cost for different 
technology nodes. All the cost numbers in the table are 
normalized 
with respect to \SI{45}{\nano\meter} wafer cost. For our analysis
we used cost numbers 
corresponding to \SI{22}{\nano\meter} technology node.
We used numbers from Table IV~\cite{tvlsi} along 
with the die area numbers to calculate the 
unit benefit and the NRE cost for our analytical cost 
model(Section~\ref{sec:model}).

\section{Validation}
\fi

For validation, we calculated the cost of a 32-core monolithic chip and 32-core chip composed of 4 8-core
chiplets through our model. We found the 32-core chip build from composing 8 cores was 1.71× cheaper. 
For comparison, \cite{amdnext} claims that their  
32-core monolithic-chip is $1.69\times$ cheaper to 
build than their 32-core chip  composed using 
4x8-core chiplets. 
%We used the area numbers for 32-core monolithic-chip %($777mm^2$) 
%and 4x8-core chiplets ($4x213mm^2 + 9.7\%$ for integration cost) from~\cite{amdnext}. 
%The reported areas are in 14nm technology node, we
%scale the area to $22nm$ technology
%node. Then we used our cost model along with the cost numbers
%for 22nm technology node
%from~\cite{tvlsi}
%to calculate the cost of 32-core monolithic chip and 
%equivalent chiplet based system (4x8-core chiplet).
%Our results show that it is $1.71\times$ cheaper to 
%build 32-core system as a combination of four 8-core chiplets
%compared to building a 32-core monolithic chip.
%The comparison of cost of monolithic and chiplet based
%systems for both ~\cite{amdnext} and our cost model 
%is presented in Figure~\ref{fig:validation}.
%Our comparison shows that our model is within 
%$\approx1.18\%$ error range compared to the cost 
%comparison reported in ~\cite{amdnext}. We believe that 
%this difference is due to the approximate area 
%scaling for different technology 
%nodes (14nm for~\cite{amdnext} vs 22nm ours). 
\iffalse
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{./images/newfigures/validation.png}
    \caption{Cost of the chiplet based systems is normalized with respect to the cost of the corresponding monolithic chip.}
    \label{fig:validation}
\end{figure}
\fi
The fact that our model and choice of parameters produced a value close to previously reported value from an industry study yields confidence in the trends and analyses generated by our model. 




==> introduction.tex <==
The semiconductor industry is becoming increasingly complex and uncertain due
to a variety of factors. More complex designs may not perform to expectations
or have other issues that delay their production. Cutting edge technology nodes
and fabrication techniques that push the limits of physics carry larger risks
of delays, and put fabs that can't keep up out of business. 20 years ago,
almost 30 companies manufactured integrated circuits at leading-edge
manufacturing processes, whereas only 5 do so today (Intel, Samsung, TSMC,
Micron, and SK Hynix)~\cite{t10}. 

There are uncertainties in the supply of chips from fabrication plants from
natural events like draughts, fires and winter storms that could become more
common with global warming, and geopolitical conflicts that are becoming more
common in areas where semiconductor fabs are concentrated, like the US-China
trade war~\cite{t11} or tensions over Taiwan~\cite{t12}.  Semiconductor supply
chains have become more complicated with additional additional entities being
involved in the value chain. This growth in Vertical Specialization is because
of several reasons. Lowered production costs from economies of scale expanded
end-user applications for semiconductors, creating opportunities for vertically
specialized firms. The increasing capital requirements of semiconductor
manufacturing provided another impetus to vertical specialization, since these
higher fixed costs made it necessary to produce large volumes of a limited
array of semiconductor components in order to achieve lower unit costs. The
design cycle for new semiconductor products also has become shorter and product
lifecycles more uncertain, making it more difficult to determine whether demand
for a single product will fully utilize the capacity of a fabrication facility
that is devoted exclusively to a particular product and increasing the risks of
investing in such “dedicated” capacity~\cite{ITIF}. As a result of these
factors, the semiconductor ecosystem has evolved from fully integrated firms in
the 1950s to a global set of firms that by the 2010s specialized in discrete
activities such as RandD, design, machine tooling, components, foundries,
assembly, test, and packaging~\cite{SCValchainFloat_src}. 

\begin{figure}
    \centering
    \includegraphics[width=4cm]{./images/SC_Value_Chain_Figure.png}
    \caption{Increasing complexity of Semiconductor Chain over years}
    \label{fig:SC_complex}
\end{figure}

The semiconductor industry is very capital and R and D intensive - according to
SIA (Semiconductor Industry Association), it is one of the most capital
intensive industries in the country~\cite{t13}. As a result, Semiconductor
companies need access to large global markets so they can amortize and recoup
their costs across a single large global marketplace~\cite{ITIF}.  Each segment
of the semiconductor value chain has, on average, 25 countries involved in the
direct supply chain and 23 countries involved in support functions. Over 12
countries have enterprises directly engaged in semiconductor chip design, 39
countries have at least 1 semiconductor fabrication facility, while over 25
countries have enterprises engaging in ATP activities ~\cite{ITIF}. The typical
production process toward a final electronics product can see the underlying
semiconductors within it cross international borders 70 or more times in a
process that takes over 100 days and includes 3 full trips around the
world~\cite{ITIF}. 
\iffalse
Another set of companies, including Applied Materials (United States), ASML
(the Netherlands), KLA Tencor (United States), and Lam Research (United
States), manufacture the machines and tooling equipment that run semiconductor
fabs. Finally, a number of enterprises, especially ones from Japan, South
Korea, and Taiwan, manufacture chemicals and components essential to the
semiconductor manufacturing process. For instance, fluorinated polyimides, a
group of specialty polymers that provide physical strength and heat resistance,
are produced by Daikin Chemical (Japan), DuPont (United States), Kaneka Asahi
Kasei (Japan), and Taimide Technology (Taiwan). Photoresists are critical
components that provide the patterns used to build micro-circuitry into
semiconductors. The Japanese firms JSR Corporation, Shin-Etsu Chemical Company,
Sumitomo Chemical, and Tokyo Ohka Kogyo Company manufacture photoresists, as do
the Korean players Dongjin Semiconductor Company and Dongwoo Fine Chemicals.
Portland, Oregon-based Inpria is the only U.S.-headquartered photoresists
manufacturer, while European players have abandoned the field
altogether~\cite{ITIF}\footnote{This paragraph may be better represented as a
table of specialized companies integral to manufacturing semiconductors}.
\fi

Uncertainties are not exclusive to just the supply of semiconductors - as
semiconductors become increasingly pervasive and accessible to more diverse
consumers, there is increasingly fluctuating demands from events like the
pandemic, crypto\-currency booms and crashes etc, and also from increasingly
stiff competition within the industry.

All of these factors that make the semiconductor supply chain more complex lead
to a bullwhip effect where there are increasing swings in inventory in response
to shifts in consumer demand as one moves further up the supply
chain~\cite{bullwhip_src}. 
\iffalse
Protectionist policies where governments funnel money. semiconductor companies
cannot face excess, non-market-based competition, such as governments pumping
in hundreds of billions of dollars in subsidies, which unfairly disadvantages
enterprises that are attempting to compete on genuinely market-based
terms~\cite{ITIF}. In other words, if leading-edge companies cannot be assured
that they can earn a reasonable, risk-adjusted rate of return on their
investments—which is put in doubt by some governments such as China investing
massive amounts of money to create a domestic semiconductor industry—then the
leading companies will cut R and D and capital expenditures~\cite{ITIF}. 


Table 3 shows a sampling of some unpredictable events and their financial
impact on the foundry. In most of the cases it's reasonable to assume that the
events caused a similar, if not more monetary loss to the chip companies that
purchased from these foundries. 
\fi

\begin{table*}[]
\small
\centering
\caption{\small Un-forcastable events, loss to foundry as result and time to recover}
\begin{tabular}{@{}llll@{}}
\toprule
Event                                                   & Loss to foundry   (\$)                          & How long to recover & When?      \\ \midrule
Power outage at TSMCs legacy process fab~\cite{t1}                & 28-35Mil   (30-40k wafers)                      & 12   hours          & Aug-21     \\
Texas winter storm froze Samsung foundry~\cite{t2}                & 286-357   Mil ($\sim$71k wafers)                & 1   month           & Apr-21     \\
Texas winter storm froze NXP foundry~\cite{t3}                    & $\sim$100   Mil                                 & 1   month           & Apr-21     \\
Fire at Renesas facility in Naka Japan~\cite{t4}                  & 171   Mill                                      & 1   month           & Mar-21     \\
\{Global Foundries quits on 7nm,   AMD shifts to tsmc\}~\cite{t5}~\cite{t6} & \{$\sim$4.255B loss just from AMD\}             & \{Permanent\}       & \{Aug-19\} \\
Current Chip shortage due to surge in demmand~\cite{t7}           & 60   Billion (what's the amount for foundries?) & 2+   years          & 2020       \\
China - US trade war causes TSMC to loose HWAWEI sales~\cite{t8}  & 13\%   of TSMCs revenue $\sim$= 455Mil          & 2   months          & 2020       \\
Fire at Asahi Kasei Foundry~\cite{t9}                             & 100Mil   \$** (unreliable source?               & ?                   & Feb-21     \\ \bottomrule
\end{tabular}
\end{table*}

\iffalse
\fi
From Table 1 it is clear that unpredictable events and delays can have a large
cost to foundries and especially for the companies whom the foundries supply.
This seems to be symptomatic of a larger problem with supply chain resiliency
in the semiconductor industry. As the ongoing chip shortage has brought to
light, semiconductor supply chains have several inherent weaknesses that make
them less resilient to supply fluctuations such as in the examples below, and
unforecasted customer demand spikes, as is currently occurring. Table 2
contains a comparison of various facets of good supply chains with those of
semiconductor supply chains:

\begin{table}[]
\tiny
\centering
\caption{\small Comparison of characteristics of resilient supply chains to Si
    supply chain}\footnote{update the table to include examples of industries
    that have the ideal supply chain characteristics}
\begin{tabular}{@{}ll@{}}
\toprule


Ideal Resilient Supply chain                                                                                                                                                                                                                                    & Semiconductor supply chain                                                                                                                                                                                                                              \\ \midrule
\begin{tabular}[c]{@{}l@{}}Multiple suppliers for the same product that aren't affected by similar \\ geographic or geopolitical conditions that can ramp up or slow down \\ production with linear cost scaling\end{tabular}                                   & \begin{tabular}[c]{@{}l@{}}Increasingly few fabs (suppliers) that are becoming more \\ geographically clustered; for high performance chips, \\ usually only one supplier.\end{tabular}                                                                 \\
Financially feasible to buffer stocks for demand spikes or supply drops                                                                                                                                                                                         & \begin{tabular}[c]{@{}l@{}}Buffering chips usually not financially feasible due to \\ cost and limited product lifespan of chips\end{tabular}                                                                                                           \\
\begin{tabular}[c]{@{}l@{}}Has intermediate components that can be sourced from different \\ suppliers are composed to create different final goods to adapt to\\  changing demand profiles or to maximize profits under high \\ demand situations\end{tabular} & \begin{tabular}[c]{@{}l@{}}Chiplet design which accomplishes a similar thing is \\ still new and not widely adopted. In current designs, \\ all or most of the chiplets in a package are manufactured\\  in the same foundry\end{tabular}               \\
\begin{tabular}[c]{@{}l@{}}Final produced goods are able to satisfy different demand streams \\ (like how a corn farmer satisfies demand for both corn-based food \\ and ethanol with his goods)\end{tabular}                                                   & \begin{tabular}[c]{@{}l@{}}Final produced good (chip) only satisfies one type of \\ demand stream.\end{tabular}                                                                                                                                         \\
\begin{tabular}[c]{@{}l@{}}Supply chain can quickly scale down or scale up production as \\ forecasts for demmand change\end{tabular}                                                                                                                           & \begin{tabular}[c]{@{}l@{}}Many foundries run at or close to full capacity, and takes \\ a 3-5 years to build a new foundry to increase supply. \\ Large lead time of 28-30 Weeks makes it hard to change \\ production levels either way.\end{tabular} \\ \bottomrule
\end{tabular}
\end{table}

These risk factors for the semiconductor supply chain are especially
concerning, because the factors for uncertainty in the semiconductor industry
are trending the wrong way. On the supply side, climate change is making fires,
and droughts like the recent one in Taiwan increasingly more common,
geopolitical tensions in the world are rising, and increasingly complex designs
and lithography techniques are steadily reducing the number of facilities that
can make cutting-edge chips. Demand for chips is also becoming more volatile as
computer chips begin to be utilized in more and more fields, with little
substitutability between fields (spike in demand in one field (eg. GPUs when
cryptocurrency values surge) cannot be full filled by slump or average demand
in another field.  

Improving supply chain resiliency for semiconductor chips has traditionally
been thought of as more of a logistics and planning/forecasting problem, but
computer architects can also play a role in improving supply chain resiliency
through creating novel architectures that allow remedial of specific risk
factors in the supply chain, as we try to show in this paper.\footnote{Will try
to find a more concrete example here of some company improving their supply
chain resilience through better product design}

Semiconductor supply chains demonstrate supply and demand uncertainties. These
uncertainties depend on a large number of geopolitical and logistical factors
and lead to increased costs. In this paper, we ask the question: can chip
architects make decisions that reduce the impact of supply chain uncertainties?

We identify three classes of interventions that chip architects can perform to
improve supply chain resilience. Architects can support {\em composition} in
design such that the same chip can be built using a different set of components
(IPs, chiplets, etc.). This enables chip demand to be satisfied even if supply
of some components are constrained. Similarly, architects can support {\em
adaptation} in design such that a given chip can be used as a replacement for a
different chip. This enables any chip shortage to be addressed using a
different chip that may be available.  Architects can also identify
opportunities for {\em disperion} - i.e., when parts of a chip can be
implemented using a technology or an IP that can be sourced by a large number
of suppliers. Dispersion allows disruptions in supply to be compensated by
other suppliers.    
 
To evaluate the effects of composition, adaptation, and dispersion on supply
chain resilience, we develop a model that estimates the impact of semiconductor
supply chain uncertainties on overall cost. The model considers both the cost
of shortages and overages that result from supply chain (and yield)
uncertainties as well as recurring and non-recurring costs of chip production
and is general enough to represent different architectural interventions. 

We provide proofs using this model that architectural interventions such as
composition, adaptation, and dispersion can indeed reduce the impact of
uncertainties - these proofs are theoretical and are independent of the values
that the model parameters may take. 

The model also allows us to make intelligent architectural decisions that
improve resilience to supply chain uncertainties. To understand and evaluate
architectural decision-making in presence of supply chain uncertainties, we
consider three case studies, one for each type of architectural intervention.
Our case studies confirm that each architectural intervention can provide
significant resilience to supply chain uncertainties. 


==> mapping_costs.tex <==
\label{sec:mapping_costs}
\begin{figure}
    \centering
    \includegraphics[width=10cm]{./images/newfigures/perfvsprice.png}
    \caption{Performance vs Price of Intel and AMD chips}
    \label{fig:perfvsprice}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=10cm]{./images/newfigures/adaptation_cost.png}
    \caption{Price of Adapted Chips}
    \label{fig:adaptation_cost}
\end{figure}

In \ref{sec:results} we explore multiple way to reduce the affect of demand and supply uncertainty on \textit{Total Cost} and offer architectural suggestions to implement these techniques. These are all some form on composition, adaptation and/or dispersion. We use the mapping decision variable in our model to realise these techniques and $\Gamma$ to incur any cost associated with that mapping.

For composition, we primarily explore monolithic chip vs chiplet based designs. Work done by AMD \cite{amdepycandryzen} suggests that the overall cost producing a chiplet based chip is lower since chip manufacturers bear the costs of low yield for monolithic chips. Since smaller chips are given higher yield and lower unit costs in the model, this is accounted for. Further, chiplet based designs have a variable interposer costs. Hence for any mapping that performs composition, $\gamma$ takes a value for an interposer of area equal to the overall chip area and also performance lost due to the use of an interposer. 

For adaptation, we explore multiple techniques and hence use various metrics to realize intervention costs. The baseline adaptation technique assumes mappings from larger chips to smaller chips, i.e, a 16-core or 8-core chip can be rebadged and sold as an 8-core or 4-core chip respectively, given market constraints. Take Figure~\ref{fig:adaptation_cost}) that shows the relationship between prices of monolithic and adapted chips. Prices for chips with the same core count are roughly the same. Hence we allow for both unit benefit and the mapping cost of this intervention to be zero. 


Alongside these baseline techniques we explore more complex adaptation and composition techniques. For example, we analyze the role that multi-isa chips can have as an adaptation technique. A multi-isa chip allows to service demand from two separate markets with the same chip. But chip manufacturers incur a performance cost as a result of an adaptable design. We use the data from Figure~\ref{fig:perfvsprice}) to add a cost to loss in performance. The figure shows the price and performance of various processors from the Intel 10000 series and the AMD 3000 series. We estimate the performance loss caused due to the technique and map it to a cost using this data.

==> methodology.tex <==
%\ subsection{Optimization}

%\nathan{
To accurately assess the impact of architectural techniques on supply
chain resilience, we must identify \textit{optimal} chip order and
chip mapping policies that minimizes expected total cost, $\E{TC}$:
\( \argmin_{\vec{x}, \vec{M^q}}\E{TC} \),
subject to several constraints, including constraints enforcing NRE is paid
for produced chips, mappings can only be used if an appropriate number of
produced chips were obtained, etc.
\iffalse
%Otherwise, it would be difficult to discern whether
%the impacts of the interventions are a a result of the interventions themselves,
%or are due to the suboptimal managerial policies.}
One can use $\E{TC}$ as the objective of an optimization problem with the goal
of minimizing expected total cost (or, dually, maximize total profit) with
$x$ and $M_x$, the chip order and mapping policies,  as decision variables.
However, this requires several constraints.

Assume $n$ produced goods and $m$ demanded goods, and $k$ mappings $M$.
Consider mappings to be parameterized as follows: the $j$'th mapping is given
by $M_j = (M^i_j, M^o_i)$ where $M^i_j$ is a vector of length $n$ where the
$k$th index corresponds to the number of the $k$th produced good needed to
perform the mapping, and $M^o_i$ represents the demand good which the mapping
produces.  The quantity of the usage of $M_j$ is designated as $M^q_j$.

\begin{itemize}
    \item $TC_{NRE} = \sum_{i} \sign{x_i} \cdot n_i$ - If $x_i$ is ordered,
        then NRE costs must be paid.
    \item $TC_{RE} = \sum_{i} x_i\cdot c_i$
    \item $TC_{prod} = TC_{NRE} + TC_{RE}$ - Total cost of production is the
        sum of NRE and RE.
    \item $\forall i \in \{1\ldots n\}, b_i = x_iy_iZ_{s_i}$ - The number of
        produced goods built is the product of the order, the yield, and
        the supply uncertainty factor.
    \item $\forall i \in \{1\ldots m\}, 
        B_i = \sum_{j}M^q_j \cdot I_{M^o_j = i}$ -
        The number of demand goods built is equal to the sum of the quantities
        of the mappings.
    \item $\forall k \in \{1\ldots n\}, b_k \geq \sum_{j} M^q_j \cdot M^i_k$ -
        Mappings can only be used if an appropriate number of produced goods
        were obtained.
    \item $TC_{benefit} = \sum_i \max\{b_i, Z_{d_i}\} \cdot r_i$.
    \item $TC_{shortage} = \sum_i \reLU(Z_d - b_i) g_i$.
    \item $TC_{salvage} = \sum_i \reLU(b_i - Z_d) h_i$.
    \item $TC_{\Gamma} = \sum_i \Gamma_i \cdot M^q_i$.
\end{itemize}

With these constrains in place, the optimization problem is
\[
    \min_{x, M^q} \E{TC_{prod} + TC_{shortage} + TC_{\Gamma} - TC_{benefit}
          - TC_{salvage}}.
\]

%\iffalse
Solving such an optimization problem is complicated by a number of factors.
First, there are multiple values which are constrained to integer values
(e.g., $x$, $M^q$).  Second, there are several non-linear constraints
(e.g., $TC_{benefit}, TC_{shortage}$, and $TC_{salvage}$).  Third,
The $Z_d$ and $Z_s$ are probability distributions, not numeric parameters.
Combined, these factors make 
\fi
Since this optimization problem is a stochastic mixed-integer non-linear
program, we use a multistage stochastic program with recourse
(MSPR)~\cite{mspr,mspr2} to solve it.
%this
%optimization problem.
The idea of an MSPR is to sequence the decision variables across multiple
temporal stages, with latter stages having `recourse' to information which was
not available in earlier stages. We perform optimizations under different
recourses---one where demand is known exactly, the other where the actual
demand is unknown. We use the global solver in the commercial mathematical
programming software Lingo~\cite{lingo}
\iffalse.
As the volume of chips produced and demanded is necessarily high (if not, 
NRE costs dominate), we relaxed the integer requirement for $x$ and $M^q$ to
be non-negative real values.  We use Lingo's global solver to find global
optima, rather than its local solver.
As the key inputs to a specific market scenario are the collection of produced
goods, the collection of demand goods, and the collection of mappings,
\fi
for finding globally optimal chip orders and mappings.
We generate Lingo models using a Rust library which transforms
collections of produced goods, demanded goods, mappings, and additional
constraints into Lingo models.

For each produced chip considered, we used the analytical cost model of
Section~\ref{sec:model} to determine NRE costs and unit costs. Unit benefits
were computed as follows $r = 2\left(c + \frac{n}{B}\right)$ (assuming a 50\%
gross margin).

In all experiments, unless otherwise stated,
$B = 10^8$,
$Z_d\sim \mathcal{N}(\mu=1, \sigma^2=0.0278)$, while
$Z_s\sim \mathcal{N}(\mu=1, \sigma^2=0.01736)$.
We study a range of variances.
%for supply and demand that we observed for
%different semiconductor manufacturers in the recent
%past~\cite{noauthor_gartner_nodate}. 
Since publicly available
data~\cite{lee_semiconductors_2022,noauthor_results_2022,noauthor_coronavirus_nodate, noauthor_gartner_nodate}
suggests that most fluctuations of semiconductor products remain within $\pm 50\%$ of
expectation, we picked the default variances of supply and demand disruption
such that three standard deviations fit into this range. In several
experiments, $Z_d$ and $Z_s$ are modeled with discrete random variables which
can take one of two values, $0$ or some positive number. In these cases, the
positive number is chosen to ensure $\E{Z_d}=1$ and $\E{Z_s}=1$.
Unless otherwise stated, all distributions are independent, and salvage value
is zero. Due to the importance of time-to-market, unless otherwise stated, unit
shortage cost is equal to unit cost.

\begin{figure}
    \centering
    %\includegraphics[width=6cm]{./images/newfigures/Uncertainity_in_semi_chain.png}
    \includegraphics[width=0.80\linewidth]{./images/Price_data/Comp_cost.png}
    \caption{Performance cost of Monolithic chips vs Chiplets}
    \label{fig:CostOfComp}
\end{figure}

For adaptation and dispersion mappings, $\Gamma$ values are zero, while for
composition mappings, $\Gamma$ takes a value for an interposer
of area equal to the overall chip area and also performance lost due to the use of an interposer. The interposer costs are estimated using the
cost model of Section~\ref{sec:model}.  In certain regimes, supply
constraints are placed on interposers themselves.  In these cases, interposers
are modeled as a stand-alone produced good, and composition mappings require
chiplets and interposers as inputs, and $\Gamma$ values are set to zero. And to take into account the cost of a monolithic chip vs a chiplet based design, we study the variation in performance as shown in Figure~\ref{fig:CostOfComp}). This performance loss is then translated into a change in selling price which is added as an additional mapping cost as opposed to varying unit benefit. 



==> model.tex <==
\section{The Model}

The above discussion of the benefits of the different interventions, while
being theoretically sound, falls short in several ways. Firstly, it does not
attempt to quantify how much each intervention could theoretically benefit a
manufacturer in the context of the semiconductor industry. Secondly, there is
no way to asses and verify how interventions perform under different situations
(variable supply, variable demand, correlated and uncorrelated suppliers etc.).
And finally, there is no way to compare relative the efficacy of the
interventions in different situations just on the basis of their theoretical
benefits.

To address all these shortcomings, we present a mathematical cost model of a
typical semiconductor supply chain. This model will be capable of accommodating
the three previously discussed interventions. It will also be able to simulate
the effects of major sources of uncertainty in the semiconductor supply chain
discussed previously. The model will be able to give a rough quantification of
the benefits of each intervention under different circumstances on a comparable
basis, thereby addressing the major shortcoming discussed above. 

%\subsection{SetupI}
Assume there is a firm which produces computer chips for customers. The
customers have some requirements for the chip, and the firm sells them chips
which will meet or beat these requirements. The firm's primary goal is to
maximize profit in selling these chips. We explore a model for deriving this
profit from supply and demand both with and without uncertainty.


\begin{table}
    \centering
    \begin{tabular}{|c|c|} \hline
        Parameters &  \\ 
        $r$ & Unit Benefit \\
        $g$ & Shortage Cost \\
        $h$ & Salvage Value \\
        $y$ & Yield Rate    \\
        $c$ & Per-Unit Cost \\
        $n$ & NRE Cost \\
        $Z_s$ & Supply \\
        $Z_d$ & Demand \\
        $M_x$ & Family of Mapping Functions \\
        $\Gamma_x$ & Family of Cost Functions\\ \hline
        Decision Variables & \\ 
        $x$ & Order Quantity \\ \hline
        Calculated Values&\\
        $o$ & Indicator for $x>0$\\ \hline
    \end{tabular}
    \caption{Complete Parameters}
    \label{tab:ComPar}
\end{table}

\subsection{The Certain Case}


We say that demand for a chip is certain when the number of chips demanded with
a given set of requirements is known from the beginning. This quantity of chips
demanded is given by $\vec{Z_{d}}$ and is a constant. $\vec{Z_{d}}$ represents
the maximum units of each demanded chip that can be sold, with each sale
assigned a benefit to the firm $\vec{r}$. Any chips produced beyond
$\vec{Z_{d}}$ are salvaged with salvage value to the firm $\vec{h}$. For every
potential sale missed there is an associated shortage cost to the firm
$\vec{g}$. The benefit represents sales price, whereas salvage represents the
value derived from scrapping or repurposing the chip. Shortage represents lost
back orders.

Assuming we sell $\vec{\alpha}$ chips with a shortage of $\vec{\beta}$ units
and overage of $\vec{\gamma}$, the total cost to the firm on the demand side is
given by

\begin{equation}
    TC_{dem} = \vec{\beta}\cdot\vec{g} - \vec{\alpha}\cdot\vec{r} - \vec{\gamma}\cdot\vec{h}
\end{equation}

\begin{align}
    \beta_{i} = [Z_{di}-p_{i}]^{+} \\
    \gamma_{i} = [p_{i}-Z_{di}]^{+}
\end{align}

In order to sell these chips to the customer, we must first produce them. In
order to do this, we order input components $\vec{x}$. These components can be
completed chips or components to a final chip (i.e. chiplets). The components
each have an associated per-unit cost $\vec{c}$ to ordering them as well as a
non-recurring engineering cost $\vec{n}$ associated with designing and tooling
to be able to produce a given component. We define the ordered vector $\vec{o}$
so that $o_{i}$ is zero if and only if $x_{i}$ is zero. Thus $\vec{o}$ states
which components, chip or chiplet, will be designed and produced for sale.

With these terms, the cost of ordering components can be given by

\begin{equation}
    TC_{prod} = \vec{x}\cdot\vec{c} + \vec{o}\cdot\vec{n}
\end{equation}

As of this point, we have two decoupled cost functions with no clear link. To
link these two, we present the mapping function
$M:\mathbb{R}^{n}\times\mathbb{R}^{m}\mapsto\mathbb{R}^{m}$. This function,
which can be selected based on available architectures and their input
components, maps input components $\vec{x}$ to saleable chips $\vec{p}$. It is
given the components received and the demand and uses this to determine what
demand goods will be produced. In the event that demand cannot be known at the
time production of final goods occurs, then it is disregarded as an input to
the mapping function such that we see

\begin{equation}
    M(\vec{x},\vec{Z_{d1}})=M(\vec{x},\vec{Z_{d2}}) \forall \vec{Z_{d1}}, \vec{Z_{d2}} 
\end{equation}

Additionally, there is a cost function associated with the selected mapping
function $\Gamma: \mathbb{R}^{n}\times\mathbb{R}^{m}\mapsto\mathbb{R}$ which
takes the same input components and returns the total cost to assemble from
those input components the saleable processors $\vec{p}$.

Thus the total cost is given by the sum of the cost of ordering components,
mapping these components into processors and selling these processors.

\begin{equation}
    TC = TC_{prod} + \Gamma(\vec{x},\vec{Z_{d}}) + TC_{dem}
\end{equation}

If we assume the ordered chiplets do not have perfect yield, and model the
average yield as $\vec{y}$, then the equation changes only slightly to 

\begin{equation}
    TC = TC_{prod} + \Gamma(\vec{x}\circ\vec{y},\vec{Z_{d}}) + TC_{dem}
\end{equation}

with final component equations

\begin{align}
    TC_{prod} =& \vec{x}\cdot\vec{c} + \vec{o}\cdot\vec{n} \\
    \begin{split}
    TC_{dem} =& (\vec{g}+\vec{r})\cdot[\vec{Z_{d}}-M(\vec{x}\circ\vec{y},\vec{Z_{d}})]^{+} \\
    & - \vec{h}\cdot[M(\vec{x}\circ\vec{y},\vec{Z_{d}})-\vec{Z_{d}}]^{+} \\
    & - \vec{r}\cdot\vec{Z_{d}}
    \end{split}
\end{align}

While the choice of order quantities and sales figures are largely outside of
the architect's hands, the mapping function and its subsequent cost function
are directly controlled by the architect's decisions. A different choice in
terms of tech node, memory sizing, or chiplet use can have major effects on how
ordered components are turned into saleable goods. Additionally, the
architect's decisions inform what to do when supply and demand are not as
certain as they are here.

\subsection{The Uncertain Case}

In the certain case, pre-existing knowledge of supply and demand allows us to
plan out our chip production exactly. If we desire to meet demand perfectly, we
could do so. If we wish to overproduce to starve out competitors for the same
supply line, we can do so. In the real world we cannot perfectly plan either
production or demand and so uncertainty is introduced.

We start with supply uncertainty. To model this, there is an additional
parameter $\vec{Z_{s}}$ which is a random variable such that our total cost is
now

\begin{equation}
    \mathop{\mathbb{E}}[TC] = TC_{prod} + \mathop{\mathbb{E}}_{\vec{Z_{s}}}[\Gamma(\vec{x}\vec{y}\vec{Z_{s}},\vec{Z_{d}})]  + \mathop{\mathbb{E}}_{\vec{Z_{s}}}[TC_{dem}]
\end{equation}

where both the mapping cost to assemble the chips and the demand costs
associated with sales are dependent on $Z_{s}$, thus we take the expectation
over all of its possible values.

for uncertainty in demand, the only change necessary is to instead make demand
$\vec{Z_{d}}$ a random variable for the demand of each chip. This adds the
simple modification

\begin{equation}
    \mathop{\mathbb{E}}[TC] = TC_{prod} + \mathop{\mathbb{E}}_{\vec{Z_{s}}}[\Gamma(\vec{x}\vec{y}\vec{Z_{s}})]  + \mathop{\mathbb{E}}_{\vec{Z_{s}},\vec{Z_{d}}}[TC_{dem}]
\end{equation}

the component terms are given by 
\begin{align}
    TC_{prod} =& \vec{x}\cdot\vec{c} + \vec{o}\cdot\vec{n} \\
    \begin{split}
    TC_{dem} =& (\vec{g}+\vec{r})\cdot[\vec{Z_{d}}-M(\vec{x}\circ\vec{y}\circ\vec{Z_{s}},\vec{Z_{d}})]^{+} \\
    & - \vec{h}\cdot[M(\vec{x}\circ\vec{y}\circ\vec{Z_{s}},\vec{Z_{d}})-\vec{Z_{d}}]^{+} \\
    & - \vec{r}\cdot\vec{Z_{d}}
    \end{split}
\end{align}
\textbf{\textcolor{red}{Look at Zs and Zd disc.}} as the sales terms are taken
under the joint expectation of both uncertainties, there are many possibilities
to consider. This makes determining the best architectural choices nontrivial
with respect to supply and demand. It may even render the best choices in the
certain case inferior in the uncertain case.

\subsection{Optimization}

We can use $\E{TC}$ as the objective of an optimization problem with the goal
of minimizing expected total cost (or, dually, maximize total profit) with
$x$ and $M_x$ as decision variables.
However, to do so we must first determine constraints.
Given $n$ produced
goods and $m$ demanded goods, and $k$ mappings $M$.  Consider mappings to be
parameterized as follows: the $j$'th mapping, $M_j = (M^i_j, M^o_i)$ where
$M^i_j$ is a vector of length $n$ where the $k$th index corresponds to
the number of the $k$th produced good needed to perform the mapping, and
$M^o_i$ represents the demand good which the mapping produces.  We designate
the quantity of the usage of $M_j$ as $M^q_j$.

\begin{itemize}
    \item $TC_{NRE} = \sum_{i} \sign{x_i} \cdot n_i$ - If $x_i$ is ordered,
        then NRE costs must be paid.
    \item $TC_{RE} = \sum_{i} x_i\cdot c_i$
    \item $TC_{prod} = TC_{NRE} + TC_{RE}$ - Total cost of production is the
        sum of NRE and RE.
    \item $\forall i \in \{1\ldots n\}, b_i = x_iy_iZ_{s_i}$ - The number of
        produced goods built is the product of the order, the yield, and
        the supply uncertainty factor.
    \item $\forall i \in \{1\ldots m\}, 
        B_i = \sum_{j}M^q_j \cdot I_{M^o_j = i}$ -
        The number of demand goods built is equal to the sum of the quantites
        of the mappings.
    \item $\forall k \in \{1\ldots n\}, b_k \geq \sum_{j} M^q_j \cdot M^i_k$ -
        Mappings can only be used if an appropriate number of produced goods
        were obtained.
    \item $TC_{benefit} = \sum_i \max\{b_i, Z_{d_i}\} \cdot r_i$.
    \item $TC_{shortage} = \sum_i \reLU(Z_d - b_i) g_i$.
    \item $TC_{salvage} = \sum_i \reLU(b_i - Z_d) h_i$.
    \item $TC_{\Gamma} = \sum_i \Gamma_i \cdot M^q_i$.
\end{itemize}

With these constrains in place, the optimization problem is
\[
    \min_{x, M^q} \E{TC_{prod} + TC_{shortage} + TC_{\Gamma} - TC_{benefit}
          - TC_{salvage}}.
\]

Solving such an optimization problem is complicated by a number of factors.
First, there are multiple values which are constrained to integer values
(e.g., $x$, $M^q$).  Second, there are several non-linear constraints
(e.g., $TC_{benefit}, TC_{shortage}$, and $TC_{salvage}$).  Third,
The $Z_d$ and $Z_s$ are probability distributions, not numeric parameters.
Combined, these factors make the optimization problem a stochastic mixed
integer non-linear program.

In order to solve this program, we model it as a multistage stochastic
program with recourse (MSPR).
The idea of an MSPR is to sequence the decision variables across multiple
temporal stages, with latter stages having `recourse' to information which
was not available in earlier stages.
In stage 1, we decide on $x$ with no knowledge about supply and demand
uncertainty beyond the shape of their distribution.
Since the constraints require that the quantities of each produced good
built are known before the quantities of each mapping can be determined,
$M^q$ is determined in stage 2 with recourse to supply uncertainty.
Depending on the specifics of the modeling scenario, it may make sense
to give the $M^q$ decision recourse to demand uncertainty, as well.
For example, the decision to sell a 16-core processor as an 8-core processor
can be made very late in the production process, as disabling cores can
be done via firmware. Table~\ref{tab:recourse} summarizes the staging
of the decision variables and recourse parameters.

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\centering
\begin{tabular}{@{}ccc@{}}
\toprule
\multicolumn{1}{l}{\textbf{Variable}} & \multicolumn{1}{l}{\textbf{Decision Stage}} & \multicolumn{1}{l}{\textbf{Recourse Stage}} \\ \midrule
$x$   & 1 & -      \\
$M^q$ & 2 & -      \\
$Z_s$ & - & 2      \\
$Z_d$ & - & 2 or 3 \\ \bottomrule
\end{tabular}
\caption{Staging for Decision Variables and Recourse Parameters}
\label{tab:recourse}
\end{table}

\subsection{Solving}

We used the commercial mathematical programming software Lingo~\cite{}.
As the volume of chips produced and demanded is necessarily high (if not, 
NRE costs dominate), we relaxed the integer requirement for $x$ and $M^q$ to
be non-negative real values.

As the key inputs to a specific market scenario are the collection of produced
goods, the collection of demand goods, and the collection of mappings,
we also built a library with Rust API which produces Lingo models from
sets of produced goods, demand goods, and mappings.




==> motivation.tex <==

The semiconductor industry is becoming increasingly complex and uncertain due to a variety of factors. More complex designs may not perform to expectations or have other issues that delay their production. Cutting edge technology nodes and fabrication techniques that push the limits of physics carry larger risks of delays, and put fabs that can't keep up out of business. 20 years ago, almost 30 companies manufactured integrated circuits at leading-edge manufacturing processes, whereas only 5 do so today (Intel, Samsung, TSMC, Micron, and SK Hynix)~\cite{t10}. 
\\

There are uncertainties in the supply of chips from fabrication plants from natural events like draughts, fires and winter storms that could become more common with global warming, and geopolitical conflicts that are becoming more common in areas where semiconductor fabs are concentrated, like the US-China trade war~\cite{t11} or tensions over Taiwan~\cite{t12}. 
Semiconductor supply chains have become more complicated with additional additional entities being involved in the value chain. This growth in Vertical Specialization is because of several reasons. Lowered production costs from economies of scale expanded end-user applications for semiconductors, creating opportunities for vertically specialized firms. The increasing capital requirements of semiconductor manufacturing provided another impetus to vertical specialization, since these higher fixed costs made it necessary to produce large volumes of a limited array of semiconductor components in order to achieve lower unit costs. The design cycle for new semiconductor products also has become shorter and product lifecycles more uncertain, making it more difficult to determine whether demand for a single product will fully utilize the capacity of a fabrication facility that is devoted exclusively to a particular product and increasing the risks of investing in such “dedicated” capacity~\cite{ITIF}. As a result of these factors, the semiconductor ecosystem has evolved from fully integrated firms in the 1950s to a global set of firms that by the 2010s specialized in discrete activities such as RandD, design, machine tooling, components, foundries, assembly, test, and packaging~\cite{SCValchainFloat_src}. 
\begin{figure}
    \centering
    \includegraphics[width=4cm]{./images/SC_Value_Chain_Figure.png}
    \caption{Increasing complexity of Semiconductor Chain over years}
    \label{fig:SC_complex}
\end{figure}
\\

The semiconductor industry is very capital and R and D intensive - according to SIA (Semiconductor Industry Association), it is one of the most capital intensive industries in the country~\cite{t13}. As a result, Semiconductor companies need access to large global markets so they can amortize and recoup their costs across a single large global marketplace~\cite{ITIF}.
Each segment of the semiconductor value chain has, on average, 25 countries involved in the direct supply chain and 23 countries involved in support functions. Over 12 countries have enterprises directly engaged in semiconductor chip design, 39 countries have at least 1 semiconductor fabrication facility, while over 25 countries have enterprises engaging in ATP activities ~\cite{ITIF}. The typical production process toward a final electronics product can see the underlying semiconductors within it cross international borders 70 or more times in a process that takes over 100 days and includes 3 full trips around the world ~\cite{ITIF}. 
\\
\iffalse
Another set of companies, including Applied Materials (United States), ASML (the Netherlands), KLA Tencor (United States), and Lam Research (United States), manufacture the machines and tooling equipment that run semiconductor fabs. Finally, a number of enterprises, especially ones from Japan, South Korea, and Taiwan, manufacture chemicals and components essential to the semiconductor manufacturing process. For instance, fluorinated polyimides, a group of specialty polymers that provide physical strength and heat resistance, are produced by Daikin Chemical (Japan), DuPont (United States), Kaneka Asahi Kasei (Japan), and Taimide Technology (Taiwan). Photoresists are critical components that provide the patterns used to build micro-circuitry into semiconductors. The Japanese firms JSR Corporation, Shin-Etsu Chemical Company, Sumitomo Chemical, and Tokyo Ohka Kogyo Company manufacture photoresists, as do the Korean players Dongjin Semiconductor Company and Dongwoo Fine Chemicals. Portland, Oregon-based Inpria is the only U.S.-headquartered photoresists manufacturer, while European players have abandoned the field altogether~\cite{ITIF}\footnote{This paragraph may be better represented as a table of specialized companies integral to manufacturing semiconductors}.
\\
\fi

Uncertainties are not exclusive to just the supply of semiconductors - as semiconductors become increasingly pervasive and accessible to more diverse consumers, there is increasingly fluctuating demands from events like the pandemic, crypto\-currency booms and crashes etc, and also from increasingly stiff competition within the industry.
\\

All of these factors that make the semiconductor supply chain more complex lead to a bullwhip effect where there are increasing swings in inventory in response to shifts in consumer demand as one moves further up the supply chain ~\cite{bullwhip_src}. 
\\
\iffalse
Protectionist policies where governments funnel money. semiconductor companies cannot face excess, non-market-based competition, such as governments pumping in hundreds of billions of dollars in subsidies, which unfairly disadvantages enterprises that are attempting to compete on genuinely market-based terms~\cite{ITIF}. In other words, if leading-edge companies cannot be assured that they can earn a reasonable, risk-adjusted rate of return on their investments—which is put in doubt by some governments such as China investing massive amounts of money to create a domestic semiconductor industry—then the leading companies will cut R and D and capital expenditures~\cite{ITIF}. 


Table 3 shows a sampling of some unpredictable events and their financial
impact on the foundry. In most of the cases it's reasonable to assume that the
events caused a similar, if not more monetary loss to the chip companies that
purchased from these foundries. 
\fi

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[]
\small
\centering
\caption{\small Un-forcastable events, loss to foundry as result and time to recover}
\begin{tabular}{@{}llll@{}}
\toprule
Event                                                   & Loss to foundry   (\$)                          & How long to recover & When?      \\ \midrule
Power outage at TSMCs legacy process fab~\cite{t1}                & 28-35Mil   (30-40k wafers)                      & 12   hours          & Aug-21     \\
Texas winter storm froze Samsung foundry~\cite{t2}                & 286-357   Mil ($\sim$71k wafers)                & 1   month           & Apr-21     \\
Texas winter storm froze NXP foundry~\cite{t3}                    & $\sim$100   Mil                                 & 1   month           & Apr-21     \\
Fire at Renesas facility in Naka Japan~\cite{t4}                  & 171   Mill                                      & 1   month           & Mar-21     \\
\{Global Foundries quits on 7nm,   AMD shifts to tsmc\}~\cite{t5}~\cite{t6} & \{$\sim$4.255B loss just from AMD\}             & \{Permanent\}       & \{Aug-19\} \\
Current Chip shortage due to surge in demmand~\cite{t7}           & 60   Billion (what's the amount for foundries?) & 2+   years          & 2020       \\
China - US trade war causes TSMC to loose HWAWEI sales~\cite{t8}  & 13\%   of TSMCs revenue $\sim$= 455Mil          & 2   months          & 2020       \\
Fire at Asahi Kasei Foundry~\cite{t9}                             & 100Mil   \$** (unreliable source?               & ?                   & Feb-21     \\ \bottomrule
\end{tabular}
\end{table*}

\iffalse
From Table 1 it is clear that unpredictable events and delays can have a large
cost to foundries and especially for the companies whom the foundries supply.
This seems to be symptomatic of a larger problem with supply chain resiliency
in the semiconductor industry. As the ongoing chip shortage has brought to
light, semiconductor supply chains have several inherent weaknesses that make
them less resilient to supply fluctuations such as in the examples below, and
unforecasted customer demand spikes, as is currently occurring. Table 2
contains a comparison of various facets of good supply chains with those of
semiconductor supply chains:
\fi

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\tiny
\centering
\caption{\small Comparison of characteristics of resilient supply chains to Si supply chain}\footnote{update the table to include examples of industries that have the ideal supply chain characteristics}
\begin{tabular}{@{}ll@{}}
\toprule
Ideal Resilient Supply chain                                                                                                                                                                                                                                    & Semiconductor supply chain                                                                                                                                                                                                                              \\ \midrule
\begin{tabular}[c]{@{}l@{}}Multiple suppliers for the same product that aren't affected by similar \\ geographic or geopolitical conditions that can ramp up or slow down \\ production with linear cost scaling\end{tabular}                                   & \begin{tabular}[c]{@{}l@{}}Increasingly few fabs (suppliers) that are becoming more \\ geographically clustered; for high performance chips, \\ usually only one supplier.\end{tabular}                                                                 \\
Financially feasible to buffer stocks for demand spikes or supply drops                                                                                                                                                                                         & \begin{tabular}[c]{@{}l@{}}Buffering chips usually not financially feasible due to \\ cost and limited product lifespan of chips\end{tabular}                                                                                                           \\
\begin{tabular}[c]{@{}l@{}}Has intermediate components that can be sourced from different \\ suppliers are composed to create different final goods to adapt to\\  changing demand profiles or to maximize profits under high \\ demand situations\end{tabular} & \begin{tabular}[c]{@{}l@{}}Chiplet design which accomplishes a similar thing is \\ still new and not widely adopted. In current designs, \\ all or most of the chiplets in a package are manufactured\\  in the same foundry\end{tabular}               \\
\begin{tabular}[c]{@{}l@{}}Final produced goods are able to satisfy different demand streams \\ (like how a corn farmer satisfies demand for both corn-based food \\ and ethanol with his goods)\end{tabular}                                                   & \begin{tabular}[c]{@{}l@{}}Final produced good (chip) only satisfies one type of \\ demand stream.\end{tabular}                                                                                                                                         \\
\begin{tabular}[c]{@{}l@{}}Supply chain can quickly scale down or scale up production as \\ forecasts for demmand change\end{tabular}                                                                                                                           & \begin{tabular}[c]{@{}l@{}}Many foundries run at or close to full capacity, and takes \\ a 3-5 years to build a new foundry to increase supply. \\ Large lead time of 28-30 Weeks makes it hard to change \\ production levels either way.\end{tabular} \\ \bottomrule
\end{tabular}
\end{table}

These risk factors for the semiconductor supply chain are especially
concerning, because the factors for uncertainty in the semiconductor industry
are trending the wrong way. On the supply side, climate change is making fires,
and droughts like the recent one in Taiwan increasingly more common,
geopolitical tensions in the world are rising, and increasingly complex designs
and lithography techniques are steadily reducing the number of facilities that
can make cutting-edge chips. Demand for chips is also becoming more volatile as
computer chips begin to be utilized in more and more fields, with little
substitutability between fields (spike in demand in one field (eg. GPUs when
cryptocurrency values surge) cannot be full filled by slump or average demand
in another field.  

Improving supply chain resiliency for semiconductor chips has traditionally
been thought of as more of a logistics and planning/forecasting problem, but
computer architects can also play a role in improving supply chain resiliency
through creating novel architectures that allow remedial of specific risk
factors in the supply chain, as we try to show in this paper.\footnote{Will try
to find a more concrete example here of some company improving their supply
chain resilience through better product design}


==> newbackground.tex <==
\iffalse
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{./images/newfigures/newbackground01.png}
    \caption{Overview of a semiconductor supply chain.}
    \label{fig:back01}
\end{figure}
\fi

\iffalse
\subsection{How Semiconductor Supply Chains Work} 
Semiconductor supply chains (Figure~\ref{fig:back01}) are arguably one of the most complex in the world~\cite{khan2021semiconductor}. When a
modern chip design is ready to be manufactured, silicon is mined, refined for
extreme purity, and formed into a cylinder in a furnace, which is then cut
into wafers. Then, advanced lithography machines etch the design into the wafer
over dozens of layers. To etch a layer, a film of material such as an insulator,
or dopant that forms the basis of the permanent layer, is deposited. Then, a
coating of photoresist material that dissolves under light is selectively
dissolved according to a mask of the circuit design (called a photomask) using
a light from a photolithography machine. Then etching tools etch the pattern
into the permanent substrate below the photoresist. Then the photoresist is
removed, and the layer is flattened to allow the next layer to be
added. Each of the required materials in this
process– silicon or other semiconductors, materials and electronic gasses for
deposition, insulators, conductors, photoresist– has its own, sometimes complex
supply chain. The same applies to Silicon Manufacturing Equipment (SME)~\cite{sme} that
goes into this process, such as (silicon) crystal growing furnaces, equipment
for crystal machining, wafer handling, photomask handling and wafer marking,
lithography equipment, etching tools, ion implanters, deposition tools, and
process control tools to inspect the product along the different
stages.
%~\cite{khan2021semiconductor}.

The next step is Assembly, Testing and Packaging (ATP)~\cite{atmp}. The finished wafer is
cut (“diced”) into separate chips, tested for proper functionality, then
packaged (and again subsequently tested with a more complete battery of tests).
These stages also require extensive use of SMEs for dicing, bonding, packaging,
integrated assembly, and for testing various aspects of the final chip’s
functionality (Memory, SoC, Burn-in etc), as well as handlers and probers to
interface with the chip. Each of these components have their own supply chain.
After packaging, the chips are ready for use.

%Figure~\ref{fig:back01} shows an overview of the
%semiconductor supply chain: 
The complexity of the semiconductor supply chains already provides a hint of
of the vulnerability of these chains to disruptions.  We detail this vulnerability in the
next section.




\subsection{Characteristics and challenges
%of Semiconductor Supply
%Chains
}

%the complex supply chain detailed above, several additional
Several characteristics of the semiconductor supply chains, many borne out of the complexity of these chains, make the semiconductor supply chains highly vulnerable to supply and demand disruptions and 
make it hard to secure chip supplies to satisfy demand.
%industry create challenges in
%securing the supply chain. These are each considered in detail in the section
%below. 

%\subsubsection{Long Lead Times}
First, modern semiconductor supply chains are characterized by {\bf long lead times}. 
Each step in the manufacturing process is very time-consuming. For
example, it takes almost one day to form one of the several dozens of layers of
the chip, a week to manufacture a photomask, and two to three weeks to test the
chip after it is manufactured. Additionally, facilities that perform various
steps of the manufacturing process may be located in different parts of the
world, adding time to travel between
facilities~\cite{monch2018survey}~\cite{beyond} . All said, a typical
semiconductor lead time is in the order of 2-4 months\cite{levadata}, which is
especially large considering the typical 18-month life cycle of a product. The
long lead times make it difficult for the semiconductor chain to quickly react
to disruptions in demand.
%, necessitating further approaches to enable the chain
%to be more reactive. 

%\subsubsection{Economies of Scale}
Semiconductor supply chains also operate under the stringent constraints of the {\bf economy of scale}.
The non-recurring expenses (NRE) that must be expended to design and
manufacture a semiconductor is extremely high and increasing due to several
factors. Firstly, it requires a lot more expertise to build a chip – studies
estimate that the number of researchers required to achieve Moore’s Law (i.e.,
doubling of computer chip density) today is more than 18 times larger than the
number required in the early 1970s~\cite{ideas}. Secondly, building
manufacturing plants for cutting edge processes that require complex SME is
very expensive – as of 2020 it was estimated that a new 10 nm fab costs \$15
billion to build, a 7 nm fab \$18 billion and a 5 nm fab \$20
billion~\cite{state}. 
%However, an individual chip comes off the production line
%at an incremental cost~\cite{ITIF}. 
Because of this, semiconductor companies
need to either sell at very high volumes or at high markups over the
incremental manufacturing costs to recoup their NRE. An industry downturn (i.e., reduced demand) can frequently lead to losses.
This is exacerbated by continuing need to expend the high NRE to maintain
the skilled workforce and equipment to continue innovation. 

%\subsubsection{Short Product Life Cycles}
Semiconductor supply chains are also characterized by {\bf short product life cycles}.
Due to the competitive nature of the semiconductor industry - the typical
product life cycle is about 18 months, which is relatively short compared to
other industries~\cite{markov06}. To add to this, semiconductor prices often
decline over their life cycles. These two factors make it less feasible to
stockpile finished chips to use as a buffer in case of supply or demand shocks
- necessitating other measures to improve resilience.
%- and lead to varying
%demand levels over the lifecycle of the product~\cite{}.

%\subsection{Global Nature of the Industry}
Semiconductor supply chains also characterized by their {\bf global nature}.
Semiconductors have a very low volume (and weight) to value ratio, and so the
cost of moving them across the globe is small relative to their actual value.
This has encouraged companies to disperse the semiconductor value chain across
the globe to play to strengths of different regions, such as availability of
cheap or highly skilled labor, low taxes, availability of raw materials
etc~\cite{beyond}.  
In fact,
no major country has capabilities in
all parts of the semiconductor value chain~\cite{} and some steps in the chain are exclusively owned by one or a few countries~\cite{}. 
%When diving further into the
%composing segments, the extent of geographic dispersion can be even more stark
%For example, ASML in Netherlands is the only manufacturer of advanced EUV
%lithography machines~\cite{khan2021semiconductor}, Japan holds 90\% of the market of photoresists~\cite{factbox}, the
%United States is the sole producer of wafer marking systems and electrical
%instruments for wafer inspection~\cite{khan2021semiconductor}. 
This geographic dispersion and the dominance of certain
firms/regions in certain sectors of manufacturing can mean that adverse events
in any country involved in the value chain are felt through the full supply
chain.
%, highlighting the sheer number of possibilities for disruptions in the
%supply and demand of chips. 
This global
nature also makes the semiconductor industry subject to geopolitical tensions~\cite{t11, t12}.


\iffalse
The table below shows which regions of the world specialize
in what parts of the semiconductor value chain:

\begin{table}[]
\tiny
\begin{tabular}{|cc|ccccccc|}
\hline
\multicolumn{1}{|c|}{}          & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Segment \\ Value add\end{tabular}} & \multicolumn{7}{c|}{Market shares}                                                                                                                                                                             \\ \cline{1-1} \cline{3-9} 
\multicolumn{1}{|c|}{}          &                                                                                  & \multicolumn{1}{c|}{U.S.} & \multicolumn{1}{c|}{S. Korea}       & \multicolumn{1}{c|}{Japan} & \multicolumn{1}{c|}{Taiwan}         & \multicolumn{1}{c|}{Europe} & \multicolumn{1}{c|}{China}          & Other \\ \hline
\multicolumn{1}{|c|}{EDA}       & 1.5\%                                                                            & \multicolumn{1}{c|}{96\%} & \multicolumn{1}{c|}{\textless{}1\%} & \multicolumn{1}{c|}{3\%}   & \multicolumn{1}{c|}{0\%}            & \multicolumn{1}{c|}{0\%}    & \multicolumn{1}{c|}{\textless{}1\%} & 0\%   \\ \hline
\multicolumn{1}{|c|}{Core IP}   & 0.9\%                                                                            & \multicolumn{1}{c|}{52\%} & \multicolumn{1}{c|}{0\%}            & \multicolumn{1}{c|}{0\%}   & \multicolumn{1}{c|}{1\%}            & \multicolumn{1}{c|}{43\%}   & \multicolumn{1}{c|}{2\%}            & 2\%   \\ \hline
\multicolumn{1}{|c|}{Wafers}    & 2.9\%                                                                            & \multicolumn{1}{c|}{0\%}  & \multicolumn{1}{c|}{10\%}           & \multicolumn{1}{c|}{56\%}  & \multicolumn{1}{c|}{16\%}           & \multicolumn{1}{c|}{14\%}   & \multicolumn{1}{c|}{4\%}            & 0\%   \\ \hline
\multicolumn{1}{|c|}{Fab Tools} & 14.9\%                                                                           & \multicolumn{1}{c|}{44\%} & \multicolumn{1}{c|}{2\%}            & \multicolumn{1}{c|}{29\%}  & \multicolumn{1}{c|}{\textless{}1\%} & \multicolumn{1}{c|}{23\%}   & \multicolumn{1}{c|}{1\%}            & 1\%   \\ \hline
\multicolumn{1}{|c|}{ATP Tools} & 2.4\%                                                                            & \multicolumn{1}{c|}{23\%} & \multicolumn{1}{c|}{9\%}            & \multicolumn{1}{c|}{44\%}  & \multicolumn{1}{c|}{3\%}            & \multicolumn{1}{c|}{6\%}    & \multicolumn{1}{c|}{9\%}            & 7\%   \\ \hline
\multicolumn{1}{|c|}{Design}    & 29.8\%                                                                           & \multicolumn{1}{c|}{47\%} & \multicolumn{1}{c|}{19\%}           & \multicolumn{1}{c|}{10\%}  & \multicolumn{1}{c|}{6\%}            & \multicolumn{1}{c|}{10\%}   & \multicolumn{1}{c|}{5\%}            & 3\%   \\ \hline
\multicolumn{1}{|c|}{Fab}       & 38.4\%                                                                           & \multicolumn{1}{c|}{33\%} & \multicolumn{1}{c|}{22\%}           & \multicolumn{1}{c|}{10\%}  & \multicolumn{1}{c|}{19\%}           & \multicolumn{1}{c|}{8\%}    & \multicolumn{1}{c|}{7\%}            & 1\%   \\ \hline
\multicolumn{1}{|c|}{ATP}       & 9.6\%                                                                            & \multicolumn{1}{c|}{28\%} & \multicolumn{1}{c|}{13\%}           & \multicolumn{1}{c|}{7\%}   & \multicolumn{1}{c|}{29\%}           & \multicolumn{1}{c|}{5\%}    & \multicolumn{1}{c|}{14\%}           & 4\%   \\ \hline
\multicolumn{2}{|c|}{Total value add}                                                                              & \multicolumn{1}{c|}{39\%} & \multicolumn{1}{c|}{16\%}           & \multicolumn{1}{c|}{14\%}  & \multicolumn{1}{c|}{12\%}           & \multicolumn{1}{c|}{11\%}   & \multicolumn{1}{c|}{6\%}            & 2\%   \\ \hline
\end{tabular}
\end{table}

From the data here, it can be seen that
\fi


\iffalse
As an example to illustrate the global nature
of the industry, let us consider Intel. Intel has 24 wafer fabs in 6 countries
around the world and its supply chain comprises more than 11,000 suppliers in
over 90 countries~\cite{intel}.   For example, the current situation in
Russia/Ukraine has affected the supply of critical materials in semiconductor
manufacturing like neon gas (used in the lasers in lithography machines), which
has nearly half its global supply coming from Ukraine~\cite{majeed}, and palladium (used in
chip packaging, sensors and memory), 35\% of which comes from Russia. As a
result, semiconductor lead times are projected to remain high.  
For example, a Dutch ban on exports of EUV scanners to China already prevents
it from building capacity more advanced than 7 nm~\cite{trump}. 

Differing monetary policies between the various countries where semiconductor
industries are concentrated are situated are a source of uncertainty. For
example, protectionist policies where governments funnel money. semiconductor
companies cannot face excess, non-market-based competition, such as governments
pumping in hundreds of billions of dollars in subsidies, which unfairly
disadvantages enterprises that are attempting to compete on genuinely
market-based terms~\cite{ITIF}. In other words, if leading-edge companies
cannot be assured that they can earn a reasonable, risk-adjusted rate of return
on their investments—which is put in doubt by some governments such as China
investing massive amounts of money to create a domestic semiconductor
industry—then the leading companies may be forced to cut R and D and capital
expenditures~\cite{ITIF}. 
%This is potentially worded in a controversial way- may need to reword/remove. 


There are also uncertainties in the supply of chips from fabrication plants
from natural events like draughts, fires and winter storms that could become
more common with global warming, and geopolitical conflicts that are becoming
more common in areas where semiconductor fabs are concentrated, like the
US-China trade war~\cite{t11} or tensions over Taiwan~\cite{t12}. 
\fi
 
%\subsection{Uncertain Demand}
 
Uncertainties in the semiconductor supply chains
(Figure~\ref{fig:SC_uncertainities}) are not exclusive to just the supply of
semiconductors - as semiconductors become increasingly pervasive and accessible
to more diverse consumers, there is increasingly {\bf fluctuating demand} from
events like the pandemic, crypto\-currency booms and crashes etc., and also from
increasingly stiff competition within the industry.
  
  
Also, because the semiconductor supply chain is so long, it is also susceptible
to the {\bf bullwhip effect}, where there are increasing swings in inventory in
response to shifts in consumer demand as one moves further up the supply chain
~\cite{bullwhip_src}. This increases uncertainties in the supply chain further.

\begin{figure}
    \centering
    %\includegraphics[width=6cm]{./images/newfigures/Uncertainity_in_semi_chain.png}
    \includegraphics[width=\linewidth]{./images/newfigures/newuncern.png}
    \caption{Example sources of uncertainty in a semiconductor supply chain}
    \label{fig:SC_uncertainities}
\end{figure}

\iffalse
%\subsection{Growing risk factors}
The risk factors for the semiconductor supply chain are especially
concerning since they
are trending the wrong way. On the supply side, climate change is making fires,
and droughts like the recent one in Taiwan increasingly more common,
geopolitical tensions in the world are rising, and increasingly complex designs
and lithography techniques are steadily reducing the number of facilities that
can make cutting-edge chips. Demand for chips is also becoming more volatile as
computer chips begin to be utilized in more and more fields, with little
substitutability between fields (spike in demand in one field (eg. GPUs when
cryptocurrency values surge) cannot be full filled by slump or average demand
in another field.
\fi
 

\subsection{Prior Work} 
\fi
\iffalse
Given these challenges in the semiconductor supply chain, there is an impetus
to make semiconductor supply chains more resilient and robust. This subsection
will delve into the existing work on supply chain resilience - specific to
semiconductors and in the general sense- and explain how this paper differs
from them.  
\fi

There is a large body of work on supply chain resilience~\cite{tukamuhabwa2015supply,ponomarov2009understanding,pereira2014achieving}.
\iffalse
Tukamuhabwa {\em et al.}~\cite{supply15} define supply chain resilience (SCRES) as "The
adaptive capability of a supply chain to prepare for and/or respond to
disruptions, to make a timely and cost-effective recovery, and therefore
progress to a post-disruption state of operations – ideally, a better state
than prior to the disruption". This definition implies that a
resilient supply chain would be prepared for a disruptive event (be it external
or due to the inherent nature of the supply chain), respond effectively to the
event and recover quickly from it, and be able to attain growth or a
competitive advantage after it – all in a cost-effective manner. The most
recognized way of assessing a system’s resilience is the Resilience triangle,
which considers factors like performance level loss estimation and recovery
time~\cite{framework01,framework02,framework03}.  Most of the
work on supply chain resilience focuses on strategies for achieving SCRES.
\fi
The strategies for supply chain resilience
proposed by these works fall into one of four general categories - improving flexibility, creating redundancy, enhancing agility, and improving supply chain collaboration~\cite{supply15}.
Flexibility is the ability of an enterprise to adapt to changing
requirements with minimum time and effort~\cite{framework10}.  Creating
redundancy involves spare capacity and inventory that can be invoked
during a crisis to cope with supply shortages or demand
surges~\cite{supply03}. Supply chain collaboration refers to the ability to
work effectively with other entities (in the supply chain) for mutual benefit
in areas such as forecasting, postponement, and risk sharing~\cite{s27}.  Supply
chain agility is the ability to respond quickly to unpredictable changes in
demand or supply~\cite{supply03}, including visibility (through the
entire supply chain) and velocity (speed of recovering from the disruption).

There has also been work on making semiconductor supply chains
resilient~\cite{coping22,fu2019unison,adobor2018supply,monch2018survey,khan2021semiconductor}. A body of research~\cite{vertical12,tang2006robust} looks into
decisions on what components to make in-house, what components to
outsource, and optimal partner selection.  Strategic network planning for
semiconductor supply chains~\cite{monch2018survey} is yet another topic of
research, focused on determining what facilities
should be built, what equipment should be purchased, what productions should be
made in what facilities, and what portion of demand should be outsourced and
what left unmet. 
%This has been done with the help of
%Mixed Integer Programs (MIPs) contained in a Manufacturing Execution Model
%(MEM) decision support system~\cite{stray06}, and %more advanced methods like
%adding stochastic MIP models with recourse~\cite{supply11}.  
There is further work on coordinating semiconductor supply chains~\cite{datta2011information} for
improved resilience and efficiency.
%i.e.  ensuring that total profit
%earned by all its agents equals what they would earn if administered as a
%single entity, by designing contracts appropriately.
There has also been work
on simulating semiconductor supply chains to evaluate policies for
production and inventory control~\cite{discrete05} to improve resilience.
\iffalse
A body
of research~\cite{james2021optimization,can2008postponement} is devoted to optimizing the Customer Order Decoupling Point (CODP) -
the point in the supply chain where material is committed to a specific
customer order and cannot be used for another, and points after this cannot
make use of stockpiling to improve resilience~\cite{monch2018survey}. 
\fi

The above works mostly target business and process optimizations.  As far as we know, there has been no work that considers the role of chip
architects in supply chain resilience.

\iffalse
However, a common thread
in most of the existing work on semiconductor supply chains is that the main
aim of research is to find ways to optimize the supply chain to generate more
profit while making the same ultimate product. There are few works focused on
applying the principles to improve resiliency -Flexibility, Creating
Redundancy, Supply Chain collaboration and Supply chain agility - into the
semiconductor supply chain, and analysis on the potential benefits of changing
the characteristics of the produced chip to improve supply resilience. 


Work
done by Begen {\em et al.} (2016) explores the effect of uncertainty in supply and
demand and the effects and benefits of reducing them using a modified
newspaper vendor model, but is not tailored to any industry in
particular~\cite{supply16}.  Work done by Jian {\em et al.} (2021)~\cite{coping12}
explores the concept of adapting semiconductor chips to lower functions when
there is uncertain supply of chips in the context of the auto industry using
max-min robust optimization approach, but this work exclusively considers the
semiconductor industry in isolation, and goes further in several aspects.  This
work considers disruptions to both supply and demands and variations of
different stages in the process where these uncertainties are resolved. We also
consider two additional tactics to improve resiliency through changing the
nature of the product – composition and dispersion - and compare their relative
efficacies under different scenarios of disruptions to supply and demand. 
\fi


==> newbackground_swamy.tex <==
Significant prior work exists in improving resilience to volatile supply/demand in \cite{} [35], [30], [28]. The strategies for resilience proposed by these works fall into one of four general categories - improving flexibility, creating redundancy, enhancing agility, and improving supply chain collaboration \cite{}[36]. Similar work also exists for semiconductors ~\cite{coping22,fu2019unison,adobor2018supply,monch2018survey,khan2021semiconductor}. A body of research~\cite{vertical12,tang2006robust} looks into decisions on what components to make in-house, what components to outsource, optimal partner selection, strategic network planning~\cite{monch2018survey}, coordinating semiconductor supply chains~\cite{datta2011information} and simulating semiconductor supply chains~\cite{discrete05} to improve resilience. The above works almost exclusively target business and process optimizations, not the actual product (chip) itself.

Existing works do generically explore the relationship between products and their supply chains. This paradigm of thinking was first proposed by Fisher~\cite{SC_right_for_product} and later extended by Lee et al.~\cite{Allign_SC_strat_Prod_Unc}. Additionally, analysis by done by Cohen et al.~\cite{Bespoke_SC_resilience} shows that for high performance chips, resilience is in fact bottlenecked by the product. Yet there has been little work done on modifying semiconductor chips within the constraints of current supply chains and (demand) markets to improve resilience. The only such example we could find was work done by Jian et al.~\cite{coping12} that explores the concept of altering semiconductor chips used in the auto industry to lower functions when there is uncertain supply of chips using a max-min robust optimization approach. This work significantly differs in several ways. It exclusively considers the semiconductor industry (specifically high-performance chips) in isolation, and goes further in several aspects. This work considers disruptions to both supply and demands and variations of different stages in the process where these uncertainties are resolved. Additionally, we consider architecturally- realizable strategies to improve resiliency in a range of market scenarios - a first, as far as we can tell.

==> newinterventions.tex <==
%\nathan{
\iffalse While the uncertainties in the semiconductor supply chains are varied
(Figure~\ref{fig:SC_uncertainities} and are often beyond control, the impact of
these uncertainties can be managed.  \fi 
\iffalse
We observe that fragility in
semiconductor supply chains (i.e., high impact on cost from supply and demand
uncertainties) is due, in part, to the frequent one-to-one correspondence
between chips produced and the chips demanded (i.e., a given produced chip only
satisfies a given demand), which, in turn, leads to
single path to satisfy chip demands. Any fluctuations in supply or demand then
can directly lead to shortages or overages leading to increased costs.    {\em
Chip architects can enable multiple paths to satisfy a chip demand, which is
the key to supply chain resilience}. 
\fi
\iffalse
Multiple paths can be enabled, for example, by decoupling produced chips from
demanded chips in such a way that chip demands can still be met using an
appropriate subset of produced chips. Newer paths can also be enabled by choice
of architecture and implementation technology that allows chips to be produced
by multiple suppliers.
%confirming their acceptability through an an analysis of the impact of these
%paths on architecture-level metrics.


The improved semiconductor supply chain resilience from enabling multiple paths
to satisfy a chip demand can be understood easily in terms of network
reliability theory~\cite{blank}.  Network reliability improves when there are
multiple paths from a source to terminal node (Figure~\ref{fig:}) - when chip
architects create multiple such paths, the cost of uncertainties is lessened. 
%}
\fi

\iffalse
There are several things that can potentially  be done to reduce the effect of
supply and demand disruptions in the semiconductor industry such as 
\begin{itemize}
    \item Doing software optimizations to gain performance, reducing the need
        to procure new, more advanced chips that may be experiencing supply
        shortages. 
    \item Designing platforms for compatible replacement chips that can be used
        when availability of the principal chip is limited.
        lead to increased resilience.
    \item Reduce the function/features of the chip, or relax the demand
        requirement to ease supply constraints.
\end{itemize}
This and similar classes of methods that jeopardize profit for the chip
manufacturer (such as by making it sell less advanced chips), or don’t require
computer architects’ intervention will not be considered in this paper. Rather,
this paper focuses on interventions requiring computer architects that don’t
significantly affect a chip firm’s profits. These include composition,
adaptation and dispersion, and are discussed in further detail below.    
\fi

We focus on three classes of techniques chip architects can use to increase the number of paths to satisfying chip demand.


\subsection{Composition}
In composition, final goods are produced by combining several input components
to make the final saleable product, such as through the use of chiplets that
can be interconnected using an interposer to make a larger chip, use of
multiple IPs to create an SoC, or use of multiple chips within a
Multi-Chip-Module (MCM). Mathematically, composition can be viewed as a
many-to-one relation between input components and a saleable product, where
input components may be present in more than one composition relation.
Figure~\ref{fig:composition_graph} depicts composition: note how input
component (IC) IC3 is used to build saleable products that satisfy
{\bf both} demand requirements D1 and D2. Composition is already widely used in industry~\cite{li2020chiplet,amdnext}, because of yield and cost benefits. Yet, supply chain
resilience benefits of composition have not been studied in any detail.

% \[
%     M \subset \bigcup_{i=1}^\infty PG^i\times DG
% \]

% \begin{figure}[ht]
%     \centering
%     %\includegraphics[width=.3\linewidth]{./images/newfigures/Composition Diagram.png}
%     \includegraphics[width=0.4\linewidth]{./images/composition.png}
%     \caption[skip=0pt]{Composition is a many-to-one relation, in which multiple produced
%     chips are combined to produce a single demanded chip.}
%     \label{fig:composition_graph}
% \end{figure}
\begin{figure}[ht]
    \captionsetup[subfloat]{farskip=0pt,captionskip=-1pt,nearskip=-8pt}
    \centering
    \subfloat[\centering \small Composition is a many-to-one relation]{
        {\includegraphics[width=0.3\linewidth]{./images/composition.png}}
        \label{fig:composition_graph}
    }
    \subfloat[\centering \small Composition mitigates risks associated with market
    uncertainty]{
        {\includegraphics[width=0.3\linewidth]{./images/composition2.png}}
        \label{fig:composition_graph2}
    }
    \caption{\small Composition Mappings}
    \label{fig:composition_graphs}
\end{figure}
Composition can enable supply chain resilience in a number of ways.  First,
the disaggregation of large, complex chips into multiple smaller chips
increases yield which, in turn, mitigates the effects of
supply constraints.  
%This is a well known property of disaggregation, and
%is a major reason for the success of chiplet based design~\cite{blank}.
Second, composition can enable \textit{multiple} paths to the same produced
good.  For example, a 16-core processor demand can be satisfied with a
monolithic 16-core chip, or several combinations of 8-core and 4-core
chiplets. This redundancy allows an alternate path when supply along
a particular path is constrained.  Composition also enhances agility, the
ability to respond quickly to supply disruptions by allowing the deferral of
decisions of how to satisfy chip demands.
%affecting the makeup of saleable goods finally produced. 
%Thus composition gives
%firms partial redressal capabilities when there is fuller realization of
%potential supply and disruptions. 
%Supply disruptions are largely known at the
%time decisions about composition will be made, because the supply of input
%components will be fully realized, and demand disruptions are better known
%because it is closer to the time the chip is actually sold (and when demand is
%fully realized). 
Figure~\ref{fig:composition_graph2} illustrates 
the agility benefits of composition.
%a potential
%exploitation of composition to benefit from this phenomenon. 
Demand D1 and D2
are fulfilled using two IC1 chiplets and four IC1 chiplets respectively.
%chips made from 2 input chiplets IC1 and 4 input chiplets
%IC4 respectively, and D2 has a higher per-unit profit for the firm. 
If there is
an unforecasted spike in demand for D2, the firm can decide to go from dedicating half of the
produced IC1s to building chips for D2 to dedicating 75\% of produced IC1s to
D2, with a much quicker turnaround time than if the firm were
satisfying D1 and D2 with separate monolithic chips.
%Similarly, when the firm’s
%supply of input chips is affected, then it can shift to manufacturing more of
%the higher margin chips to limit its losses. 
Finally, composition also enables {\em dispersion}, (see
Section~\ref{ssec:dispersion}).

% \begin{figure}
%     \centering
%     \includegraphics[width=0.6\linewidth]{./images/composition2.png}
%     \caption{Composing two different demand chips from the same produced chip
%     helps mitigate risks associated with market uncertainty.}
%     \label{fig:composition_graph2}
% \end{figure}

\iffalse
Composition can also enhance the flexibility of the supply chain, or its
ability to adapt to changing requirements with minimum time and effort, because
the final product is \st{fragmentized} \nathan{disaggregated}. For example, if a
customer wants additional security features on their processor, it may require
less time and effort to meet this requirement by designing a ‘security chiplet’
that is composed with the existing components of the chip, as opposed to
designing and integrating the requisite logic within an existing die. Analysis
of this aspect of composition’s benefit is outside the scope of the proposed
model, and thus will not be discussed further. The final benefit of composition
to the supply chain is it allows for gradated redundancy, through allowing the
firm to forgo redundancy for only certain parts of the chip to meet demand
requirements. Concretely, this may mean that a firm can design a chip with
performance-limiting logic (such as the core and cache) on a leading edge node
that lacks redundancy, while implementing the rest of the logic for the chip,
such as the I/O and memory controller on a trailing edge node that has more
redundancy because more fabs are capable of manufacturing it. 


%The technique of

%it results in lower area in individual chiplets (which
%improves yield) as well as allowing for the feasibility of 
as well as for building chips larger than what a
monolithic die would allow due to reticle limits~\cite{blank}.
However, the supply composition is being leveraged to improve the
resilience of such products.  

%These additional benefits and the maturity of the
%technique make composition a potentially attractive technique to bolster
%resilience if it proves effective. 



%\nathan{
Architectural techniques to promote composition extend beyond disaggregation
and chiplet based architectures.  Composition can also be exploited in a SoC design,
where composable IPs can be stitched together using standardized interfaces
to a system NoC, or a multi-chip module design where multiple chips are integrated in the same package.
%.  Other forms of composition can also occur at the package level
%via 3D integration techniques which use through-silicon vias,
%or by using wireless communications to transmit data %between chips.
%}
\fi




\subsection{Adaptation}
\iffalse
\begin{itemize}
    \item What Adaptation is – theoretically, concretely and mathematically. 
    \item How it can theoretically be of use
    \begin{itemize}
        \item Agility
        \item Potential for flexibility ???
    \end{itemize}
    \item How it is being done now, how it can be taken further. 
\end{itemize}
\fi

In adaptation, a single input good (e.g., chips) is designed to meet the requirements of several demanded goods (through the use of binning~\cite{binning}, rebadging~\cite{rebadge01,rebadge02}, reprogramming~\cite{reprog}, etc., as well as non-conventional architectures such as multi-ISA designs and consolidated designs - see Section~\ref{sec:adapt_tech}). 
%How this may be
%implemented in the real world is discussed later in this subsection.
Mathematically, adaptation may be viewed as a one-to-many relation between a
saleable product and multiple demand requirements.
Figure~\ref{fig:adaptation_graph} depicts adaptation.


% \begin{figure}
%     \centering
%     %\includegraphics[width=0.3\linewidth]{./images//Adaptation Diagram.png}
%     \includegraphics[width=0.3\linewidth]{./images/adaptation1.png}
%     \caption{Adaptation is a one-to-many relation, in which a single produced
%     chip is able to satisfy requirements for multiple demanded chips.}
%     \label{fig:adaptation_graph}
% \end{figure}
\begin{figure}[ht]
    \captionsetup[subfloat]{farskip=0pt,captionskip=-1pt,nearskip=-8pt}
    \centering
    \subfloat[\centering \small Adaptation is a one-to-many relation]{
        {\includegraphics[width=0.3\linewidth]{./images/adaptation1.png}}
        \label{fig:adaptation_graph}
    }
    \subfloat[\centering \small Adaptation can create alternate paths to the
    same demand]{
        {\includegraphics[width=0.3\linewidth]{./images/adaptation2}}
        \label{fig:ada-multi-path}
    }
    \caption{Adaptation Mappings}
    \label{fig:adaptation-mappings}
\end{figure}
%\subsubsection{Agility}

Adaptation improves supply chain resilience in different ways. First, similar to composition, adaptation allows deferral of decisions about the  type of
demand a chip will need to satisfy to later in the
supply chain, where there is greater clarity about potential
disturbances to supply and demand. This, in turn, can improve the speed with
which the firm can respond to these disturbances. For example, if a firm
produces an  input component IC1-based saleable product  which primarily satisfies demand D1, but can be adapted to also satisfy higher profit margin demand D2 (Figure~\ref{fig:adaptation_graph}), and there is a spike in
demand for D2, the firm can adapt a higher proportion of the IC1 it produces to
satisfying D2.
%, and simultaneously sell SP1 to meet D1 at a higher profit in a
%relatively short time frame relative to the lead time of producing SP1. 
Adaptation also creates alternate supply paths for conventionally produced
goods (i.e., ones whose demand is primarily satisfied without adaption). In
Figure~\ref{fig:ada-multi-path}, input component IC1-based saleable product is produced
conventionally, and it is the most profitable way to satisfy D1. IC2-based saleable product, which is
adaptable and principally satisfies D2, can also be adapted to satisfy D1. In
this scenario, there are multiple paths to meeting demand D1, which can improve
the redundancy and, therefore, the resilience of the supply chain. 

Composition and adaptation are already popular techniques both in research and
practice~\cite{tadayon2020moore,venkat2014harnessing,chiplet,amdnext,binning,rebadge01,reprog}.
However, conventionally, their focus has been different.
%Conventionally, composition, for example, is focused on minimizing cost by maximizing disaggregation~\cite{}; we focus on enabling multiple paths for supply chain resilience.
%Chip designers currently use several of the interventions discussed above.
For example, AMD's 4th generation Zen 3 chips are built out of  combinations of
Chip Complex Dies (CCD) and I/O Dies chiplets to minimize cost through
disaggregation. The various Zen 3 Ryzen models are differentiated by the number
of CCDs (e.g., 2x CCDs in Ryzen 9 series vs 1x CCD in Ryzen 7 series), and the
number and $f_{max}$ of (active) cores per CCD - this
%. The different number and type of compute chiplets on different models 
enables effective performance binning.
%based on performance and correctness, and also enables \textit{rebadging} based
%on market factors. 
Similarly, rebranding is prevalent in the GPU sector, in which the same chip is
used in multiple systems 
%(e.g., different coolers, different IO ports, etc.)
(e.g., Radeon R7 265 vs Radeon HD 7850, GeForce 8800 GT vs GeForce 9800 GT), to
minimize cost.
%Thus, industry already performs composition (as dissagregation), and adaptation
%(as binning/rebadging) for different reasons.  However, 
Our focus is different - we intend to optimize for supply chain resilience which
leads to very different choices. We show in Section~\ref{sec:results}, for
example, that supply chain resilience in case of composition is not maximized by
the most disaggregated architecture; a less disaggregated architecture or a
collection of architectures of different amounts of disaggregation are often
more cost-effective in presence of supply chain uncertainties. 

%and adaptation can
%be used to increase supply chain resilience by creating \textit{multiple paths}
%to the same demand good; 

\iffalse
\subsubsection{Flexibility} 
\st{
Adaptation may offer limited efficacy in improving the flexibility of a supply
chain to changing requirements. A potential way adaptation can make the supply
chain more flexible is when the demand requirements change in a way that the
existing adaptability capabilities of the produced saleable product are
sufficient to adapt said saleable product to meet the new demand requirement. 
}
\nathan{
Adaptation allows vendors to `flex' produced goods to meet changing market
demands.  As a market evolves, the quantities of goods demanded by the market
change, and adaptation reduces risks associated with inaccurate demand
forecasting through this flexibility.  This is especially relevant in markets
where demand for goods are negatively correlated, as then excess demand
for one good can be made up with the adapted supply that, by forecast, would
have satisfied the correlated demand good.
}


\subsection{Redundancy}
While adaptation does not inherently create redundancy, it can be utilized to
create it, by 
\fi


% \begin{figure}
%     \centering
%     %\includegraphics[width=0.3\linewidth]{./images/newfigures/Adaptation_redundancy.png}
%     \includegraphics[width=0.3\linewidth]{./images/adaptation2.png}
%     \caption{Adaptation can create alternate paths to satisfying the same demand.}
%     \label{fig:ada-multi-path}
% \end{figure}

\iffalse
There are several ways adaptation can be manifested with semiconductors, few of
which are already in use today. Adaptation can be achieved through binning.
Binning is the process of categorizing the hardware components by their quality
and performance. Architects can also use voltage/frequency scaling (VFS) to
design adaptable hardware. Demanded hardware may have varying performance and
energy efficiency requirements based on the workloads that its supposed to
target. Architects can use voltage/frequency scaling (VFS) techniques to adapt
the supplied hardware according to the performance and energy efficiency
requirements of the demand hardware\cite{}. % Original citation was '[12]'
Refreshing or rebranding chips can 
also be considered a form of adaptation. More advanced architectural methods to
achieve adaptability are through incorporating programmable hardware to adapt
hardware to different applications, or multiple ISA chips. 
\fi

\subsection{Dispersion}
\label{ssec:dispersion}
In dispersion, a chip is designed in such a way that
allows for sourcing from more than one independent supplier (e.g., foundries)
of the entire saleable product, or of one or more of the input components
(e.g., chiplets) that can be composed to make the final saleable product.
Figure~\ref{fig:dispersion-multip-path} illustrates dispersion. IC1 is identified as a component that can come from either supplier S1 or supplier S2. 

 \begin{figure}
     \centering
     %\includegraphics[width=0.3\linewidth]{./images/newfigures/Dispersion.png}
     \includegraphics[width=0.3\linewidth]{./images/dispersion1.png}
     \caption{Architectures designed for dispersion allow for some or all of a chip's components to be sourced from multiple independent suppliers.}
     \label{fig:dispersion-multip-path}
 \end{figure}


Dispersion can improve the redundancy of the supply chain. When there are
multiple independent suppliers, disruptions to one supplier do not affect the
other supplier, and so the firm still has a supply of the commodity, albeit at
a potentially lower production rate. This redundancy improves the resilience of
the supply chain. Dispersion can be achieved by making parts of the chip with
low performance sensitivity in a trailing edge process node that more fabs
support. For example, as multiple foundries exist at legacy technodes,
microcontrollers and other low-cost ICs are ideal candidates to use dispersion
to mitigate supply chain risks. Alternatively, architectures can employ
commodity hard and soft IPs or hardware components that may have multiple
suppliers. Some of these IPs may be implemented as chiplets (so the dispersible architecture is a composition of chiplets some of which are sourced by multiple suppliers). 

%and/or by designing
%memory heavy demand architectures that utilize memory and flash chips that are
%highly commoditized.
%\nathan{

%}




\iffalse
We also recommend architects consider adaptation via multi-isa designs.  We
argue this is appealing in the microcontroller space, where various competing
RISC architectures have strong similarities, reducing multi-isa support overhead.
Apple's M1 ARMv8.5-A processor was designed with backwards compatibility with
x86 in mind.  To support this, legacy x86 code is translated into ARM code
using Rosetta 2 software~\cite{prj_champ_rosetta2}.
When executing this translated code, the M1 is toggled to enforce the stronger
TSO memory model of the x86~\cite{rocha2022lasagne}. That is, the M1 provides hardware support
for both x86 and ARMv8.5-A memory models.
We are unaware of any industrial use of dispersion. It is concievable that
chips with significant demand will disperse production across multiple foundries,
however, we are unaware of industrial use of multi-technology dispersion in
efforts to increase supply chain resilience.
For these reasons, our baselines for composition use maximal ammounts of
disaggregation, and our baselines mappings for adaptation use only
chips with exactly the demanded core-count). 
The yield model used is slightly na\"ive.  When a chip fails to yield, it is
rendered as junk, and cannot be binned down to a lower core count.  However,
this na\"ivete affects both baseline results and results with interventions.

\fi

\iffalse
%\nathan{
The usefullness of both dispersion and adaptation may be impacted by correlations
between supply and demand uncertainties.  For example, given a \textit{global}
chip shortage, dispersion may become especially effective, as dispersion enables
procuring chips from multiple foundries, potentially decreasing time to market,
and increasing overall supply.
Adaptation is especially useful when the demands for two adaptable goods
is negatively correlated, as supply overages in the less demanded good may
be used to cover supply shortages in the more demanded good.
On the other hand, positive correlations between
demands for adaptable goods may limit the usefullness of adaptation, as there
is a high liklihood for either simultaneous overages or shortages of both
produced goods.
%}
\fi

\iffalse
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{./images/newfigures/SCRES_strategies.png}
    \caption{Summary of Benefits of each intervention}
    \label{fig:SCRES_strat}
\end{figure}
\fi


==> newintro.tex <==
% The semiconductor industry is becoming increasingly complex and uncertain due
% to a variety of factors. More complex designs may not perform to expectations
% or have other issues that delay their production. Cutting edge technology
% nodes and fabrication techniques that push the limits of physics carry larger
% risks of delays, and put fabs that can't keep up out of business. 20 years
% ago, almost 30 companies manufactured integrated circuits at leading-edge
% manufacturing processes, whereas only 5 do so today (Intel, Samsung, TSMC,
% Micron, and SK Hynix)~\cite{t10}. 

%In recent times, 

Semiconductor supply chain issues are at the front and center these days as chip
shortages continue to wreak havoc on our lives---on the supply of
computers~\cite{comp}, automobiles~\cite{auto}, and even sex toys~\cite{toys}.

While the mass awareness of supply chain issues has been recent, the
semiconductor industry has long been vulnerable to uncertainties (Figure~\ref{fig:SC_uncertainities}) in both
demand and supply of chips~\cite{monch2018survey}, and is becoming increasingly so~\cite{recent}. 
%As discussed in the next section, 
Indeed, natural disasters~\cite{natural}, geopolitical tensions~\cite{geopol}, economic
shocks~\cite{shock}, and characteristics inherent to the industry, such as long lead
times~\cite{leadtime}, economy-of-scale constraints~\cite{monch2018survey}, and short product
lifecycles~\cite{lifecycles},  cause uncertain supply and demand, which is compounded by
the global nature of the industry~\cite{monch2018survey}.
%compounds many of these problems, and current trends point to these problems
%getting worse. These interruptions can have a large cost to firms.
%Table~\ref{fig:disrupt_cost} lists some examples of unpredictable events and
%their financial impact to foundries. In most cases, it is reasonable to assume
%a similar, if not greater, monetary loss to chip companies that purchased from
%these foundries due to increased margins. 

\subsection{Data}
(Figure~\ref{fig:PC_mar_fluct}): \\
- Shows normalized total volume of PCs shipped for the total market, as well as for two individual vendors - HP and ASUS \\
-	There are significant variations in PC units shipped each year, and (more regular) quarterly variations within the same year. \\
-	Individual vendors don’t necessarily track with the market as a whole (ASUS) and even if they do in the case of HP, profits are unlinked from units shipped and still fluctuate \\

(Figure~\ref{fig:Util_revenue}): \\
- Shows month-by-month CPI-adjusted semiconductor sales as well as utilization (Output/Capacity percent) from 1986-2021 \\
-	Major (potentially unforecastable) events cause drops in sales – dotcom bust:8.2B drop in monthly revenue from previous year, 2008 financial crisis – 8.9B drop in sales, 2018 insustry downturn- 8.3 Billion \\
-	Semiconductor utilization does not correlate with sales- signaling regimes of supply or demand constraints. \\

(Figure~\ref{fig:Unc_in_forcast}): \\
- Projections for total yearly semiconductor revenue vs actual revenue from 2018 -2021 \\
-	Projections and actual sales data differ by 30-40 Billion dollars (RMS) per year over the last 4 years and the two induvidual projections have a 38 Billion dollar RMS difference\\
-	Projections are made at the middle of the year for the whole year, so are only forecasting half a year’s worth of revenue \\
-	A similar difference for the other half of the year would represent about a +/- 20 percent error in predicting\\
- The fact that the fluctuations cannot be predicted suggest that these fluctuations are in fact uncertainties\\

(Figure~\ref{fig:disrupt_cost}): \\
-	Sudden shocks to supply chains have become increasingly frequent, and result in significant losses to foundries, and potentially represent an even larger opportunity cost for chip companies that use these foundries \\
%This only reflects costs to foundries, not to the chip companies, which limits its credibility. 

%fluctuations can still cause losses because there is a need to adapt/scale which comes with added costs. 

\begin{figure}
    \centering
    %\includegraphics[width=6cm]{./images/newfigures/Uncertainity_in_semi_chain.png}
    \includegraphics[width=0.80\linewidth]{./images/newfigures/newuncern.png}
    \caption{Example semiconductor supply chain uncertainties}
    \label{fig:SC_uncertainities}
\end{figure}

\begin{figure}
    \centering
    %\includegraphics[width=6cm]{./images/PC_mar_fluct.png}
    \includegraphics[width=0.80\linewidth]{./images/PC_mar_fluct.png}
    \caption{Fluctuations in the PC industry}
    \label{fig:PC_mar_fluct}
\end{figure}

\begin{figure}
    \centering
    %\includegraphics[width=6cm]{./images/PC_mar_fluct.png}
    \includegraphics[width=0.80\linewidth]{./images/Util_revenue.png}
    \caption{Semiconductor production Utilization and Inflation-adjusted Revenues}
    \label{fig:Util_revenue}
\end{figure}

\begin{figure}
    \centering
    %\includegraphics[width=6cm]{./images/PC_mar_fluct.png}
    \includegraphics[width=0.80\linewidth]{./images/Unc_in_forcast_fluct.png}
    \caption{Semiconductor Revenues vs IDC and Gartner Projections}
    \label{fig:Unc_in_forcast}
\end{figure}



\begin{table*}[]
\small
\centering
\caption{\small Unforecasted events, resulting loss to foundry, and time to recover}
%\begin{tabular}{@{}llll@{}}
\begin{tabular}{p{0.34\linewidth}p{0.28\linewidth}p{0.15\linewidth}p{0.12\linewidth}}
\toprule
Event                                                   & Loss to foundry   (\$)                          & Time to recover & Occurrence      \\ \midrule
Power outage at TSMCs legacy process fab~\cite{t1}                & 28--35M (30--40K wafers)                      & 12   hours          & 8/2021     \\
Texas winter storm froze Samsung foundry~\cite{t2}                & 286--357M ($\sim$71K wafers)                & 1   month           & 4/2021     \\
Texas winter storm froze NXP foundry~\cite{t3}                    & $\sim$100M                                 & 1   month           & 4/2021     \\
Fire at Renesas facility in Naka Japan~\cite{t4}                  & 171M                                      & 1   month           & 3/2021     \\
Global Foundries quits on 7nm,   AMD shifts to TSMC~\cite{t5,t6} & $\sim$4.255B loss just from AMD             & Permanent       & 8/2019 \\
Current chip shortage due to surge in demand~\cite{t7}           & 60B & 2+   years          & 2020       \\
China-US trade war causes TSMC to lose HWAWEI sales~\cite{t8}  & 13\%   of TSMC's revenue $\sim$= 455M          & 2   months          & 2020       \\
Fire at Asahi Kasei Foundry~\cite{t9}                             & 100M               & ?                   & 2/2021     \\ \bottomrule
\label{fig:disrupt_cost}
\end{tabular}
\end{table*}


\begin{table}[]
    \centering
    \caption{\small Features of Colgate-Pamolive's supply chain and how/if chip companies can emulate them}
    \begin{tabular}{p{0.5\linewidth}p{0.5\linewidth}}
    \hline
        Colgate Pamolive & Semiconducor (chip company) \\ \hline
        100s of geographically dispersed suppliers and secondary suppliers not subject to trade embargoes or other restrictions & No control over secondary suppliers, process the chip(let) is designed for bounds max no of fabs their chips can be manufactured in \\ \hline
        Ability to stockpile significant amounts of product because of long product life time/shelf life & Can extend product lifetime by either making an innovative product or if the existing chip won't be a bottleneck even in next-generation designs eg. I/O \\ \hline
        Easy to adapt a product to sell it to a different market (slap a different label on it) & Can make the product adaptable through novel architectures \\ \hline
        Demand for products in over 200 countries, and constant demand & Can enter more markets to diversify demand, but not much can be done about this \\ \hline
        Large number of suppliers for each of the components of the final product & Don't have control over this (eg. there are only so many supplier of EUV scanners) \\ \hline
        85\% of production done under the same platform, only customize products in 15\% of the production & Currently most of production is specific to a product, but companies design their product line in a way that maximizes ability to compose from a set of basic chiplets \\ \hline
    \end{tabular}
\end{table}

The data presented above suggests that chips have high supply and demand uncertainty, and this is the conclusion Lee et al (2002)~\cite{Allign_SC_strat_Prod_Unc} came to as well. A popular framework for managing supply chains first proposed by Fisher (1997)~\cite{Allign_SC_strat_Prod_Unc} suggests that supply chains should be calibrated to the nature of the product they are servicing. Supply chains have a physical function (converting raw materials to product efficiently) and a market mediation function (mediating supply and demand). According to this framework,  supply chains for  products with high uncertainties should focus on improving their market mediating function whereas products with low uncertainties need to focus on making their supply chains more physically efficient. Thus high-performance ICs which Fisher and Lee et al. say have high uncertainties, fit best with a market-responsive or agile supply chain. The features of physically efficient and market responsive processes, as well as the corresponding features of semiconductor chains are described in table~\ref{fig:process_comp}. 

\begin{table*}[]
    \centering
    \caption{\small Comparison of Semiconductor supply chain characteristics to efficient and market-responsive processes}
    \begin{tabular}{p{0.12\linewidth}p{0.2\linewidth}p{0.2\linewidth}p{0.32\linewidth}}
    \toprule
        Aspect & Efficient Process & Market-Responsive Process & Silicon Process  \\ \hline
        Manufacturing Focus & Maintain High Average Utilization Rate & deploy excess buffer capacity & High utilization to keep costs down  \\ \hline
        Inventory Strategy & Generate high turns and minimize inventory throughout the chain & deploy significant buffer stocks of parts or finished goods & No significant buffering after wafer phase due to short product life cycle  \\ \hline
        Lead-time Focus & Only shorten lead time if it doesn't increase cost & Aggressively invest to reduce lead time & Limited opportunities to reduce lead time  \\ \hline
        Approach to choosing suppliers & select primarily for cost and quality & Select primarily for speed, flexibility and quality & Limited choice of suppliers (fabs) for leading edge nodes and intermediary equipment (eg EUV scanners)  \\ \hline
        Product-Design Strategy & maximize performance and minimize cost & Design to postpone product differentiation for as long as possible & Limited Product Differentiation Possible after fabrication in conventional designs, so designed to maximize performance and minimize cost (area)  \\ \hline
    \end{tabular}
    \label{fig:process_comp}
\end{table*}

It is thus clear from this that Silicon Processes are more physically efficient than market responsive, demonstrating that there is a mismatch between the product and the supply chain.  According to Lee et. Al, this mismatch can be bridged through changing the product or the supply chain. Changing the semiconductor supply chain will take a long time (it takes more than 6 years to build a fab) and be very expensive, and for the most part is out of the control of chip companies. But our analysis shows that changes to the product can be made to match it better to existing semiconductor supply chains. Likewise, analysis done by Cohen et. Al (2022)~\cite{Bespoke_SC_resilience} shows that for high performance chips, the constraint is product. 
The table~\ref{fig:Product_redesign} details some ways products can be re-designed to create a more market-reactive. 


\begin{table}[!ht]
    \centering
    \caption{\small Comparison of Semiconductor supply chain characteristics to efficient and market-responsive processes}
    \begin{tabular}{p{0.4\linewidth}p{0.4\linewidth}}
    \hline
        Desired Characteristic & Potential Product redesign  \\ \hline
        Ability to maintain buffer stocks & Create products with longer life cycle by aggregating components that are reused in successive designs  \\ \hline
        Have broader supply base & Design (parts of) products on trailing processes that support multiple manufacturers  \\ \hline
        Delay Product Differentiation & Design products to be adaptable to different products after manufacturing  \\ \hline
    \end{tabular}
   \label{fig:Product_redesign} 
\end{table}



\iffalse
Addressing the resilience of semiconductor supply chains has taken a unique
    salience in the context of the present day. Geopolitical tensions and
    natural disasters that have the potential to severely disrupt the global
    industry are increasing, and the current global semiconductor shortage has
    created an increased receptiveness to building resilience, as designers
    have already been forced to alter designs to account for supply
    constraints~\cite{spectrum}. 
\fi

Improving semiconductor supply chain resilience has traditionally
been thought of as a logistics and planning/forecasting problem concerned
with selecting the correct suppliers~\cite{suppliers}, managing inventory~\cite{inventory,suppliers},
ensuring good communication between entities in the supply chain~\cite{communication,communication02},
etc.  In this paper, we ask: {\em do computer architects have
a role in improving semiconductor supply chain resilience?}

The key observation driving this paper is that any one-to-one correspondence
    between produced chips and demanded chips can lead to
    {\em fragility} in the semiconductor
    supply chains -- high impact on cost from supply and demand
    uncertainties. I.e., if we produce a single chip (or a single collection of chips) to
    satisfy a given demand, this creates a single path to satisfy the
    chip demand.  Any fluctuations in supply or demand then can directly lead
    to shortages or overages leading to increased costs. {\em Chip architects
    can enable multiple paths to satisfy a chip demand, which can improve
    supply chain resilience}.  Multiple paths can be enabled, for example, by
    decoupling produced chips from demand in such a way that a chip demand is
    met using an appropriate subset of produced chips depending on supply and demand. Newer paths can also be
    enabled by choice of architecture and implementation technology that allows
    chips to be produced by multiple suppliers.

%However, in this paper We seek to show that Computer Architects can play a
%role in mitigating the effect of supply chain disruptions by creating
%novel architectures that allow for remedial of specific risk factors in
%the supply chain. 


% \footnote{Will try to find a more concrete example here of some company
    % improving their supply chain resilience through better product design}

We study three classes of techniques (Figure~\ref{fig:overview}) that chip architects can use to
increase the number of paths to satisfying chip demand and, therefore, improve
semiconductor supply chain resilience. 
\begin{itemize}
    \item {\em Composition}:  The demanded chip is  built using multiple
        unequal, sometimes disjoint,  sets of produced components (IPs,
        chiplets, etc.). This enables chip demand to be satisfied even if
        supply of some produced components are constrained. Conventionally,
        composition is focused on minimizing cost by maximizing
        disaggregation~\cite{chiplet,amdnext,tadayon2020moore}; we focus
        instead on enabling multiple paths for supply chain resilience.  
    \item {\em Adaptation}:  A chip produced to satisfy a given chip demand is
        built so it can be used also as a replacement for a different
        chip demand. This enables any chip shortage to be addressed using a
        different chip that may be available. Conventionally, adaptation has not been considered for addressing supply and demand disruptions.   
    \item {\em Dispersion}:  A chip is built such that all or part of a chip
        can be implemented using a technology or an IP that can be sourced from
        numerous suppliers. Dispersion allows disruptions in supply to be
        compensated by other suppliers. 
        %We are unaware of the    
 
 \end{itemize}
 
To evaluate the efficacy of composition, adaptation, and dispersion on
improving semiconductor supply chain resilience, we develop a model that
estimates the impact of semiconductor supply chain uncertainties on overall
cost with and without the application of these techniques. The model considers both the cost of shortages and overages that result
from supply chain (and yield)  uncertainties as well as recurring and
non-recurring costs of chip production.
%and is general enough to represent the different architectural interventions. 
Composition, adaptation, and disruption are expressed in the model as different
mappings between produced chips and chip demands. 
%using a variety of `mappings' and replications of supply goods.
We then use a multistage stochastic program with recourse
(MSPR)~\cite{mspr,mspr2} to find optimal purchasing and mapping
decisions under different regimes of supply/demand uncertainty in order to
better compare the various techniques and evaluate their efficacy in different
scenarios.

\iffalse
The model also allows us to make intelligent architectural decisions that
improve resilience to supply chain uncertainties. To understand and evaluate
architectural decision-making in presence of supply chain uncertainties, we
consider three case studies, one for each type of architectural intervention.
\fi

Our results confirm that semiconductor supply chains that do not use
composition, adaptation, or dispersion are fragile and have high cost increases
in the presence of supply chain uncertainties and shocks. We find that composition
is very effective at addressing supply uncertainties and shocks, but not
very effective at addressing uncertainties and shocks in demand.
Effectiveness of composition also depends strongly on the supply and timing of
packaging. Adaptation is much more effective at addressing demand uncertainties
and shocks but not as effective with supply disruptions. The orthogonal
benefits from composition and adaptation motivate architectures that support
both. Dispersible architectures provide effective resilience against supply
disruptions,
but risk increasing overall costs if NRE costs are not amortized well over multiple suppliers.
%and, therefore, must be used
%with caution. 
%To the best of our knowledge, this is the first paper that
%studies the role of chip architecture in providing supply chain resilience.

This paper makes the following contributions.
\begin{itemize}
    \item We perform the first study on the role of chip architecture in
        providing semiconductor supply chain resilience.
    \item We make a key observation (and demonstrate quantitatively) that a
        one-to-one mapping between produced and demanded chips leads to high
        cost from supply and demand disruptions.
    \item We develop a model that allows us to analyze the impact of different
        architectural techniques on supply chain costs. This is the first such
        model and will be open sourced as a tool as it may have wider use.
    \item We show quantitatively that composition, adaptation, and dispersion
        can be effective techniques at providing supply chain resilience.
    \item We provide specific recommendations for architects in different
        supply and demand regimes. These are the first such recommendations for
        architects, as far as we know.
 \end{itemize}




\begin{figure}
    \centering
    \includegraphics[width=0.65\linewidth]{./images/newfigures/intro.png}
    \caption{Composition, adaptation, and dispersion can be used to decouple produced chips and chip demands}
    \label{fig:overview}
\end{figure}

\iffalse

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{./images/newfigures/intro2.png}
    \caption{Caption}
    \label{fig:my_label}
\end{figure}

\fi


==> newintro_rama.tex <==
% The semiconductor industry is becoming increasingly complex and uncertain due
% to a variety of factors. More complex designs may not perform to expectations
% or have other issues that delay their production. Cutting edge technology
% nodes and fabrication techniques that push the limits of physics carry larger
% risks of delays, and put fabs that can't keep up out of business. 20 years
% ago, almost 30 companies manufactured integrated circuits at leading-edge
% manufacturing processes, whereas only 5 do so today (Intel, Samsung, TSMC,
% Micron, and SK Hynix)~\cite{t10}. 

%In recent times, 

Semiconductor supply chain issues are at the front and center these days as chip
shortages continue to wreak havoc on our lives---on the supply of
computers~\cite{comp}, automobiles~\cite{auto}, and even sex toys~\cite{toys}.

While the mass awareness of supply chain issues has been recent, the
semiconductor industry has long been vulnerable to uncertainties (Figure~\ref{fig:SC_uncertainities}) in both demand and supply of chips~\cite{monch2018survey}, and is becoming increasingly so~\cite{recent}. 
%As discussed in the next section, 
Indeed, natural disasters~\cite{natural}, geopolitical tensions~\cite{geopol}, economic
shocks~\cite{shock}, and characteristics inherent to the industry, such as long lead
times~\cite{leadtime}, economy-of-scale constraints~\cite{monch2018survey}, and short product lifecycles~\cite{lifecycles},  cause uncertain supply and demand, which is compounded by the global nature of the industry~\cite{monch2018survey}.

\begin{figure}
    \centering
    %\includegraphics[width=6cm]{./images/newfigures/Uncertainity_in_semi_chain.png}
    \includegraphics[width=0.80\linewidth]{./images/newfigures/newuncern.png}
    \caption{Example semiconductor supply chain uncertainties}
    \label{fig:SC_uncertainities}
\end{figure}
%compounds many of these problems, and current trends point to these problems
%getting worse. These interruptions can have a large cost to firms.
%Table~\ref{fig:disrupt_cost} lists some examples of unpredictable events and
%their financial impact to foundries. In most cases, it is reasonable to assume
%a similar, if not greater, monetary loss to chip companies that purchased from
%these foundries due to increased margins. 

Figure~\ref{fig:PC_mar_fluct} shows the variation in number of PCs per quarter by HP, ASUS and all PC suppliers. We normalize the PCs sold by all suppliers and ASUS  to number of HP PCs sold in order to understand the variance. Clearly, there are significant variations every year and even per quarter as a result of demand and supply uncertainty. 

There are multiple techniques that chip manufacturers can apply to account for this variation and attain a market equilibrium that brings maximum profit. One solution is that chip manufacturers reduce lead time and have large inventories for produced chips. Short lead times can help react to demand uncertainty in the market and inventories can act as a buffer for for both supply and demand uncertainty. But, the inherent process of chip manufacturing makes it impossible to have short lead times during production. Assuming the chip is designed and verified, and the mask to manufacture the chip has been acquired, there are still multiple engineering processes that need to be followed before the chip is sold. All chips need to be tested using ATPG to discard faulty chips. Operating voltage and frequency needs to be determined per chip to account for process variation and then they have to be binned into respective performance/power categories before being sold. Furthermore, this estimation assumes that semiconductor fabs can respond to demand from chip manufacturers immediately. Take Figure~\ref{fig:Util_revenue} that shows month-by-month CPI-adjusted semiconductor sales as well as utilization from 1986-2021. Fabrication plants service multiple chip manufactures and run almost constantly at capacity. So there is a large lead time cost that is incurred here as well making it even more challenging for chip manufacturers to respond to fine grain variations in the demand market. 

Another technique that is used to account for supply and demand uncertainty is forecasting. Predicting market behaviour can help mask the uncertainty and help manufacturers with inflexible supply chains to adapt to market variation. Figure~\ref{fig:Unc_in_forcast} depicts projections for total yearly semiconductor revenue vs actual revenue from 2018 -2021. The data for projections and actual sales differ by 30-40 billion dollars per year. this is evidence that market behaviour is unpredictable and fluctuations are in fact uncertainties. 

\begin{figure*}[ht]
    \centering
    %\includegraphics[width=6cm]{./images/PC_mar_fluct.png}
    \captionsetup[subfloat]{captionskip=-2pt,nearskip=-4pt}
     \subfloat[\centering Fluctuations in the PC industry]{
        {\includegraphics[width=0.27\linewidth]{./images/PC_mar_fluct.png}}
        \label{fig:PC_mar_fluct}
    } \qquad
    \subfloat[\centering Semiconductor production Utilization and Inflation-adjusted Revenues]{
        {\includegraphics[width=0.27\linewidth]{./images/Util_revenue.png}}
        \label{fig:Util_revenue} 
    }\qquad
    \subfloat[\centering Semiconductor Revenues vs IDC and Gartner Projections]{
        {\includegraphics[width=0.27\linewidth]{./images/Unc_in_forcast_fluct.png}}
        \label{fig:Unc_in_forcast} 
    }
    \label{fig:motivation}
    \caption{Semiconductor industry trends}
\end{figure*}

(Figure~\ref{fig:disrupt_cost}): \\
-	Sudden shocks to supply chains have become increasingly frequent, and result in significant losses to foundries, and potentially represent an even larger opportunity cost for chip companies that use these foundries \\
%This only reflects costs to foundries, not to the chip companies, which limits its credibility. 

%fluctuations can still cause losses because there is a need to adapt/scale which comes with added costs. 



% \begin{figure}
%     \centering
%     %\includegraphics[width=6cm]{./images/PC_mar_fluct.png}
%     \includegraphics[width=0.80\linewidth]{./images/PC_mar_fluct.png}
%     \caption{Fluctuations in the PC industry}
%     \label{fig:PC_mar_fluct}
% \end{figure}

% \begin{figure}
%     \centering
%     %\includegraphics[width=6cm]{./images/PC_mar_fluct.png}
%     \includegraphics[width=0.80\linewidth]{./images/Util_revenue.png}
%     \caption{Semiconductor production Utilization and Inflation-adjusted Revenues}
%     \label{fig:Util_revenue}
% \end{figure}

% \begin{figure}
%     \centering
%     %\includegraphics[width=6cm]{./images/PC_mar_fluct.png}
%     \includegraphics[width=0.80\linewidth]{./images/Unc_in_forcast_fluct.png}
%     \caption{Semiconductor Revenues vs IDC and Gartner Projections}
%     \label{fig:Unc_in_forcast}
% \end{figure}



\begin{table*}[]
\small
\centering
\caption{\small Unforecasted events, resulting loss to foundry, and time to recover}
%\begin{tabular}{@{}llll@{}}
\begin{tabular}{p{0.34\linewidth}p{0.28\linewidth}p{0.15\linewidth}p{0.12\linewidth}}
\toprule
Event                                                   & Loss to foundry   (\$)                          & Time to recover & Occurrence      \\ \midrule
Power outage at TSMCs legacy process fab~\cite{t1}                & 28--35M (30--40K wafers)                      & 12   hours          & 8/2021     \\
Texas winter storm froze Samsung foundry~\cite{t2}                & 286--357M ($\sim$71K wafers)                & 1   month           & 4/2021     \\
Texas winter storm froze NXP foundry~\cite{t3}                    & $\sim$100M                                 & 1   month           & 4/2021     \\
Fire at Renesas facility in Naka Japan~\cite{t4}                  & 171M                                      & 1   month           & 3/2021     \\
Global Foundries quits on 7nm,   AMD shifts to TSMC~\cite{t5,t6} & $\sim$4.255B loss just from AMD             & Permanent       & 8/2019 \\
Current chip shortage due to surge in demand~\cite{t7}           & 60B & 2+   years          & 2020       \\
China-US trade war causes TSMC to lose HWAWEI sales~\cite{t8}  & 13\%   of TSMC's revenue $\sim$= 455M          & 2   months          & 2020       \\
Fire at Asahi Kasei Foundry~\cite{t9}                             & 100M               & ?                   & 2/2021     \\ \bottomrule
\label{fig:disrupt_cost}
\end{tabular}
\end{table*}


% \begin{table*}[]
%     \centering
%     \caption{\small Features of Colgate-Pamolive's supply chain and how/if chip companies can emulate them}
%     \begin{tabular}{p{0.5\linewidth}p{0.5\linewidth}}
%     \hline
%         Colgate Pamolive & Semiconducor (chip company) \\ \hline
%         100s of geographically dispersed suppliers and secondary suppliers not subject to trade embargoes or other restrictions & No control over secondary suppliers, process the chip(let) is designed for bounds max no of fabs their chips can be manufactured in \\ \hline
%         Ability to stockpile significant amounts of product because of long product life time/shelf life & Can extend product lifetime by either making an innovative product or if the existing chip won't be a bottleneck even in next-generation designs eg. I/O \\ \hline
%         Easy to adapt a product to sell it to a different market (slap a different label on it) & Can make the product adaptable through novel architectures \\ \hline
%         Demand for products in over 200 countries, and constant demand & Can enter more markets to diversify demand, but not much can be done about this \\ \hline
%         Large number of suppliers for each of the components of the final product & Don't have control over this (eg. there are only so many supplier of EUV scanners) \\ \hline
%         85\% of production done under the same platform, only customize products in 15\% of the production & Currently most of production is specific to a product, but companies design their product line in a way that maximizes ability to compose from a set of basic chiplets \\ \hline
%     \end{tabular}
% \end{table*}

The data presented above suggests that chips have high supply and demand uncertainty, and this is the conclusion Lee et al (2002)~\cite{Allign_SC_strat_Prod_Unc} came to as well. A popular framework for managing supply chains first proposed by Fisher (1997)~\cite{Allign_SC_strat_Prod_Unc} suggests that supply chains should be calibrated to the nature of the product they are servicing. Supply chains have a physical function (converting raw materials to product efficiently) and a market mediation function (mediating supply and demand). According to this framework,  supply chains for  products with high uncertainties should focus on improving their market mediating function whereas products with low uncertainties need to focus on making their supply chains more physically efficient. Thus high-performance ICs which Fisher and Lee et al. say have high uncertainties, fit best with a market-responsive or agile supply chain. The features of physically efficient and market responsive processes, as well as the corresponding features of semiconductor chains are described in table~\ref{fig:process_comp}. 

\begin{table*}[]
    \centering
    \caption{\small Comparison of Semiconductor supply chain characteristics to efficient and market-responsive processes}
    \begin{tabular}{p{0.12\linewidth}p{0.2\linewidth}p{0.2\linewidth}p{0.32\linewidth}}
    \toprule
        Aspect & Efficient Process & Market-Responsive Process & Silicon Process  \\ \hline
        Manufacturing Focus & Maintain High Average Utilization Rate & deploy excess buffer capacity & High utilization to keep costs down  \\ \hline
        Inventory Strategy & Generate high turns and minimize inventory throughout the chain & deploy significant buffer stocks of parts or finished goods & No significant buffering after wafer phase due to short product life cycle  \\ \hline
        Lead-time Focus & Only shorten lead time if it doesn't increase cost & Aggressively invest to reduce lead time & Limited opportunities to reduce lead time  \\ \hline
        Approach to choosing suppliers & select primarily for cost and quality & Select primarily for speed, flexibility and quality & Limited choice of suppliers (fabs) for leading edge nodes and intermediary equipment (eg EUV scanners)  \\ \hline
        Product-Design Strategy & maximize performance and minimize cost & Design to postpone product differentiation for as long as possible & Limited Product Differentiation Possible after fabrication in conventional designs, so designed to maximize performance and minimize cost (area)  \\ \hline
    \end{tabular}
    \label{fig:process_comp}
\end{table*}

It is thus clear from this that Silicon Processes are more physically efficient than market responsive, demonstrating that there is a mismatch between the product and the supply chain.  According to Lee et. Al, this mismatch can be bridged through changing the product or the supply chain. Changing the semiconductor supply chain will take a long time (it takes more than 6 years to build a fab) and be very expensive, and for the most part is out of the control of chip companies. But our analysis shows that changes to the product can be made to match it better to existing semiconductor supply chains. Likewise, analysis done by Cohen et. Al (2022)~\cite{Bespoke_SC_resilience} shows that for high performance chips, the constraint is product. 
The table~\ref{fig:Product_redesign} details some ways products can be re-designed to create a more market-reactive. 


\begin{table}[!ht]
    \centering
    \caption{\small Comparison of Semiconductor supply chain characteristics to efficient and market-responsive processes}
    \begin{tabular}{p{0.4\linewidth}p{0.4\linewidth}}
    \hline
        Desired Characteristic & Potential Product redesign  \\ \hline
        Ability to maintain buffer stocks & Create products with longer life cycle by aggregating components that are reused in successive designs  \\ \hline
        Have broader supply base & Design (parts of) products on trailing processes that support multiple manufacturers  \\ \hline
        Delay Product Differentiation & Design products to be adaptable to different products after manufacturing  \\ \hline
    \end{tabular}
   \label{fig:Product_redesign} 
\end{table}



\iffalse
Addressing the resilience of semiconductor supply chains has taken a unique
    salience in the context of the present day. Geopolitical tensions and
    natural disasters that have the potential to severely disrupt the global
    industry are increasing, and the current global semiconductor shortage has
    created an increased receptiveness to building resilience, as designers
    have already been forced to alter designs to account for supply
    constraints~\cite{spectrum}. 
\fi

Improving semiconductor supply chain resilience has traditionally
been thought of as a logistics and planning/forecasting problem concerned
with selecting the correct suppliers~\cite{suppliers}, managing inventory~\cite{inventory,suppliers},
ensuring good communication between entities in the supply chain~\cite{communication,communication02},
etc.  In this paper, we ask: {\em do computer architects have
a role in improving semiconductor supply chain resilience?}

The key observation driving this paper is that any one-to-one correspondence
    between produced chips and demanded chips can lead to
    {\em fragility} in the semiconductor
    supply chains -- high impact on cost from supply and demand
    uncertainties. I.e., if we produce a single chip (or a single collection of chips) to
    satisfy a given demand, this creates a single path to satisfy the
    chip demand.  Any fluctuations in supply or demand then can directly lead
    to shortages or overages leading to increased costs. {\em Chip architects
    can enable multiple paths to satisfy a chip demand, which can improve
    supply chain resilience}.  Multiple paths can be enabled, for example, by
    decoupling produced chips from demand in such a way that a chip demand is
    met using an appropriate subset of produced chips depending on supply and demand. Newer paths can also be
    enabled by choice of architecture and implementation technology that allows
    chips to be produced by multiple suppliers.

%However, in this paper We seek to show that Computer Architects can play a
%role in mitigating the effect of supply chain disruptions by creating
%novel architectures that allow for remedial of specific risk factors in
%the supply chain. 


% \footnote{Will try to find a more concrete example here of some company
    % improving their supply chain resilience through better product design}

We study three classes of techniques (Figure~\ref{fig:overview}) that chip architects can use to
increase the number of paths to satisfying chip demand and, therefore, improve
semiconductor supply chain resilience. 
\begin{itemize}
    \item {\em Composition}:  The demanded chip is  built using multiple
        unequal, sometimes disjoint,  sets of produced components (IPs,
        chiplets, etc.). This enables chip demand to be satisfied even if
        supply of some produced components are constrained. Conventionally,
        composition is focused on minimizing cost by maximizing
        disaggregation~\cite{chiplet,amdnext,tadayon2020moore}; we focus
        instead on enabling multiple paths for supply chain resilience.  
    \item {\em Adaptation}:  A chip produced to satisfy a given chip demand is
        built so it can be used also as a replacement for a different
        chip demand. This enables any chip shortage to be addressed using a
        different chip that may be available. Conventionally, adaptation has not been considered for addressing supply and demand disruptions.   
    \item {\em Dispersion}:  A chip is built such that all or part of a chip
        can be implemented using a technology or an IP that can be sourced from
        numerous suppliers. Dispersion allows disruptions in supply to be
        compensated by other suppliers. 
        %We are unaware of the    
 
 \end{itemize}
 
To evaluate the efficacy of composition, adaptation, and dispersion on
improving semiconductor supply chain resilience, we develop a model that
estimates the impact of semiconductor supply chain uncertainties on overall
cost with and without the application of these techniques. The model considers both the cost of shortages and overages that result
from supply chain (and yield)  uncertainties as well as recurring and
non-recurring costs of chip production.
%and is general enough to represent the different architectural interventions. 
Composition, adaptation, and disruption are expressed in the model as different
mappings between produced chips and chip demands. 
%using a variety of `mappings' and replications of supply goods.
We then use a multistage stochastic program with recourse
(MSPR)~\cite{mspr,mspr2} to find optimal purchasing and mapping
decisions under different regimes of supply/demand uncertainty in order to
better compare the various techniques and evaluate their efficacy in different
scenarios.

\iffalse
The model also allows us to make intelligent architectural decisions that
improve resilience to supply chain uncertainties. To understand and evaluate
architectural decision-making in presence of supply chain uncertainties, we
consider three case studies, one for each type of architectural intervention.
\fi

Our results confirm that semiconductor supply chains that do not use
composition, adaptation, or dispersion are fragile and have high cost increases
in the presence of supply chain uncertainties and shocks. We find that composition
is very effective at addressing supply uncertainties and shocks, but not
very effective at addressing uncertainties and shocks in demand.
Effectiveness of composition also depends strongly on the supply and timing of
packaging. Adaptation is much more effective at addressing demand uncertainties
and shocks but not as effective with supply disruptions. The orthogonal
benefits from composition and adaptation motivate architectures that support
both. Dispersible architectures provide effective resilience against supply
disruptions,
but risk increasing overall costs if NRE costs are not amortized well over multiple suppliers.
%and, therefore, must be used
%with caution. 
%To the best of our knowledge, this is the first paper that
%studies the role of chip architecture in providing supply chain resilience.

This paper makes the following contributions.
\begin{itemize}
    \item We perform the first study on the role of chip architecture in
        providing semiconductor supply chain resilience.
    \item We make a key observation (and demonstrate quantitatively) that a
        one-to-one mapping between produced and demanded chips leads to high
        cost from supply and demand disruptions.
    \item We develop a model that allows us to analyze the impact of different
        architectural techniques on supply chain costs. This is the first such
        model and will be open sourced as a tool as it may have wider use.
    \item We show quantitatively that composition, adaptation, and dispersion
        can be effective techniques at providing supply chain resilience.
    \item We provide specific recommendations for architects in different
        supply and demand regimes. These are the first such recommendations for
        architects, as far as we know.
 \end{itemize}




\begin{figure}
    \centering
    \includegraphics[width=0.65\linewidth]{./images/newfigures/intro.png}
    \caption{Composition, adaptation, and dispersion can be used to decouple produced chips and chip demands}
    \label{fig:overview}
\end{figure}

\iffalse

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{./images/newfigures/intro2.png}
    \caption{Caption}
    \label{fig:my_label}
\end{figure}

\fi


==> optim.tex <==
%\label{sec:optimal_policies}

\nathan{
In order to isolate the benefits of interventions, interventions must be applied
with optimal order and mapping policies.  Were they not, then it would be
difficult to discern whether benefits are derived from interventions, or are
simply artifacts of sub-optimal order and mapping policy decisions.
}
Under many circumstances, finding policies which minimize total cost is
possible.  Consider first a baseline case in which there are $n$ of goods whose
demand is met by directly producing those goods (i.e., $M_x$ is identity, and
$\Gamma_x$ evaluates to constant $0$), and in which supply and demand
uncertainty are modeled by constant random variables.
This can be modeled as the optimization problem
% \begin{alignat}{3}
%     \argmin_x & \quad & TC(x) \\
%     \text{subject to: } x \geq 0.
% \end{alignat}

\begin{alignat}{3}
\argmin_x           &\quad&  TC(x)     && \\
\text{subject to: } &\quad&  x_i \geq 0 &&\quad \forall i \in \{1, \ldots, n\}.
\end{alignat}

As supply and demand for each good is independent (as \textit{any} collection
of constant random variables is independent), this optimization problem
can be decomposed into $n$ disjoint subproblems, one for each good.
In this case, the optimal quantity of each good
to \textit{produce} is either exactly the ammount demanded, or zero (in the
case that NRE for that good is high relative)\footnote{assuming salvage value
$h$ is lower than unit cost $c$}.  If more than the required quantity of goods
is produced, then excess goods can only be sold for $h < c$.
On the other hand, if fewer goods are produced
than demanded, then profits are minimized by $r-c$.  If $r-c < 0$, then
the optimal quantity to produce is $0$, as no profit can be generated from
this good.

With this in mind, the following (realistic) assumptions are used for all
optimization problems. For all goods
\begin{itemize}
    \item $h\cdot Z_s < c$, since otherwise the optimal quantity to order is $+\infty$.
    \item $r\cdot Z_s > c$, since otherwise the optimal quantity to order is $0$,
          trivially.
    \item $\expectation{Z_d(r-c)} > n$, since otherwise the optimal quantity
          to build is 0, trivially.
\end{itemize}

\subsection{Baseline with Uncertainty}
Incorporating uncertainty into the baseline optimization problem leads to a
more interesting optimization problem.
First, 



==> optimization.tex <==
Each of the previous intervention strategies are potentially useful in mitigating supply and demand uncertainty. However, the question of what decisions to make with respect to these strategies is still unclear. To provide a roadmap of which decisions may be best, the following optimization problems are proposed, each of which target a different intervention strategy.

\subsection{Composition}
The primary decision to be made when dealing with composition is the components to produce and how to compose them. To discover this best decision, we will minimize total cost with respect to the selected mapping.

Start with multiple demands, a list of components that can be produced and a list of architectures which use these components to meet the demands.

The problem is simply that of selecting the mapping from the family of mappings $M_{x}$ which minimizes total cost


\begin{equation}
    \underset{M \in M_{x}}{\operatorname{argmin}}TC_{M}
\end{equation}

And rerunning the minimization with growing supply and demand uncertainty to see the impact this has on the optimal $M$.

The composition-specific costs to be added into the model consist of the cost of integration, which will be represented by the cost-of-mapping function $\Gamma$. Integration costs consist of the cost of bonding, the cost of the interposer, and the cost of testing the packaged chip. Everything else is covered by the parameters of per-unit cost, NRE and yield.

Further optimization problems to consider would include the optimal number of components per chip (if one number must be selected) or the optimal form of composition (i.e. chiplets vs multipackage). Both would still be a minimization over cost with respect to mappings, but the pool of mappings would be thinned to allow for comparison i.e. only mappings of four-chiplet processors will be used.

\subsection{Adaptation}
The primary decision to be made when dealing with adaptation is the level of adaptation supported. 

\begin{equation}
    \min_{M \in \mathbb{M}}\mathbb{E}_{Z_{s}}[TC_{M}]
\end{equation}

Additionally, we can perform the optimization with demand uncertainty instead of supply uncertainty, giving

\begin{equation}
    \min_{M \in \mathbb{M}}\mathbb{E}_{Z_{d}}[TC_{M}]
\end{equation}

\subsection{Commoditization}
The primary decision to be made when dealing with commoditization is the types of commodity good used. One way to represent this is through mixed process node usage.

To allow for this, we replay the composition optimization problem with chiplets in different process nodes and foundries. Some chiplets may be impossible to place in a simpler node i.e. the I/O chiplet can almost certainly go into a older node than the core itself.

%subsection to bring adapt and comp together with accelerator chiplet?


==> rebadgingTable.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[htp]
\small
\label{tab:rebadging}
\caption{Rebadging/Rebranding and Refreshing}
\begin{tabular}{@{}lll@{}}
\toprule
Rebadged/Refreshed                                                                                   & Original                      & Notes                                                                                                                                                          \\ \midrule
P1: A12X                                                                                             & P2: A12Z                      & \begin{tabular}[c]{@{}l@{}}P1: 8 processing cores @2.48GHz, \\ 7 GPU cores, 1 latent GPU core; \\ P2: 8 processing cores @2.48GHz, \\ 8 GPU cores\end{tabular} \\
P1: A5 (iPad 2)                                                                                      & P2: A5 (3rd Gen apple TV)     & \begin{tabular}[c]{@{}l@{}}P1: Dual core processor, \\ P2: Single core processor \\ (other core is disabled)\end{tabular}                                      \\
P1: Google Pixel 6                                                                                   & P2: Exynos 9855 (whitechapel) &                                                                                                                                                                \\
AMD Ryzen 5 5500U                                                                                    & Ryzen 5 4600U                 & \begin{tabular}[c]{@{}l@{}}The Ryzen 5 5500U is effectively \\ a Ryzen 5 4500U with SMT enabled, \\ or a rebranded Ryzen 5 4600U.\end{tabular}                 \\
Core i3 8350K                                                                                        & Core i5 7600K                 & \begin{tabular}[c]{@{}l@{}}Mildly downclocked, Rated maximum \\ memory controller frequency of \\ 2,400MHz, as opposed to 2,666MHz,\\ \$100 less\end{tabular}  \\
Radedon RX 640                                                                                       & Radeon RX 550X                &                                                                                                                                                                \\
Radeon 630                                                                                           & Radeon RX 540                 &                                                                                                                                                                \\
Radeon 625                                                                                           & Radeon 530                    & Previous Previous Name: Radeon R7 430                                                                                                                          \\
Radeon 620                                                                                           & Radeon 530                    & Previous Previous Name: Radeon R7 430                                                                                                                          \\
Radeon 610                                                                                           & Radeon 520                    & Previous Previous Name: Radeon R5 435                                                                                                                          \\
                                                                                                     &                               &                                                                                                                                                                \\
\begin{tabular}[c]{@{}l@{}}Radeon R5 240 OEM, \\ Radeon R7 240 (OLAND)\end{tabular}                  & Radeon HD 8570 OEM            & Rebadged                                                                                                                                                       \\
Radeon R7 240                                                                                        & Radeon HD 8670 OEM            & Rebadged                                                                                                                                                       \\
Radeon R7 250X (Cape Verde XT)                                                                       & Radeon HD 7770 GHz Edition    & Rebadged                                                                                                                                                       \\
Radeon R7 265                                                                                        & Radeon HD 7850                & Rebadged                                                                                                                                                       \\
Radeon R9 270 (Pitcairn XT)                                                                          & Radeon HD 7870                & Rebadged                                                                                                                                                       \\
Radeon R9 270X (Pitcairn XT)                                                                         & Radeon HD 7870 GHz Edition    & Rebadged                                                                                                                                                       \\
Radeon R9 280                                                                                        & Radeon HD 7950                & Rebadged                                                                                                                                                       \\
Radeon R7 270/270X                                                                                   & Radeon HD 7870                & Rebadged                                                                                                                                                       \\
Radeon R9 280X                                                                                       & Radeon HD 7970 GHz Edition    & Rebadged                                                                                                                                                       \\
\begin{tabular}[c]{@{}l@{}}Radeon R7 350 OEM,\\ Radeon R7 340 OEM\end{tabular}                       & Radeon R7 250                 & Rebadged                                                                                                                                                       \\
Radeon RX 455 OEM                                                                                    & AMD Radeon R7 360             & Rebadged                                                                                                                                                       \\
                                                                                                     &                               & Rebadged                                                                                                                                                       \\
P1: NVIDIA Titan RTX                                                                                 & P2: RTX 2080 Ti               & \begin{tabular}[c]{@{}l@{}}Both have TU102 GPU, \\ P1: 4608 CUDA Cores, \\ P2: 4352 CUDA Cores\end{tabular}                                                    \\
P1: GeForce GT 730M                                                                                  & P2: GeForce GT 640M           &                                                                                                                                                                \\
                                                                                                     &                               &                                                                                                                                                                \\
GeForce 9800 GT                                                                                      & GeForce 8800 GT               & Rebadged                                                                                                                                                       \\
GeForce GTX 760 Ti OEM                                                                               & GeForce GTX 660 Ti            & Rebadged                                                                                                                                                       \\
GeForce 605 OEM                                                                                      & GeForce 510 OEM               & Rebadged                                                                                                                                                       \\
\begin{tabular}[c]{@{}l@{}}GeForce GT 610, \\ GeForce GT 620 OEM, \\ GeForce GT 705 OEM\end{tabular} & GeForce GT 520                & Rebadged                                                                                                                                                       \\
GeForce GT 620                                                                                       & GeForce GT 530 OEM            & Rebadged                                                                                                                                                       \\
\begin{tabular}[c]{@{}l@{}}GeForce GT 730 (DDR3), \\ GeForce GT 630 (DDR3)\end{tabular}              & GeForce GT 440                & Rebadged                                                                                                                                                       \\
GeForce GT 640 OEM Rebrand (GF116)                                                                   & GeForce GT 545                & Rebadged                                                                                                                                                       \\
GeForce GT 645 OEM                                                                                   & GeForce GTX 560 SE            & Rebadged                                                                                                                                                       \\
GeForce GT 730 GDDR5                                                                                 & GeForce GT 630 Rev. 2         & Rebadged                                                                                                                                                       \\
GeForce GTX 770 (GK104)                                                                              & GeForce GTX 680               & Rebadged                                                                                                                                                       \\
GeForce GTX 760 Ti OEM                                                                               & GeForce GTX 670               & Rebadged                                                                                                                                                       \\
                                                                                                     &                               &                                                                                                                                                                \\
GeForce GTX 580 (Fermi)                                                                              & GeForce GTX 480               & Refreshed                                                                                                                                                      \\
GeForce GT 740 (Kepler GK107)                                                                        & GeForce GT630                 & Refreshed                                                                                                                                                      \\
Radeon R7 260, Radeon R7 260X                                                                        & Radeon HD 7790                & Refreshed                                                                                                                                                      \\
Radeon R7 360                                                                                        & Radeon R7 260                 & Refreshed                                                                                                                                                      \\
Radeon R7 370                                                                                        & Radeon R7 265                 & Refreshed                                                                                                                                                      \\
Radeon R9 380                                                                                        & Radeon R9 285                 & Refreshed                                                                                                                                                      \\
Radeon R9 390                                                                                        & Radeon R9 290                 & Refreshed                                                                                                                                                      \\
Radeon R9 390X                                                                                       & Radeon R9 290X                & Refreshed                                                                                                                                                      \\
Radeon RX 560 (Polaris 21)                                                                           & Radeon RX 460 (Polaris 11)    & Refreshed                                                                                                                                                      \\
Radeon RX 570                                                                                        & Radeon RX 470                 & Refreshed                                                                                                                                                      \\
Radeon RX 580                                                                                        & Radeon RX 480                 & Refreshed                                                                                                                                                      \\ \bottomrule
\end{tabular}
\end{table*}

==> relatedwork.tex <==
x\color{red}
\subsection{Semiconductor Supply Chain}

\newcommand{\comment}[1]{}

%need citation for the four stages and classification
At high level 
semiconductor supply chain 
consists of four principal stages: Wafer fabrication, Probe, Assembly, and Test, as shown in Figure~\ref{fig:ssc}-a. The wafer fabrication and the probe 
constitute the 
front-end operations 
whereas the assembly 
and test are generally categorized as the back-end operations 
of the semiconductor supply chain.

%need citation for the layer count and turnaround time on production
%tentative source: https://semiengineering.com/battling-fab-cycle-times/
%gives both per-layer manufacturing time and layer estimations
Consumer semiconductor products consist of millions to billions of transistors fabricated, connected and tested as a single unit. Wafer fabrication consists of up to 100 layers of material masked, etched and deposited on top of each other to create an intricate final product. With each layer taking around a day, this means that even the best fabricators have a manufacturing time on the order of several months. Additionally, a precondition for manufacturing is acquiring masks for etching features into the silicon wafer. These masks take over a week to manufacture and are taking even longer with each subsequent process node. The latest mask technology is extreme ultraviolet lithography or EUV; necessary for emerging process nodes, EUV machinery is only produced by a single company in the Netherlands, adding further complications if a machine breaks down or more machines are necessary.

%comment out first stage description to write my own-JAD
\comment{
The CMOS (Complementary Metal Oxide Semiconductor) device 
is the basic building block of almost all the consumer semiconductor 
products such as integrated circuits, microprocessors, memories etc. 
Semiconductor manufacturing activity actually involves the fabrication of 
billions of transistors and connecting them together to make an integrated circuit. 
The front-end of
the fabrication process of an integrated circuit involves, building
layers of different materials with varying electrical characteristics 
on top of a semiconductor (usually silicon but sometimes gallium arsenide or indium 
phosphide) wafer. 
The layer fabrication process starts with doping, which basically means the introduction 
of impurities into a semiconductor crystal to change it's electrical characteristics. 
Boron, phosphorus, aluminum, indium, arsenic and antimony are most commonly used 
dopants in the CMOS manufacturing. From manufacturing point of view doping process 
involves thermal processing to ensure the diffusion of the dopants into the semiconductor
layer then unwanted materials are removed by etching and a dielectric is deposited 
to electrically isolate the consecutive layers. 
Even at the modest capacity CMOS manufacturing process, upto forty layers of 
materials can be deposited on top of each other with dielectric layers in between them,
in the manufacturing cycle time of orders of 10-15 weeks.}

%stage two, probing
%also leads into a discussion of binning as the process starts here
With the wafers manufactured, the devices on a wafer are then probed for functionality. Devices can be functional, non-functional or partially functional. A partially functional device is one that, through imperfections in the wafer and fabrication process, fails to meet the desired specifications but can meet a lesser set of specifications. For an example of partial functionality, imperfections may result in a lower maximum frequency, reduced cache size or a reduction in core count for a processor. To make the most of these inevitable imperfections, the technique of binning is commonly used. Manufacturers lay out a series of ``bins" ordered from highest to lowest specifications. Manufactured dies are then sorted into the best possible bin on the basis of their probed characteristics.

%commented out stage two to write my own-JAD
\comment{
In the second phase of the front-end operations
the CMOS devices on a wafer are electrically probed and classified as fully, partially or
non-functional devices. }

%this is fairly straightforward, only addition over Husnain is
%discussing the need to pair/cluster for designs of multiple 
%dies/packages
%need source for how long this process takes
In the back-end operations, the wafer is next diced into individual dies which are then packaged into ceramic or plastic for testing. In the case of a package containing multiple dies, the dies involved may be chosen from the same or similar bins to have as similar of characteristics as possible. The package is then run through a gauntlet of tests to ensure it is fully operational. This process takes on the order of two to three weeks.

%stage 3/4 commented out to write my own version-JAD
\comment{
In the back-end operations (assembly) the probed wafers are first diced to get 
individual 
CMOS devices which are then packaged into ceramic or plastic 
packages to protect them from the environment. 
Once assembled into packages the CMOS devices are then tested against rigorous 
consumer-specific tests. The cycle time for back-end operations takes orders of two 
to three weeks.}

%comment out this part on binning-JAD
\comment{
Semiconductor products may have alternative manufacturing routing both within or 
across wafer foundries, 
due to the rapid evolution of process technology and semiconductor products.
The evolution of process technology and equipment may result in 
alternative machines capable of processing same product steps  
e.g. the newer machines are usually 
capable of processing older semiconductor products while 
the older machines will not be able to meet the cutting edge specifications of the 
newer semiconductor products. 
The process of probing and final testing may identify some of the devices to work on more 
relaxed specifications than the designated specification e.g. a micorprocessor designed for 3GHz
may not be functional at 3GHz fmax and may still be functional at 2.6GHz fmax.
Hence the inventory of the higher grade products might be able to meet the 
requirements of the lower grade products but the vice versa will not be true. }



%new intro to BOM discussion
%this discussion should be redone as well, perhaps with a "real" example
%of BOM allowing multiple paths
\iffalse
As architectures can be comprised of many components or produced in different process nodes, there are many possible supply routes to a given demand. We represent this with a bill of materials (BOM) describing the alternative routes possible. This BOM needs to consider the bins, fabs, process node and associated manufacturing time among many other factors to lay out a path to the demanded semiconductors.
\comment{
Hence the decision to reach a specific end-product may have different routes where 
alternative components may be used. A bill of materials (BOM) describing all the alternative routes will 
need to consider binning, probing, alternative choices for machines/tools and the fabrication 
plant location etc. In this scenario} A decision made for a specific component may 
significantly affect the choice of components for the other semiconductor products on the list. 
The existence of alternative routes between supply and demand introduces combinatorial 
complexity in the decision making. We use 
a hypothetical semiconductor-BOM as an example to show the combinatorial complexity of decision 
making to match
supply to demand
(Figure~\ref{fig:ssc}-b). 
Let's assume hypothetical semiconductor parts P1 to P6, where part P1 bins into P2, P3 and P4 with
probabilities 20\%, 30\% and 50\%, respectively.
Dotted line in Figure~\ref{fig:ssc}-b indicate that the part P3 can substitute for parts P2 and P4
while P2 can only 
substitute for part P3.
In our example semiconductor-BOM the part P5 can be manufactured using part P3 or P4
while the part P6 can be manufactured using P2, P3 or P4.
Since there exist alternative routes to match supply to demand and each stage can also 
share tools or use alternative tools the combinatorial complexity of the problem 
is evident from the Figure~\ref{fig:ssc}-b.  
\fi

\begin{figure}[htbp]
  \centering
    \subfloat[\centering Manufacturing stages]{
        {\includegraphics[width=0.48\linewidth]{./images/process.png}}
    }
    \subfloat[\centering A hypothetical BOM]{
        {\includegraphics[width=0.48\linewidth,height=0.43\linewidth]{./images/bom.png}}
    }
    \caption{\small Semiconductor Supply Chain}
  \label{fig:ssc}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{./images/matrix.png}
    \caption{Semiconductor Sypply Chain Planning Matrix}
    \label{fig:matrix}
\end{figure}

%this part on management functions seems entirely unnecessary
%especially since it may not even be that accurate to semiconductors
%i.e. the months-long manufacturing and fast-paced market w/demand 
%fluctuations means that the short (and maybe medium) term
%is far more agile here than in the real-world of semiconductors
%
%so it is commented out-JAD
\comment{
An example semiconductor supply chain management matrix 
%modified to reflect semiconductor supply chain 
is shown in Figure~\ref{fig:matrix}. 
The matrix consists of planning functions tailored to depict semiconductor 
supply chain management at a high level. 
The decisions made inside each planning functions, may act 
as inputs for other planning functions. 
The vertical axis of the semiconductor supply chain management matrix (Figure~\ref{fig:matrix}) 
shows the time frame whereas the 
material flow  
across various business functions is represented along the horizontal axis. 
The time frame is categorized into three categories the long-term, the mid-term and the 
short-term time frames. 
The strategic network planning takes place for the long term time frame 
across all the business functions of the semiconductor supply chain. 
The main goal of the strategic network planning function is to make decisions 
about 1) the products to produce, 2) the markets to target and 3) the location/sizes of the 
production facilities to build (semiconductor fabrication facilities in our case).
The second major function of the semiconductor supply chain management matrix is 
demand planning, it is responsible for developing demand forecasts for
long-term strategic network planning function as well as short-term master planning function. 
The master planning function is responsible for 
coordinating the material flow over the semiconductor supply chain.
It takes the decisions of strategic networks planning function 
as input 
correlates them with the 
alternative manufacturing processes and BOMs
to generates a time phased plan 
which specifies the quantity of each product or product family 
to be produced in different fabrication facilities. 
The aggregation in Master Planning function can vary from the semiconductor resource and product 
family level to individual product level. 
The Master Planning function handles seasonal demand fluctuations by 
building inventories ahead of peak demand periods, outsourcing or delaying product demand.
After the Master Planning has finished generating production targets 
for production facility, the Production Planning gets the capacity feasible release plan 
and release it to the production facilities. 
The progress of each semiconductor production facilities is controlled by it's internal 
scheduling function. 
On the mid-term and short-term time frames the demand planning function also generates 
the inputs for the Master Planning function which then 
manages the Procurement, Production and Distribution functions accordingly. 
One of the important aspect of the semiconductor supply chain is that, 
the Master Planning function must consider alternate sources of inputs for different items across 
the supply chain, 
while Production Planning function must consider alternative process routings 
within the individual manufacturing facilities. 
Hence, the Master Planning and Production Planning functions also often address significant 
elements of the Material Requirements Planning function. 
Hence, specifically for semiconductor supply chain management 
the Master Planning function often incorporates some of the 
functionality allocated to Production Planning and Inventory Management functions 
in other industries. 
The Capacity Planning function in semiconductor supply chains takes place 
between the time scale of 
Strategic Network Planning and Master Planning function as the
time for purchasing new production equipment can easily exceed six months. 
In the medium-term time frame the Master Planning function is 
used to determine the estimated availability of
material for projected or realised customer demands, which is also called Available to 
Promise (ATP) quantities, 
The Demand Fulfilment function is responsible to allocate the available material to customer
orders in the short-term time frame by allocating the available ATP quantities to individual 
customers or orders. 
The 
existing inventories can be also be reallocated 
between different end products, due to the availability of 
random co-production capabilities,
this makes the semiconductor supply chain even more complex, as the particular product
demand can be met via alternative means.
}


\subsection{Challenges in Semiconductor Supply Chain}
Some of the important characteristics of the semiconductor products and the semiconductor manufacturing process 
that directly impact the semiconductor supply chain are 
1) Strong economies of scale,
2) Pervasive uncertainty throughout the supply chain,
3) Short product life cycles and
4) Global nature of the semiconductor industry.
\subsubsection{Strong economies of scale}
Due to the extremely capital intensive nature of 
semiconductor production facilities 
the semiconductor supply chains exhibit strong economies of scale.
The complex equipment used in the semiconductor production has very high 
development cost as it works at the intersection of electrical, mechanical and chemical subsystems.
Especially, for the latest semiconductor technologies, the equipment is usually in the 
research and development phase is not optimized for 
maintainability and reliability. 
These challenges with the latest semiconductor equipment 
increase the operational uncertainty within production facilities. 
Moreover, the semiconductor fabrication facilities require a cleanroom environment with very strict air quality 
maintenance requirements. 
The equipment used to maintain the air quality standards of the cleanrooms is extremely expensive to build and maintain. 
The complexity of the semiconductor products is increasing with time, hence the device probe and test stations 
require sophisticated equipment which adds to the over all cost of the fabrication facility. 
Maintaining the workforce of highly skilled engineers, technicians, and 
scientists even during
industry downturns imposes substantial fixed costs to the semiconductor production. 

\subsubsection{Pervasive uncertainty throughout the supply chain}
The uncertainty in the overall yield of the semiconductor process 
is a critical concern for the semiconductor industry. 
Although there has been a lot of research in increasing the yield of the semiconductor manufacturing process, 
the overall yield of the semiconductor process still varies significantly 
over time, across facilities and across different semiconductor manufacturing technologies and products. 
The main reasons behind the uncertainties of overall semiconductor yield are the 
the complexity of the production processes and the often incomplete understanding of the underlying science.

\subsubsection{Short product life cycles}
The semiconductor products have relatively short life cycles due to the competitive nature of semiconductor industry. 
The continuous introduction of newer processes and products, with enhanced functionalities 
and/or lower costs, is necessary to 
stay competitive in the semiconductor industry.
The yield of the semiconductor manufacturing is at its worst when the latest 
semiconductor technology (tech. node) or products are introduced for high production volume, as the 
newer processes/products might not be ready for mass manufacturing. 
The uncertainties associated with both product and process introductions motivate
the need for innovative solutions. E.g. Intel’s well-known ‘tick-tock’ approach, where product and 
process introductions never take place simultaneously, was targeted to mitigate the uncertainties 
associated with the semiconductor product and process introductions. 
Existing research works ~\cite{Leachman1996}, ~\cite{Iansiti2000}, and ~\cite{SalomonandMartin2008}
present empirical evidences that effective management of the introduction of new products into high-volume 
manufacturing provides significant competitive advantage. 
The continuous introduction of new products/processes results in small amount of time for debugging/learning 
process specific methods 
to improve the overall yields. 
Moreover, the product prices decrease sharply over the product's already short life cycle.
The impact of short life cycle of semiconductor process/product, on the 
product price and process yield uncertainties, have special implications 
for firms that target commodity
products (such as DRAM), as lower product prices and scheduled product deliveries are critical for these firms. 
Whereas, the firms competing on innovation are also severely impacted by the short life cycles of 
semiconductor products, 
as the competitors may first introduce improved
semiconductor process technology, enhanced products 
or may offer lower prices for products with similar specifications. 
The latest products may not be backward compatible with the older circuit boards, in this case 
additional delays may be introduced 
in the supply chain as the electronics firms might have to upgrade their circuit boards to support 
latest semiconductor products. 

\subsubsection{Global nature of the semiconductor industry}
In the early days of the semiconductor industry 
the probe, assembly, and test operations were largely manual, 
and were heavily labour intensive. 
In order to reduce the overall cost of the semiconductor device, it was extremely 
critical to have access to cheap labour and low-cost manufacturing locations.
Hence, in early 1970s many European and US firms established semiconductor manufacturing facilities in 
the countries that had cheap labour e.g. South Asia and eastern Europe.  
Historically, governments viewed the semiconductor industry as an important component of their national economies. 
The governments of countries like Japan, South Korea, Taiwan and more recently
China have provided considerable support for the development of semiconductor manufacturing facilities in their 
respective countries. 
Hence the semiconductor supply chains are distributed across the globe as 
the manufacturing facilities are in different countries with differing tax laws, import controls and 
local content regulations.
Historically, semiconductor supply chain industry has focused on 
vertically integration where manufacturing firms 
focus on performing all the four stages of 
the semiconductor manufacturing (Figure~\ref{fig:ssc}-a) themselves. 
In recent years the focus of semiconductor manufacturing industry 
has started to shift to vertical disintegration strategy.
In vertical disintegration some firms focus on specialising in
particular stages of the semiconductor manufacturing and outsource other operations 
to the relevant specialized firms. 
Outsourcing 
certain manufacturing stages 
allows firms to mitigate/avoid the risks associated with building extremely expensive
production facilities in the face of uncertain demands. 
Recently, variations of fabless supply chains have 
started to appear where some firms 
outsource all the
semiconductor manufacturing operations, 
others outsource all or some of the front-end operations and perform the remaining
back-end operations themselves.
Contractual arrangements are needed between the firms to seamlessly regulate the operation outsourcing. 
Many virtual firms regulate these contractual agreements and become part of the
semiconductor supply chains.
Different supply chains can also be categorized into the following
two distinctive categories based on the mode of operation of the corresponding manufacturing firms
\begin{itemize}
    \item Make to stock (MTS) mode
    \item Make to order (MTO) mode.
\end{itemize}

Firms that focus on the mass production of commodity products (microprocessors, DRAM, flash memory etc) 
generally operate in MTS mode. 
Whereas, the firms that varying quantities of semiconductor products and target 
a wide range of customers 
generally operate in MTO mode.
Many firms operate in an intermediate mode, where 
some demands are stabilized to some extent by the contractual agreements with certain 
customers, whereas some demand is highly uncertain. 
For the firms that do not target the high-volume commodity manufacturing and want
to operate in MTS mode, 
a common strategy is to maintain a significant inventory of probed die (die-bank inventory),
between the wafer probe and assembly stages. 
This strategy will help in avoiding the long cycle times of the wafer fabs, as
the customisation usually takes place in assembly and test operations.  
The probed wafers can be pulled from die-bank inventory and processed rapidly through final
test for delivery. 

\subsection{Supply Chain Resilience}
Supply chain resilience (SCRES) can be defined as 
"The adaptive capability of a supply chain to prepare for and/or respond to disruptions, to make a
timely and cost effective recovery, and therefore progress to a post-disruption state of
operations – ideally, a better state than prior to the disruption." ~\cite{}

\iffalse
Hence, SCRES strategies 
aim to endure that the following four aspects
are maximised in a timely way and at minimum cost
\begin{itemize}
\item Preparation for a disruptive event; 
\item Response to an event; 
\item Recovery from the event; and, 
\item Growth/competitive advantage after the event. 
\end{itemize}
A supply chain is considered to be adaptive if it 
has a latent ability to develop
different responses to match the nature of the threats it faces.
I.e. instead of selecting response from a set of pre-existing responses, 
an adaptive supply chain has the capability to change its elements and generate an appropriate 
response towards a disruptive event.
The supply chain disruptive events may be unforeseeable or 
inherent to the supply chain, an adaptive supply chain has the 
capability to reflect the nature of these disruptive events. 
Moreover, an adaptive supply chain may learn from the disruptive events over time and develop 
new capabilities that may make it more resilience to similar threats in the future. 

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{./images/scres.png}
    \caption{Different events of supply chain resilience.}
    \label{fig:scres}
\end{figure}
The four main aspects of SCRES are illustrated in Figure~\ref{fig:scres}. 
The x-axis of the figure shows time whereas the y-axis is the performance of the resilience process. 
Two different disruptive events occur at two different time periods, 
a bigger loss is incurred due to disruptive event A than disruptive event B, this might be due to the 
adaptive capabilities of the supply chain. 
The learning experience of the first disruptive event has helped the supply chain to 
recover faster when the second disruptive event hit.
P-o refers to the normal performance level before the disruptive event occurs, 
P-a is the acceptable minimum performance level below which operations are presumed to shut down,
P-b is the best outcomes anticipated after recovery,
P-w is the worst outcomes anticipated after recovery,
Td-a is the time when the first disruptive event begins,
Tr-a is the actual recovery time for the first disruptive event and 
T-a is the maximum acceptable recovery time for the first disruptive event.
One way to measure of the resilience of the supply chain is the area of the shaded region, 
it gives some measure of performance loss and the recovery time, it can also be extended to calculate the 
growth or shortfall. This is a static measure of the resilience of the supply chain. 
A more dynamic measure of the resilience would be to compare the response regions of 
different disruptive events over time, this can give a sense of the adaptive nature 
of the supply chain and show if supply chain is becoming more resilient over time. 
Although these approaches are useful, we should also take in acknowledge that 
measuring SCRES is partly subjective and context specific e.g. what constitutes an acceptable time
for recovery (T-a) may vary in different circumstances. 
\fi

The research on supply chain resilience has suggested that 
four key strategies for building SCRES include
1) Increasing the flexibility,
2) Creating redundancy,
3) Building collaborative supply chain relationships and 
4) Improving the agility of supply chain. 
Some of these are interrelated e.g. redundancy can aid flexibility. 
In the next subsections we will discuss these strategies in detail.

\subsubsection{Flexibility}
The supply chain flexibility is "the ability of an enterprise to adapt 
to the changing requirements of its environment and stakeholders 
with minimum time and effort"~\cite{}.
Postponement, a flexible supply base, flexible transportation, 
flexible labour arrangements and flexible order fulfilment 
are some of the most commonly used flexibility practices that can 
improve the resilience of the supply chain. 
E.g. if the postponement strategy is adopted during a crisis some of the 
demand will be deferred to the future time periods which will enhance the 
resilience of the supply chain. 
Flexibility actually enhances the adaptability of the enterprise 
which makes the enterprise more resilient to disruptions. 
The ability of an enterprise to flexibly adopt the alternative choices, such as 
alternative suppliers, transportation and labour resources,
during a crisis period will improve the response to the disruption and reduce 
the recovery time of the supply chain~\ref{fig:scres}.
The value of flexibility can be "priced" using  
extreme value theory. 
\subsubsection{Creating redundancy}
Redundancy can be defined as 
"the strategic and selective use of spare capacity and inventory that can be invoked 
during a crisis to cope, e.g. with supply shortages or demand surges." ~\cite{} 
A supply chain can be made more resilient 
by having a spare capacity along the critical path that might help to 
mitigate some of the potential vulnerabilities. 
But creating spare capacity and inventory along the critical path 
can be an expensive means of building resilient. 
In order to effectively use redundancy to build supply chain resilience, 
certain factors such as geographical location and the total demand should 
be considered. 
E.g. global events (e.g. an earthquake or flood) may impact all the suppliers that are in the 
close proximity along with their redundant inventories.
On the other hand if suppliers are geographically far apart and if one of them 
encounters a major disruptions the redundant inventories of other suppliers can chime in to 
mitigate the effect of this disruption on the global demand. 
As redundancy involves the duplication of resources, 
it actually increases flexibility as it facilitates response through an easily adaptable 
deployment of redundant resources.
Flexibly picking some of the redundant resources may help in mitigating some of the delays
which can improve the recovery time for some disruptive events.
Flexibility that does not rely on redundancy, rather is achieved by some other ways 
e.g. by employing a multi-skilled labour force, installing multi-purpose machines, creating flexible contractual
arrangements etc is usually preferred. 


\subsubsection{Supply chain collaboration} 
Supply chain collaboration is the ability to work effectively with
other entities for mutual benefit in areas such as forecasting, postponement and risk sharing. 
If the information about supply chain risks and uncertainties is shared between the collaborating 
entities, it may help 
to reduce uncertainty, increase transparency and facilitate the creation and sharing
of knowledge. 
The entities in the 
supply chain collaboration process can also 
share the cost of building security, resources and skills needed 
to recover from a disruptive event. 
The collaboration 
can also improve the performance of SCRES as the collaborating 
entities can share the SCRES knowledge base and resources to
come up with a flexible and 
coordinated response to disruptive events. 
When it comes to supply chain collaborations certain relationships such as just-in-time supply and 
single-sourcing supply partnerships, 
are usually the most vulnerable links that must be traded off against the benefits offered by those 
entities. 

\subsubsection{Supply chain agility}
Supply chain agility is the ability to respond quickly to unpredictable changes in
demand or supply. 
Supply chain agility is mainly composed of visibility and velocity. 
Where supply chain visibility is the ability to see through the entire supply chain to have a clear view,
which may help in detecting signals of impending disruptions.
Visibility can also help to avoid 
overreactions, unnecessary interventions and ineffective decisions in circumstances of risk.
Furthermore, a clear view of the entire supply chain may also
help the supply chain to effectively respond to and recover
from disruptions. E.g. visibility may help in identifying the vulnerable suppliers,
thereby allowing enough time to develop countermeasures against failures.
One way to strengthen the supply chain visibility can be by installing monitoring tools throughout the supply chain, 
so as to improve the threat
awareness and receive timely warnings of potential disruptions.
The second element of agility is the supply chain velocity. 
It focuses on the pace of flexible adaptations, and thus determines the recovery speed of the supply chain from a
risk event.
%\subsection{Conventional Approaches to Semiconductor Supply Chain 
%Resilience}

% \section{Architectural Interventions for Improving Supply Chain Resilience}
% \subsection{Composition}
% Composition is the process in which final demand goods are produced 
% by combining a set of input goods. 
% In this way, the supply and the demand chains are not tightly coupled/linked, 
% rather "de-linked" to some extent with the goal to improve the overall 
% resilience of the supply chain.
% Mathematically, composition can be treated as many-to-one mapping 
% problem as shown in Figure~\ref{fig:composition}-a. 

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{./images/composition.png}
%     \caption{Caption}
%     \label{fig:composition}
% \end{figure}
% A hypothetical example for composition is shown in figure~\ref{fig:composition}-a. 
% Where demand goods are labeled as D1, D2 and D3; and supplied goods are
% labeled as S1, S2, S3 and S4. 
% The arrows connecting the supplied goods to demand goods show the mapping 
% required to build the demand goods by the specific combination of supplied goods.
% As shown in figure~\ref{fig:composition}-a the demanded product D1 can be made 
% by combining the supplied goods S1, S2 and S3. 
% And product D3 can be made by combining a different subset of supplied goods 
% (S2, S3 and S4 in this hypothetical example). 
% Different supplied goods can also be used to different demand products e.g. in this 
% example S4 is used to build D2 and D3. 
% Mathematically this can be treated as many-to-one mapping problem with 
% selective optimization targets that may improve the resilience of the 
% supply chain.

% In the context of semiconductor hardware, the composition can be defined, 
% as the process in which instead of building bigger monolithic integrated circuits (chips),
% we build a set of smaller integrated circuits (chiplets) and combine them
% together, using interconnects, to build the final product. 
% Composing a system from a set of smaller chiplets instead of a single monolithic 
% chip can help in improving the overall yield of the semiconductor manufacturing 
% due to multiple reasons 

% As discussed in section~\ref{sec:uncertainity}, 
% uncertainties in the overall yield is a critical component that 
% introduces uncertainty in semiconductor supply chain. 
% The semiconductor products have short life cycles~\ref{sec:lifecycles}, 
% newer products and processes are continuously introduced to meet the 
% competition of the market.
% As yield is at its worst for newer products/processes, 
% due to developing science of the newer processes and short debugging/learning time.
% The composition can help in decoupling the process and final demand products.  

% Moreover, building larger area monolithic systems would require cutting edge process nodes
% as it might not be possible to use older technology 
% nodes to build large area monolithic systems due to the reticle limit~\cite{}.
% As discussed earlier, the cutting edge process nodes are usually in the 
% early stages of development and are not resilient.
% Building the large systems as a combination of 
% smaller chiplets will allow us to use mixed/older technology nodes, which have established 
% science and are more resilient.
% This will not only improve the overall yield but also increase
% the overall flexibility and adaptability 
% of the semiconductor supply chain 
% as there are more choices for the technology node to pick from. 

% The cost/mm2 of the semiconductor dies is increasing as newer 
% technology nodes are being introduced. 
% The cost of $250mm^2$ die on 7nm process is $\approx 4\times$
% the cost on 45nm process and it's expected to continue to increases with 
% newer/smaller technology nodes.
% Hence building larger monolithic chiplets is increasingly becoming 
% less economical. 
% Breaking down monolithic systems to smaller chiplets considerably increases 
% the yield with minimum area penalty 
% ($>2\times$ increase in yield when a $360mm^2$ die is 
% broken down to 4-chiplet design with only $\approx 10\%$ area penalty ~\cite{}).
% ~\cite{}~\cite{} claim that 
% if critical processor components are partitioned into separate chiplets
% and integrated on highperformance interconnects
% it will not cause significant performance
% degradation (<5\%) compared to large area monolithic SoCs.

% As the cost negatively impacts the resilience of the supply chain, 
% the chiplet based designs will improve the 
% resilience of semiconductor supply chain with minimum performance degradation. 

% In summary, the composition strategy 
% can make the semiconductor supply chain 
% more flexible, more adaptable and more economical, 
% as discussed in section ~\ref{sec:} these are some of the key characteristics 
% to improve the resilience of the supply chain.
% And smart decisions made by 
% architects for building heterogeneous end products 
% by smart combination of chiplets can 
% directly impact the resilience of the semiconductor 
% supply chain. 


% \subsection{Adaptation}

% The adaptation is the process in which the supplied goods 
% can be adapted to meet the requirements of several demanded goods.
% Like composition, adaptation also decouples the supplied goods from 
% demanded goods with the potential to improve the overall 
% resilience of the supply chain.
% Mathematically, adaptation can be treated as one-to-many mapping 
% problem from supply to demand, as shown in Figure~\ref{fig:composition}-b. 

% A hypothetical example for adaptation is shown in figure~\ref{fig:composition}-b. 
% Where demand goods are labeled as D1 and D2; and the supplied goods are
% labeled as S1 and S2.
% The arrows connecting the 
% supplied goods to the demanded goods show the adaptation capability of the 
% supplied goods. 
% As shown in figure~\ref{fig:composition}-b 
% the supplied good S1 can be adapted to 
% meet the demands of D1, D2 and D3 and 
% the supplied good S2 can be adapted to 
% meet the demands of D4 and D5.
% Mathematically this can be treated as one-to-many mapping problem that can be 
% optimized with the goal to improve the overall resilience of the 
% supply chain. 

% In the context of semiconductor hardware, the adaptation can be defined, 
% as the process in which
% the supplied hardware can be adapted to target the specifications 
% of more than one demand products. 
% One way to achieve adaptation is to use the programmable or 
% reconfigurable hardware, 
% instead of fixed function hardware. 
% If the we consider our demand as applications, we can either design 
% application specific integrated circuits (ASICS)
% to target those applications or use programmable 
% such as FPGA (Field Programmable Gate Arrays) and 
% programmable network devices (Switches, smart NICs) hardware.
% Designing programmable hardware that can adapt to 
% different demand requirements can improve the flexibility of the 
% semiconductor supply chain and makes the supply chain less prune to disruptions, which 
% will make the semiconductor supply chain more resilient to disruptions. 
% Moreover, the programmable hardware can be mass produces as commodity 
% product, which reduces the cost of hardware and in tern make the 
% supoply chain more resilient. 

% Adaptation in the semiconductor supply chain can also be achieved by binning
% the hardware. 
% Binning is the the process of categorizing the hardware components
% by their quality and performance. 
% The semiconductor components, such as microprocessors, GPUs, CPUs, RAMs etc,
% are designed for certain performance specifications but sometimes they fall short 
% to meet those specifications due to the complexities of the 
% semiconductor manufacturing process.
% One example of binning can be, if a four core Intel i5 processor fails to meet the 
% required power specifications, they might disable two of it's cores and 
% bin it as two core i3 processor ~\cite{binexample}. 
% Adaptation of the hardware that doesn't meet the strict specification 
% of higher end products by binning to lower end products 
% can reduce the effective overall cost 
% and improve the effective overall yield. 
% The lower cost and higher yield translate to improvement in the 
% resilience of the semiconductor supply chain. 
% Architects can also use voltage/frequency scaling (VFS) to design adaptable hardware. 
% Demand hardware may have varying performance and energy efficiency requirements based on the workloads that 
% its supposed to target.  
% Architects can use voltage/frequency scaling (VFS)
% techniques to adapt the supplied hardware according to the performance 
% and energy efficiency requirements of the demand hardware~\cite{onlineVFS}.
% This will introduce flexibility in the supply chain and intern make it more resilient. 

% Rebadging/rebranding and refreshing
% techniques 
% can also be used to make the hardware more adaptable. 
% In semiconductor hardware context rebadging/rebranding 
% is the process of taking the older products, preferably from previous
% generations, and selling them by changing their names. 
% In rebadging/rebranding
% process, certain hardware features can be enabled or disabled or clock 
% speed changes may be applied but the core architecture and the 
% chip remain the same. 
% E.g. Apple's A12Z Bionic Chip (2020-iPad-Pro) is a rebadged 
% A12X Bionic with an enabled GPU core. 
% Whereas, a "refresh" is 
% the techniques in which minor enhancements are 
% applied to improve the performance and/or efficiency of the chip.
% E.g. the AMD Radeon-RX-500 series is a refresh of the older 
% AMD Radeon-RX-400 series where both series use Polaris GPU 
% architecture~\ref{refreshlist}.
% Rebadging/rebranding and refresh may make the hardware adapt to 
% different demand requirements. 

% If architects design the hardware to be adaptable then, 
% in the case of a disruptive event if the manufacturing of certain low-end hardware product is 
% affected, then certain features of high-end hardware can be disabled to make it meet the 
% specifications of the disruptive low-end product. Industry commonly uses rebadging to sell hardware 
% under different product specifications, many examples of rebadging are presented in Table~\ref{tab:rebadging}.
% %\input{./texFiles/rebadgingTable}
% Rebadging usually cuts the 
% overall cost of the semiconductor product and increase its life-cycle, 
% as new chip design and architecture cost money, resources and time.
% Lower cost and improved life-cycle of the product aid in 
% improving the resilience of the semiconductor supply chain.
% which improves the resilience of the semiconductor supply chain.
% Rebadging increases the flexibility of the semiconductor supply chain, which improves 
% the resilience of the supply chain.


% \subsection{Commoditization}

% The commoditization is the process in which final demand goods are produced 
% by combining a set of commodity supplied goods. 
% Commoditization also decouples the supply and demand 
% to some extent with the goal to improve the overall 
% resilience of the supply chain.
% Mathematically, commoditization can be treated as 
% one-to-many mapping from demand to supply.
% A hypothetical example for commoditization is shown in figure~\ref{fig:composition}-c. 
% Where demand goods are labeled as D1 and D2; and 
% commodity supplied goods are
% labeled as S1, S2, S3 and S4. 
% The arrows connecting the demand goods to the commodity supplied goods show the mapping 
% required to build the demand goods by the specific combination of commodity goods.
% As shown in figure~\ref{fig:composition}-c the demand D1 can be met 
% by the commodity products S1, S2 and S3.
% And the demand D2 can be met 
% by the commodity products S2 and S3.
% Mathematically this can be treated as one-to-many mapping problem from demand to supply 
% with selective optimization targets that may improve the resilience of the 
% supply chain.

% In the context of semiconductor hardware, the commoditization can be defined, 
% as the process in which
% the final demand architecture is build by 
% selecting commodity products and connecting them together 
% according to the demand specifications. 
% The commodity products can be commercial chiplets that are mass produced 
% by commodity firms and can be connected using interconnects to meet the 
% final specifications of the demand architecture. 
% Building an architecture by connecting a set of commodity chiplets 
% can improve the resilience of the semiconductor supply chain in many ways. 

% Architects have the choice to pick mixed process nodes, instead of only using the 
% cutting edge process nodes to build the final demand architecture. 
% Cutting edge process nodes usually have lower yield and have 
% higher cost/mm2 ~\ref{sec:composition}. 

% Older process nodes usually have higher yield and lower cost/mm2 and 
% architects can quantify the PPA (performance, power and area) penalties 
% of different architectural choices.
% Architects can do a design space exploration to study the impacts 
% of picking different mixed process based commodity chiplets on the overall 
% cost and yield, with the goal to find the sweet spots that meet the 
% specifications of the demand architecture with minimum cost and maximum yield. 
% As discussed in section~\ref{sec:} the cost minimization and yield maximization 
% can make the supply chain more resilient. 

% There are many commodity firms that mass produce commodity 
% chiplets for DRAM and flash memory, which are usually build 
% using well established older technology nodes and have high yields. 
% Architects can 
% design memory heavy demand architectures to maximize the use of these commodity
% memory chiplets. Such architectural decisions can maximize the yield, minimize the 
% cost and improve the resilience of the semiconductor supply chain. 

% Commoditization creates redundancy 
% in terms of supplied goods 
% as a large redundant inventory of commodity supplied goods 
% can be procured 
% from different commodity firms. 
% The redundancy, created by commoditization, can 
% make supply chain more resilient to disruptive event e.g. if a 
% disruptive event ceases the operation of one or two manufacturing firm 
% 1) either redundant inventory can be used to respond 
% to this disruptive event and/or 2) 

% Commoditization promotes 
% supply chain collaboration 
% by providing many potential suppliers
% as there are many commodity firms. 
% As discussed in section~\ref{sec:} supply chain collaboration 
% makes the supply chain more resilient to disruptive events. 
% E.g. when a disruptive event causes some manufacturing unit to cease operations 
% the collaboration approach gives the supply chain the flexibility 
% to respond to the disruptive event by picking a different commodity supplier.  

% Commoditization also improves the flexibility and overall adaptability
% of the supply chain due to the availability of the large number of choices for 
% commodity suppliers and commodity goods.

\color{black}

\let\comment\undefined


==> results.tex <==
\section{Results}
\label{sec:results}

Here we present results on total cost under several regimes of uncertainty.  
We use box plots which annotate minimum, maximum, first
quartile, third quartile, and median points of non-outlier data using solid
black bars; outliers are explicitly annotated (black diamonds).
Some charts also give the `wait-and-see'
objective---the expected total cost assuming all decision variables have
recourse to both supply and demand uncertainty---using a horizontal green bar.
%The wait-and-see objective is strictly no worse than the expected total cost,
%but outliers can and do beat the wait-and-see objective (as the wait-and-see
%objective is an expectation).
A white square represents the expected total
cost of the boxplot distributions, whereas a green diamond represents expected
total cost when interventions are not used. 
Optimal chip ordering policies are depicted with pie charts above box plots.
%\footnote{In some cases, such as
%certain dispersion results, where the ratio between chips in the optimal order
%policy is dictated by constraints, the pie charts are omitted.} 
Unless otherwise stated, blue represents 16-core chips, green represents 8-core
chips, gold represents 4-core chips, and red represents interposers.
The y-axis of the graphs is the total cost, $TC$.  As such, lower is better,
and corresponds to higher profits.


\subsection{Fragility of Supply Chains}

We first demonstrate the fragility of supply chains to disruptions due to single paths between produced and demanded chips.
%\iffalse
First consider whether market and supply chain uncertainties impact profits.
Figure~\ref{fig:supplydemanddisruption0} shows total cost distributions in a
market where quantities of 16, 8, and 4 core chips are demanded.  Demand and
supply disruption are modeled as scaling factors impacting quantities demanded
and yield, respectively.  If a firm produces exactly what it assumes will be
demanded, it is highly susceptible to both supply and demand disruptions.
Subfigures~\ref{subfig:sd0d} and \ref{subfig:sd0e} show total cost sensitivity
to demand and supply uncertainty in a market for 16-core chips.  As demand
uncertainty increases, interquartile range increases from $0$ to over
$5\times 10^6$. Significantly, there is a large jump in interquartile distance
when variance increases from $0$ to $0.007$.  Even a small variance in demand
and supply uncertainty yields a large jump in variance in total cost.
Surprisingly, even mean and median total cost increases. This is due to
shortage cost driving increasing order sizes (10\% for demand disruption, 27\%
for supply disruption) in optimal order policies. This shows that uncertainty
in production and in the market have major impact on both uncertainty for total
cost, and expected profitability, when there is one-to-one correspondence between produced chips and demanded chips.
Note that in Subfigure~\ref{subfig:sd0d}, the minimum and median values
are the same. This is because 1) supply is deterministic, and 2) it is better
to have overages than shortages due to shortage costs.  Thus, the optimal policy
is one in which the ordered supply is large enough to satisfy demand with
probability $\geq 0.5$.
%}
%Subfigures~\ref{subfig:sd0d} and~\ref{subfig:sd0e} show distributions with
%monotonically increasing mean and variance, which shows that as market and
%supply chain uncertainties grow, profits shrink, and cost uncertainties rise.

\iffalse
For reasons like political instability, embargoes, natural disasters, and
market competition, it may not be possible to order the desired quantities of a
chip.  
\fi
Figure~\ref{fig:none1} considers a market with demand for 16-core,
8-core, and 4-core processors. The
`Supply Constraint Factor', $s$, represents an additional constraint imposed on
the optimization program, which requires the number of ordered chips of each
type to not exceed $x\cdot s$, where $x$ is the number ordered in an
unconstrained optimization. The box plots show the distribution of total cost
for various values of $s$. The results show that  supply shortages, modeled as
supply constraints, can have large impact on total cost distributions. 

Both supply and demand may also be subject to \textit{shocks}, where the supply
or demand changes greatly.  
%Supply shocks can arise for the same reasons as
%supply constraints (e.g., political instability), but can also be due to
%technical reasons (e.g., a design bug is not identified until post silicon test
%and validation).  
Figure~\ref{fig:none-shock} models supply and demand shocks
using discrete random variables.  With probability `Supply Shock Factor', $s$,
the supply/demand for a good becomes zero. Not only do supply and demand shocks
greatly increase expected total cost (dually, greatly reduce expected profit),
they also lead to a large increase in total cost variance, reducing
predictability and increasing risk of extreme losses.
Of particular note is that supply and demand shocks cause nearly orthogonal
losses.  At $s = 0.5$, The loss caused by supply and demand shock is $84\%$ of the
sum of the losses caused by supply shock and demand shock alone.
\iffalse
Having demonstrated that a policy of building exactly the chips demanded is
susceptible to supply chain and market uncertainties (resulting in reduced
profit and total cost uncertainties), we now ask how effective interventions
are at reducing cost uncertainties and mitigating profit losses.
\fi

% TODO: Build tri-subfig main figure showing importance of intermediate layer

\begin{figure}[ht] %[htbp]
    \captionsetup[subfloat]{farskip=0pt,captionskip=-1pt,nearskip=-4pt}
  \centering
     \subfloat[\centering Sensitivity to demand variance]{
        {\includegraphics[width=0.75\linewidth]{./images/distribution/Figure6d.png}}
        \label{subfig:sd0d} 
    }

    \subfloat[\centering Sensitivity to supply variance]{
        {\includegraphics[width=0.75\linewidth]{./images/distribution/Figure6e.png}}
        \label{subfig:sd0e} 
    }
    \caption{\small Producing exactly the demanded goods is vulnerable to
    supply and demand disruptions.}
  \label{fig:supplydemanddisruption0}
\end{figure}


\begin{figure}[ht]
    \centering
    \captionsetup{skip=0pt}
    \includegraphics[width=0.75\linewidth]{./images/distribution/NoneSupplyConstrainedWithBaseline.png}
    \caption{\small Producing exactly the demanded goods is vulnerable to
    supply shortages.}
    \label{fig:none1}
\end{figure}

\begin{figure*}[ht]
    \centering
    \captionsetup[subfloat]{captionskip=-2pt,nearskip=-4pt}
     \subfloat[\centering Demand shock]{
        {\includegraphics[width=0.25\linewidth]{./images/distribution/NoneShockA.png}}
        \label{subfig:nsA} 
    } \qquad
    \subfloat[\centering Supply shock]{
        {\includegraphics[width=0.25\linewidth]{./images/distribution/NoneShockB.png}}
        \label{subfig:nsB} 
    }\qquad
    \subfloat[\centering Supply and demand shock]{
        {\includegraphics[width=0.25\linewidth]{./images/distribution/NoneShockC.png}}
        \label{subfig:nsC} 
    }
    \caption{\small Producing exactly the demanded goods is vulnerable to 
                    supply and demand shocks.}
    \label{fig:none-shock}
\end{figure*}

\subsection{Benefit of Architectural Interventions}


% Figure~\ref{fig:baselines} show that composition and adaptation can reduce
% cost (maximize profit) when supply and/or demand disruptions exist.
% The studied regime is a market for 16 and 8 core processors.  Adaptation
% enables selling 16 core chips as 8 core chips, while composition enables
% combining two 8 core chips into a single 16 core chip (with additional
% interposer costs).  Composition is a highly effective intervention,
% resulting in a 23\% increase in expected profit when both supply and demand
% disruption are present.  Adaptation is marginally effective in the presence of
% independent supply and demand disruption.  Later, we show that the effectiveness
% of adaptation is correlated with correlations in supply and demand disruptions.

% TODO: Add dispersion to this graph
% TODO: Also explore with different default values
% TODO: Get rid of 'Scenario'
% TODO: Either full names (Adaptation) or just 'A'
% TODO: Show mean, as well.
% \begin{figure*} %[htbp]
%   \centering
%     \subfloat[\centering Demand disruption]{
%         {\includegraphics[width=0.33\textwidth]{./images/distribution/BaselineA.png}}
%     }
%     \subfloat[\centering Supply disruption]{
%         {\includegraphics[width=0.33\textwidth]{./images/distribution/BaselineB.png}}
%     }
%       \subfloat[\centering Supply and demand disruptions]{
%         {\includegraphics[width=0.33\textwidth]{./images/distribution/BaselineC.png}}
%     }
%     \caption{\small Adaptation and Composition reduce cost in the presence
%     of supply and demand disruptions.}
%   \label{fig:baselines}
% \end{figure*}

\subsubsection{Composition}
Composition includes benefits from disaggregation---integrating multiple
chiplets into a single chip---and from having several paths to creating a
demand good.  Since economic benefits of disaggregation are widely
known~\cite{amdnext}, let us try to isolate the benefits of multiple paths.

Figure~\ref{fig:composition1} models a market for 16-core processors. In the
base case, this demand is met by packaging four 4-core chiplets into a 16-core
system.  Composition enables \textit{multiple paths} to  16-core, including
building monolithic 16-cores and by packaging 8-core and 4-core chiplets. In
the ideal case, the optimal policy is to order a set number, $x$, of 4-core
chiplets, as the increased yield from disaggregation more than offsets the
increased packaging costs. This baseline isolates the benefits from composition
associated with enabling multiple paths from the (substantial) benefits
associated with disaggregation.  The `Supply Constraint Factor', $s$, is an
additional constraint, which requires the number of ordered 4-core chiplets to
not exceed $x\cdot s$.

The box plots show the distribution of total cost for various values of $s$
when composition enables multiple paths to the 16-core demand good.
For all values of $s$, many paths yield positive expected
profits, whereas expected profits are positive only for values of $s > 0.55$
when only a single path exists. Multiple paths enable higher profit for all values $s
<0.9$. Thus, we see the importance of multiple routes to meet demand in the
presence of supply uncertainty. 

\begin{figure}[ht]
  \centering
  \captionsetup{skip=0pt}
    \includegraphics[width=0.75\linewidth]{./images/distribution/CompositionSupplyConstrainedWithBaseline.png}
    \caption{\small Composition's impact on a supply constrained market.
    Green diamonds represent expected total cost without interventions.
    The Supply Constraint factor limits the number of available 4-core processors available
    to a fraction of the optimal, unconstrained order policy.
    The smaller the factor, the fewer the 4-core chips available.
    By using both 8-core chips and 4-core chips, composition
    effectively mitigates the losses of the baseline (green diamonds).
 }
  \label{fig:composition1}
\end{figure}

At $s = 0.00$, all chip production gets shifted to 8-core chips (green).
Beginning at $s = 0.20$, a mixture of 8-core and 4-core chips (gold) are used.
For $s \geq 0.90$, only 4-core chips are procured, as the benefits of
additional 8-core chips does not offset the increased NRE of designing and
building two different chips.

\begin{recom}
In a supply-constrained world, architects should create multiple versions of their design (each with a different level of disaggregation, for example). This allows the  demand to be satisfied even when supply of some constituents is constrained.
\end{recom}

Figure~\ref{sfig:interposer} shows the sensitivity of total
cost to a supply constraint on interposers in a market for 16-core chips
using composition.
As the supply constraint increases,
expected profit falls by 18\%, suggesting that interposer supply issues can
significantly impact profit rates.  Also of concern is the increase in total
cost variability.  Variance of total cost more than doubles, increasing by
107\%, driven largely by an increase in the number of outliers.
%Interposer costs are assumed to scale proportionally with chip area, and are
%invariant with respect to number of chiplets.
When interposer constraints are severe, the expected profit optimizing policy
is to build only monolithic 16-core chips (blue).
As interposers (red) become available, the 
orders for monolithic cores shrink, until none are ordered when interposers
reach 75\% of desired availability.

\begin{figure}[ht]
  \centering
  \captionsetup{skip=0pt}
        {\includegraphics[width=0.75\linewidth]{./images/distribution/Figure8c.png}}
    \caption{\small Sensitivity to interposer supply constraints.
    The Supply Constraint factor limits the number of interposers available to a
    fraction of the the optimal, unconstrained order policy.  The smaller the factor,
	the fewer the interposers available.
    }
    \label{sfig:interposer}
\end{figure}

\begin{recom}
Unless the interposer shortages are extreme, architects should continue to prefer disaggregated designs since the cost benefits from such design is simply too high. For extreme interposer shortages, 
a monolithic architecture improves
%In the face of shortages for interposers, 
%or expected supply constraints at
%foundries or OSAT companies, 
%design and production of monolithic cores can
%significantly improve 
supply chain resilience. 
%Further, disaggregation is such an
%effective intervention, that even when interposer shortages are present,
%the optimal mixture of produced goods often includes chiplets and interposers.
\end{recom}

Figure~\ref{fig:composition-shock} shows the benefit of multiple paths enabled
by composition in a high-risk market for 16-core processors, again aiming to
isolate the benefits of multiple paths from the benefits of disaggregation. In
the baseline case (total costs represented by green diamonds), all demanded
processors are assembled from 4-core chiplets.  Here, there is no constraint on
the number of 4-core chips which may be ordered, but demand of 16-core chips~(\ref{
sfig:composition-shock-a},
\ref{ sfig:composition-shock-c}) and supply
(\ref{ sfig:composition-shock-b}, \ref{ sfig:composition-shock-c})
of four core chips are modeled
as discrete random variables, with a `Shock Factor', $s$.  With probability
$s$, demand (supply) for a given demanded (supplied) good drops to zero. The multiple
paths from composition cannot effectively deal with demand shock, as multiple
paths cannot increase sales when the there is no demand for the good at all.
Multiple paths are, however, highly effective for supply shock.  At a shock
factor of $s=0.10$, the optimal policy begins to order 8-core chips, eschewing
the volatile supply of 4-core chips.

\begin{recom}
Architects should mitigate the risk of \emph{supply} shocks by independently
sourcing production of a diverse set of chips, of which several subsets
may be composed into the demanded chip.  If supplies are stable, architects
should pursue the greatest disaggregation possible even if {\em demand}
shocks are possible or likely.
%Indeed, in the face of supply
%shock, disaggregation \emph{alone} is detrimental, and instead a
%combination of designs should be used to meet market demand.
\end{recom}



\begin{figure*}[ht]
  \captionsetup[subfloat]{captionskip=0pt,nearskip=-4pt}
  \centering
    \subfloat[\centering Demand shock]{
        {\includegraphics[width=0.25\linewidth]{./images/distribution/ComShockA.png}}
        \label{ sfig:composition-shock-a}
    } \qquad
    \subfloat[\centering Supply shock]{
        {\includegraphics[width=0.25\linewidth]{./images/distribution/ComShockB.png}}
        \label{ sfig:composition-shock-b}
    } \qquad
      \subfloat[\centering Supply and demand shock]{
        {\includegraphics[width=0.25\linewidth]{./images/distribution/ComShockC.png}}
        \label{ sfig:composition-shock-c}
    }
    \caption{\small Composition's impact in a high risk market.
    	Composition is effective at mitigating \textit{supply shock}, but is ineffective at
    	mitigating \textit{demand shock}.
    }
    \label{fig:composition-shock}
\end{figure*}

Figure~\ref{fig:recourse} depicts the impact of delaying mapping decisions
until recourse to demand is available, such as by using some form of delayed
just-in-time packaging~\cite{angkiriwang2014managing}, in the presence of supply and demand uncertainties in a market for 16-core, 8-core, and 4-core chips.
Increased chip agility via packaging decisions made with `\textbf{K}'nown demand, total
cost distributions are significantly better than when mapping decisions are
made with `\textbf{U}'nknown demand. Further, the benefits of delaying packaging until
demand is known grows as demand uncertainty grows.  Thus, delayed or `just-in-time'
packaging is especially useful in the presence of market uncertainties.

\begin{recom}
When demand uncertainties are high, architects should design systems around
less-intrusive packaging strategies (e.g., 2.5D integration over monolithic
3D integration) so integration can be deferred. Novel packaging and
assembly techniques such as self-assembly~\cite{black2007polymer} and
capacitive or wireless coupling~\cite{charlet2006chip} also become
attractive.
%strategies that can integration strpursue The profit increase from just-in-time packaging indicates composable
%designs can help architects and managers mitigate losses from production
%delays which impact time-to-market. Although late product launches correspond
%to lower overall profits~\cite{}, delayed launch also means just-in-time
%packaging can be done with a better understanding of market demands.
\end{recom}


% TODO: Change stage to different numbers "known demand, unknown demand"
% TODO: No need for correlations
% TODO: Change to demand variance sweep
% TODO: Move to be with interposer graph
\begin{figure}[ht]
    \includegraphics[width=\linewidth]{./images/distribution/RecourseC.png}
    \caption{\small 
    Impact of Delaying Packaging on Total Cost.
    	Witholding packaging until market demand is known leads to significant
    	increases in profit.
    }
    \label{fig:recourse}
\end{figure}

%\subsection{Interposers and Supply Chain}

\iffalse
We have attempted to isolate composition's benefits due to multiple paths to a
demanded good from benefits due to disaggregation but the results also show a
significant advantage of disaggregation beyond the commonly-known benefit to
profit: \textit{disaggregation also leads to reduced total cost variance in the
presence of supply uncertainties}.
\fi

\subsubsection{Adaptation}
\label{sec:adapt_tech}

\iffalse
\st{In considering using chips designed for one demand to satisfy a different
demand, let us specifically look at a form of adaptation usable with multi-core
chips: an $n$-core chip is used to satisfy an $m$-core demand for $m < n$.}
\fi
A market for 16-core, 8-core, and 4-core chips is considered, in which 16-core
chips can be repurposed to meet demand for 8-core or 4-core chips, and 8-core
chips can be repurposed to meet demand for 4-core chips. 
%Electrical and socket compatibility across designs is assumed.

Figure~\ref{fig:adaptation4} shows the sensitivity of total cost to supply and
demand uncertainties in the presence of adaptation.  Adaptation is very effective in
mitigating demand uncertainty, but is not effective at dealing with supply
uncertainty. We also found (not shown) that benefits are higher (up to 23\%
profit) when demands are negatively correlated (e.g., when a popular computer
manufacturer decides to use 4-core chips, instead of 8-core chips in its
flagship product). This is not surprising since the leftover (e.g., 8-core)
chips can be adapted down to other (e.g., 4-core) chips. We also notice that
most adaptations are to the immediately lower performance point (e.g., from
16-core to 8-core and from 8-core to 4-core). Again, this is not surprising
since the high NRE cost of a much larger chip often outweighs the benefits of
adaptation.


Figure~\ref{fig:adaptation-constrained} introduces supply constraints on 8-core
(green) and 4-core (gold) chips.  Adaptation is very useful in this scenario,
as even when 8-core and 4-core chips are unavailable, adaptation enables
meeting their demand via 16-core (blue) chips.  Adaptation enables an expected
profit at all supply constraint factors, whereas without adaptation, an
expected profit is only achieved with supply constraint factor $> 0.30$. This
result prompts a more general insight: \emph{architectural flexibility or
generality enables meeting unanticipated market demands with existing general
purpose hardware}.

\iffalse
Figure~\ref{fig:adaptation3} shows the sensitivity of total cost to
correlations between supply uncertainties and between demand uncertainties in
the presence of adaptation.  With negative correlations (e.g., shortage of
4-core chips means higher likelihood of abundance of 8-core chips), adaptation
is highly effective at increasing expected profit (up to 23\%) and reducing
interquartile range and variance.  However, these improvements are muted at
high positive correlation.  This is because with high positive correlations,
the likelihood of a shortage of 4-core chips but a surplus of 8-core or 16-core
chips is less than when there is a negative correlation, and these are exactly
the scenarios in which adaptation is useful.
\fi

\begin{recom}
Architects should build adaptive architectures that satisfy multiple demands,
especially when demand uncertainties are high. Adaptive architectures are less
attractive when only supply uncertainties exist. 
\end{recom}



Figure~\ref{fig:adashock} shows how adaptation can help deal with supply and
demand shocks. Unlike composition,
%having multiple paths to a single demand good,
adaptation \textit{is effective}
at mitigating demand shocks since there are multiple paths \textit{from}
produced goods.  That is, excess supply of produced goods (due to demand shock)
can be used to meet supply shortages of other goods.  This principle expresses
itself in the optimal order quantity of 16-core chips, which grows by 86\% as
shock factor grows from $0.0$ to $0.5$. Adaptation can also be used to mitigate
supply shocks, once again by privileging chips which can be adapted to multiple
demands, however the benefits are less pronounced than with composition.  


\iffalse
\begin{figure}[ht]
  \centering
      \subfloat[\centering Supply and demand disruptions]{
        {\includegraphics[width=1.0\linewidth]{./images/distribution/Figure11c.png}}
    }
    \caption{\small (A)daptation's benefits for 16 core, 8 core, and 4 core systems for
    different Pearson Correlation Coefficient (PCC) values}
  \label{fig:adaptation3}
\end{figure}
\fi

% Replace with 3d-plots (x-axis dem var, y-axis sup var, z-axis Adaptation Gain)
\begin{figure}[ht]
  \captionsetup[subfloat]{farskip=-3pt,captionskip=-1pt}
  \centering
    \subfloat[\centering Sensitivity to demand variance]{
        {\includegraphics[width=1.00\linewidth]{./images/distribution/Figure12a.png}}
    }

    \subfloat[\centering Sensitivity to supply variance]{
        {\includegraphics[width=1.00\linewidth]{./images/distribution/Figure12b.png}}
    }
    \caption{\small Sensitivity of adaptation for 16-core, 8-core, and 4-core systems to supply and demand uncertainty.
    		Adaptation mitigates some losses from \textit{demand uncertainty},
    		but is not effective at mitigating losses from \textit{supply uncertainty}.	
    }
  \label{fig:adaptation4}
\end{figure}

\begin{figure}[ht]
  \centering
    \includegraphics[width=1.00\linewidth]{./images/distribution/AdapatationSupplyConstrainedWithBaseline.png}
    \caption{\small Adaptation's impact on a supply constrained market.
    	The Supply Constraint factor limits the number of 8-core and 4-core chips available.
    	The smaller the factor, the fewer the chips available.  Adaptation helps mitigate
    	losses by enabling 16-core chips to be repurposed and sold as 8-core or 4-core
    	chips.
    }
  \label{fig:adaptation-constrained}
\end{figure}

\begin{figure*}[ht] %[htbp]
  \captionsetup[subfloat]{captionskip=-4pt}
  \centering
    \subfloat[\centering Demand shock]{
        {\includegraphics[width=0.30\textwidth]{./images/distribution/AdaShockA.png}}
    }
    \subfloat[\centering Supply shock]{
        {\includegraphics[width=0.30\textwidth]{./images/distribution/AdaShockB.png}}
    }
      \subfloat[\centering Supply and demand shock]{
        {\includegraphics[width=0.30\textwidth]{./images/distribution/AdaShockC.png}}
    }
    \caption{\small Adaptation is better at mitigating losses from \textit{demand shock} than
    	from \textit{supply shock}.
    }
  \label{fig:adashock}
\end{figure*}


These
results suggest that 
%composition and adaptation provide \textit{orthogonal}
%benefits. As such, their combined use should provide benefits beyond the
%benefits of either individual intervention.
adaptation and composition are complementary interventions not just in
\textit{which} uncertainties they mitigate (adaptation is best suited to mitigate demand uncertainty while composition is
best suited to mitigate supply uncertainty), but also in \textit{when} they can
be applied. Composition based on packaging may require mapping decisions
\emph{before} knowing exact market demand (unless some delayed or just-in-time integration techniques are used).  Adaptation, often based on
modifying firmware, can be employed \textit{after} market demand becomes clear. 
%\subsection{Combining Interventions}
%As noted, adaptation and composition provide complimentary benefits, since. 
Figure~\ref{fig:ada-comp} shows the
total cost distributions using no interventions, adaptation, composition, and
both adaptation and composition concurrently under standard assumptions for a
market with demands for 16-core, 8-core, and 4-core chips.
In terms of expectation, adaptation and composition are nearly orthogonal: when
both interventions are enabled, the improvement in expected total cost is 91\%
of the sum of the improvements seen by adaptation alone, and composition alone.

\begin{recom}
When demand for goods is susceptible to shocks, architects should ensure
designs are adaptable to multiple demanded goods. In the face of both
supply and demand shocks or uncertainty, adaptation and composition can be
used jointly.  Architectures which support composable designs that can be
adapted to multiple demands benefit from both the mitigation of supply
uncertainty from composition and the mitigation of demand uncertainty from
adaptation.
\end{recom}

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.75\linewidth]{./images/distribution/AdaComp.png}
    \caption{\small Combined, Adaptation and Composition provide better results
    than either alone.  }
    \label{fig:ada-comp}
\end{figure}

%\subsection{Salvage Value}
\begin{figure}[ht]
  \captionsetup[subfloat]{farskip=0pt,captionskip=-1pt,nearskip=-8pt}
  \centering
    \subfloat[\centering Composition]{
        {\includegraphics[width=0.5\linewidth]{./images/CompOverageSweepPie.png}}
        \label{subfig:overagea} 
    }
     \subfloat[\centering Adaptation]{
        {\includegraphics[width=0.5\linewidth]{./images/AdaOverageSweepPie.png}}
        \label{subfig:overageb} 
    }
    \caption{\small
    Chip salvaging enhances the impact of adaptation and composition.
    }
  \label{fig:overagesredux}
\end{figure}

Previous results assumed excess chips were unsalvageable.  However, a large body
of recent work shows that excess chip production can be salvaged via
recycling~\cite{recycle} or repurposing~\cite{repurpose01}. Figure~\ref{fig:overagesredux} shows
how composition and adaptation's effectiveness improves if chips can be salvaged.  `Salvage factor',
$s$, is a scaling factor which determines the salvage value of produced 4-core,
8-core, and 16-core chips, in a market where production of 4-core chips is
constrained. Salvage value is computed as $g = sc$ where $c$ is the unit cost
of the chip. Results show that increased salvaging increases the effectiveness of both composition and adaptation. 
%Subfigure~\ref{subfig:overagea} shows impact of salvaging on the effectiveness of composition. With composition, increasing salvage value actually leads to a 32\%
%increase in number of 8-core chips ordered, as increased salvage value
%decreases the net cost of production overages. Subfigure~\ref{subfig:overageb}
%shows adaptation's impact on this market. With adaptation, increasing salvage
%value leads to a 22\% increase in 8-core chips and an 8\% increase in 16-core
%chips ordered. In both cases, 
High salvage factor helps to reduce shortages
since it lessens the penalty associated with overproduction.  Further, high
salvage factor privileges building \textit{large} chips (e.g., a 32\%
increase in number of 8-core chips ordered in case of composition,  a 22\% increase in 8-core chips and an 8\% increase in 16-core
chips ordered in case of adaptation) since larger chips
have a higher salvage value.  
%Despite this, in the adaptation case, 8-core chip
%growth outpaced 16-core chip growth, due to 8-core's being better suited for
%adaptation to a 4-core demand (since 8-core chips are cheaper to produce that
%16-core chips).

\begin{recom}
Architects should improve salvageability of adaptable and composable
architectures (e.g., through standard electrical and IO interfaces), since
salvageable architectures enable greater use of adaptation and composition
mappings by mitigating costs associated with overproduction.
\end{recom}

Finally, we observe that the above examples of adaptation were between architectures with monotonic relationships (4, 8, 16-core chips). However, adaptation may be beneficial even across non-monotonically related architectures as long as they  target different demands. As an example, consider a case where a microcontroller chipmaker build a microcontroller supporting ISA1 and another microcontroller supporting ISA2, each obviously targeting a different demand.
%supports two ISAs each with a separate microcontroller  as there is a market for each ISA.
%Adaptation is especially useful when there are negative correlations between
%demand uncertainties.  Consider the case of microcontrollers, in which multiple
%RISC, load-store ISAs compete for market share. 
Figure~\ref{fig:multi-isa} suggests that an adaptable \textit{multi-ISA
microcontroller} may instead be a better idea when considering supply chain
resilience. 
%reduces risk and
%increases profit in a microcontroller market. The figure considers a case where
%demand exists for two ISAs, `ISA1' and `ISA2'.  
Each boxplot represents the
distribution of total cost when maximizing for total profit under several
assumptions.  First, `scale' is a scaling factor which indicates how much more
expensive it is to develop a multi-ISA core which implements both `ISA1' and
`ISA2'.  Second, `PCC' is the Pearson correlation coefficient between the
demand uncertainties for ISA1 and ISA2.
%The coloring of each boxplot is a function of the optimal policy.
Blue, red, and green boxplots indicate that the optimal policies are to build
\textit{only} multi-ISA cores, \textit{no} multi-ISA cores, and all three
cores, respectively.  This form of adaptation is immediately useful when the
cost overhead of supporting multi-ISA designs is low.  Multi-ISA cores are the
right cores to build in all scenarios when the overhead is $\leq5\%$. When
multi-ISA overhead approaches 15\%, the effectiveness of Multi-ISA designs is
limited, and only used when there is a negative correlation in the
uncertainties.
%Thus, if overhead for support of multi-ISA can be kept low, then multi-ISA
%design is effective.
Fortunately, as microcontroller ISAs tend to be RISC, load-store architectures
with similar operations and similarly sized register files, low overheads
($\leq5\%$) may be feasible for supporting popular ISA pairs.
% We estimated the overhead of supporting MIPS ISA
% on RISC-V-based Ibex core to be $10\%$.

As another example, consider two separate demands for lightweight encryption
engines supporting two different ISO-certified algorithms -
PRESENT~\cite{bogdanov2007present} and Simon~\cite{kolbl2015observations}.
Both block ciphers support 64-bit blocks with 128-bit keys and are both
designed for efficient hardware implementations. 
As Figure~\ref{fig:multi-isa} shows, it may be more supply chain resilient to build a consolidated design which supports both Simon and PRESENT in lieu of individual
accelerators, regardless of the anticipated correlation between demands for the
two accelerators, as long as the overhead of consolidation is $\leq5\%$. 
We observe that the registers used to store
the key and block make up the majority of the area in hardware implementations
of both ciphers~\cite{present01,simon01}. Therefore, it is indeed possible to create a low overhead consolidated accelerator
for \textit{both} ciphers. We implemented both a consolidated design and
individual designs and found that the area after synthesis for a consolidated
accelerator for both ciphers in a \SI{45}{\nano\meter} technology process is
less than 1\% larger than an accelerator for PRESENT, only, and less than 5\%
larger than an accelerator for Simon, only.
%Thus, from Figure~\ref{fig:multi-isa}, it makes sense to build the `Franken
%Accelerator' which supports both Simon and PRESENT in lieu of individual
%accelerators, regardless of the anticipated correlation between demands for the
%two accelerators.

Note also how a multi-ISA design or a consolidated accelerator targeting separate demands is typically not interesting in terms of conventional architectural metrics such as power or performance. However, such architectures become interesting  once supply chain resilience is considered.  

\begin{recom}
Architects should build novel architectures that consolidate multiple hardware
    designs which share a lot of functionality and structure, but target
    different demands (e.g., microcontrollers supporting different ISAs,
    hardware block-based encryption engines with same block and key size but
    supporting  different ciphers, etc.) into a single design. Such
    architectures will have high supply chain resiliency, especially when the
    overhead of consolidation is low and the demands are negatively correlated.  
\end{recom}

% \begin{figure}[ht] %[htbp]
%   \centering
%     \subfloat[\centering Demand disruption]{
%         {\includegraphics[width=1.00\linewidth]{./images/distribution/MultiISAa.png}}
%     }
% 
%     \subfloat[\centering Supply disruption]{
%         {\includegraphics[width=1.00\linewidth]{./images/distribution/MultiISAb.png}}
%     }
% 
%       \subfloat[\centering Supply and demand disruptions]{
%         {\includegraphics[width=1.00\linewidth]{./images/distribution/MultiISAc.png}}
%     }
%     \caption{\small Multi-ISA Scenarios.}
%   \label{fig:multi-isa}
% \end{figure}
\begin{figure}[ht] %[htbp]
  \centering
    {\includegraphics[width=1.00\linewidth]{./images/distribution/MultiISAc.png}}
    \caption{\small Multi-ISA with supply and demand uncertainty.
    	Cost Scaling Factor determines how much more expensive a Multi-ISA chip
    	is than a single-ISA chip.
    }
  \label{fig:multi-isa}
\end{figure}

% \begin{figure*} %[htbp]
%   \centering
%     \subfloat[\centering Demand disruption]{
%         {\includegraphics[width=0.33\textwidth]{./images/distribution/MultiISABaselineA.png}}
%     }
%     \subfloat[\centering Supply disruption]{
%         {\includegraphics[width=0.33\textwidth]{./images/distribution/MultiISABaselineB.png}}
%     }
%       \subfloat[\centering Supply and demand disruptions]{
%         {\includegraphics[width=0.33\textwidth]{./images/distribution/MultiISABaselineC.png}}
%     }
%     \caption{\small Two ISA Scenarios. (No multi-ISA core)  }
%   \label{fig:multi-isa-baseline}
% \end{figure*}



\subsubsection{Dispersing Supply Risks}

Figure~\ref{fig:dispersion0} shows the effect of dispersion on cost in the
presence of supply constraints.  In baseline cases, a single produced good is
manufactured by a single foundry but in other cases, a single produced good is
manufactured by multiple foundries. Besides the supply constraint, there is
also an order equality constraint which requires the amount of chips of each
type ordered from each foundry to be equal.
This constraint is necessary because an $\E{TC}$ minimizing policy
may choose to order uneven amounts of chips from suppliers, but variance
is minimized when orders are evenly distributed among
(independent and identically distributed) suppliers.
As such, pie charts are omitted. As additional
foundries are added, the sequence of distributions formed by increasing the
supply constraint factor takes on a `hockey stick' shape, as the intervention
proves useful in obtaining adequate supply even when individual foundries
cannot meet the demand.  With a single foundry, the medians of the
distributions have a strong linear correlation with supply factor throughout
the entire range of supply factors; they require a supply factor of 1.00 to
implement an optimal order policy.

\begin{recom}
When demand outstrips supply, architects should, if possible, design chips that
can be fabricated by a variety of foundries. This can be enabled by using a
trailing edge process node, a commodity IP or component, or non-proprietary
technologies.
%Voltage and frequency scaling can be used to mitigate potential performance
%or power shortcomings associated with using an older tech node.  When
%possible, hard IPs can be used instead of soft IPs to accelerate
%multi-technology design.
\end{recom}

\begin{figure}[ht]
  \centering
   {\includegraphics[width=1.00\linewidth]{./images/distribution/DispersionSupplyConstrainedC.png}}
    \caption{\small Dispersion's impact on a supply constrained market.
    	Multiple suppliers enables market demand to be met, even when a single
    	supplier is unable to produce adequate chip volume.
    }
  \label{fig:dispersion0}
\end{figure}

\begin{figure}[ht]
 \captionsetup[subfloat]{farskip=0pt,captionskip=0pt}
 \centering
   \subfloat[\centering Demand disruption]{
       {\includegraphics[width=1.00\linewidth]{./images/distribution/Figure13a.png}}
       \label{sfig:13a}
   }

   \subfloat[\centering Supply disruption]{
       {\includegraphics[width=1.00\linewidth]{./images/distribution/Figure13b.png}}
       \label{sfig:13b}
   }

     \subfloat[\centering Supply and demand disruption]{
       {\includegraphics[width=1.00\linewidth]{./images/distribution/Figure13c.png}}
   }
   \caption{\small Sensitivity of dispersion to  supply and demand uncertainty.}
 \label{fig:dispersion1}
\end{figure}

\begin{figure}[ht]
  \centering
    \includegraphics[width=1.00\linewidth]{./images/distribution/DispersionShockB.png}
  \centering
    \caption{Dispersion provides resilience to supply shocks}
    \label{fig:dispersion-shock}
\end{figure}

% In the demand disruption case, we see that dispersion
% has no benefit, as dispersion is suited for dealing with supply disruption
% only (since if supply is deterministic, there is no reason to purchase from
% multiple vendors), and, in fact, hurts profitability due to increases in
% NRE.  On the other hand, in the supply disruption case,
% dispersion massively reduces interquartile range, maximum total cost, variance, 
% and reduces the total cost of outliers.  Dispersion is highly effective at
% reducing uncertainty in the face of supply disruptions, reducing total cost
% variance by up to 71\%.
Figure~\ref{fig:dispersion1} shows the sensitivity of dispersion to supply and
demand variance.  As in Figure~\ref{fig:dispersion0}, there are order equality
constraints and pie charts are omitted. Under demand disruption
(Subfigure~\ref{sfig:13a}), dispersion gives no benefit since deterministic and
unconstrained supply militates use of multiple vendors, and, in fact, hurts
profitability due to more NRE. Interesting behavior emerges in
Subfigure~\ref{sfig:13b}.  As supply uncertainty variance increases, so does
total cost variance.  However, with multiple suppliers,
there is a discrete jump in total cost variance.
With two
second suppliers this jump occurs
between $0.105$ and $0.112$.
Adding a third supplier pushes this jump later, to between $0.12$ and $0.128$.
This nonlinearity in total cost variance can be delayed (and
thus mitigated) by using additional suppliers.

% \st{Figure~\ref{fig:dispersion-shock} shows how dispersion helps mitigate risks
% from \textit{supply shocks}. Previously we modeled uncertainty with a Gaussian
% distribution, but now we consider a single demand good with two producers; one
% producer's supply uncertainty is a Bernoulli random variable with $p=1-x$ where
% $x$ is the captioned value.  In the first set of results, chips are purchased
% only from this risky supplier.  In the second set of results, dispersion is
% used na\"ively so only a single supplier at a time is used, where that supplier
% is chosen to maximize expected profit.  In the third set of results (prefixed
% by `Equal'), equal numbers of chips are purchased from both suppliers.  Notice
% that dispersion can minimize risk to supply shock, with purchasing from both
% suppliers reducing variance by up to 47\%.}

The results also motivate the need to amortize NRE costs across suppliers.
Sharing verification efforts, physical design components such as IO ring, or
even GDS/OASIS geometries (whenever possible) can help increase benefits from
dispersion.

Figure~\ref{fig:dispersion-shock} shows how dispersion helps mitigate risks
from supply shocks. While purchasing from multiple suppliers can provide modest
improvements to expected benefit, its major impact comes in reducing total cost
variance.  purchasing from multiple suppliers reduces variance by up to 47\%.



\begin{recom}
Architects should consider designing dispersible architectures (e.g, ones where they have determined through application-level analysis the components that are not performance-sensitive and can, therefore, be implemented in a trailing edge process node) to
%one when accurately
%projecting profits is difficult due to the incredible effectiveness at
reduce risks from supply shocks and supply uncertainty, even if it does
not necessarily lead to increased profits. Conversely, dispersible architectures increase NRE costs and should, therefore, be avoided when supply variations are limited.
\end{recom}

\iffalse
The results show that novel interventions can improve semiconductor supply
chain resilience.  While industry performs composition and adaptation in the
form of disaggregation and binning/rebadging, to the best of our knowledge,
industry \textit{does not} use these intervention techniques to create multiple
paths from produced to demanded goods, such as by performing non-equal set
composition, trans-demand adaptation, or dispersion. These interventions,
which have architectural, packaging, and design implications, are effective at
increasing profits and decreasing risks of extreme losses in the face of supply
and demand uncertainties and shocks.
\fi

\iffalse
Let us note that dispersion does lead to significant increases in profit when
individual foundries are unable to satisfy chip demand; this effectiveness
depends on the NRE Reuse factor.  The more a design can be reused between
foundries, the lower aggregate NRE costs and thereby higher profits.
\fi

\iffalse
\subsubsection{Sensitivity to Salvage Value}

\begin{figure}[ht]
  \centering
    \includegraphics[width=1.0\linewidth]{./images/distribution/Overage.png}
    \caption{\small Impact of salvage value and overage costs.  }
  \label{fig:overage}
\end{figure}

Figure~\ref{fig:overage} shows total cost for varying salvage values and
overage costs for 16, 8, and 4-core chips. At $-1.00$, each unsold chip costs
its unit production cost whereas at $1.00$, each unsold chip provides a salvage
benefit equal to its production cost.  Other salvage values lie between these
extremes. Distributions prefixed with `A' have (A)daptation interventions
enabled; otherwise no interventions are used.  Supply and demand uncertainties
are Gaussian distributed. Under these conditions, optimal policies privilege
increased 16-core chips as the salvage benefit increases. This is especially
true when adaptation is enabled, which sees nearly twice the increase in
16-core orders as when no interventions are used. This is because the salvage
of the larger 16-core chips is higher than for the smaller 8-core and 4-core
chips, which provides further incentive to produce 16-core chips --- even when
there is not excess 8 or 4-core demand, 16-core losses can be recouped via
salvage.

Architectural decisions can effect chip reuse and recyclability.  For
example, pin compatibility between chips may allow a chip to be adapted
for use in a system it was not originally intended for.  Use of organic
packaging can reduce chip recycling costs~\cite{green01}~\cite{green02}~\cite{green03}.
\fi



%\iffalse
%\subsection{Franken-Accelerators, Multi-ISA Designs, etc.}
%\label{sec:multi-isa}


\iffalse
\subsection{Amortizing NRE Costs}
Figure~\ref{fig:nre-reuse} shows the impact of `NRE Reuse' on the effectiveness
of dispersion.  NRE Reuse is when NRE can be amortized across multiple physical
designs, either because they share architectural and RTL level design and
verification efforts, or because they even share physical design components
such as IO ring, or even GDS/OASIS geometries (as when the same design is
manufactured in multiple foundries using the same technology and process).
The NRE Reuse factor, $f$, is the amount of NRE which is shared between designs.
Hence at $f = 0.0$, each produced chip has full NRE costs, while at $f = 1.0$,
only the first version of each chip costs full NRE, while subsequent versions
of the chip have zero NRE costs. As is expected, a high-NRE reuse factor
enables the risk-mitigation of dispersion while also maintaining the high
expected profit associated with a single produced good.

\begin{figure}[ht]
    \centering
    \includegraphics[width=1.00\linewidth]{./images/distribution/NreReuse.png}
    \caption{Impact of NRE Reuse factor.}
    \label{fig:nre-reuse}
\end{figure}
\fi

\iffalse
\subsection{Reducing Compatibility Costs}
Figure~\ref{fig:adaptation-compatability-costs} demonstrates adaptation's
sensitivity to costs associated with enabling adaptation.  In the figure,
the $x$-axis represents the adaptation cost factor, $f$.  The unit cost of each
chip is incremented by $f\cdot c_{\text{4-core}}$ where $c_{\text{4-core}}$ is
the base unit cost of the 4-core chip.  This additional cost represents
the costs associated with ensuring compatibility between the chips
(e.g., electrical compatibility, socket compatibility, etc).  
The figure shows that adaptation is sensitive to this adaptation cost factor,
with the benefits of adaptation under standard assumptions of supply and
demand uncertainty disappearing when the factor $f \geq 0.11$.  Often, though,
this factor is minimal.  For example, Intel's i3, i5, i7, and i9 lines of
12th generation Alder Lake processors are all compatible with the Z690
motherboard chipset.

\begin{figure}[ht]
    \centering
    \includegraphics[width=1.0\linewidth]{./images/distribution/AdaptationCostOfCompatability.png}
    \caption{\small Sensitivity of adaptation for 16-core, 8-core, and 4-core
    systems to adaptation compatibility costs.}
    \label{fig:adaptation-compatability-costs}
\end{figure}
\fi


==> scenarios.tex <==
\subsection{Production of Undemanded Goods}

Consider a scenario in which two different produced goods may be used to
satisfy a single demand good.  The first produced good, $g_1$, is exactly
the demanded good, while the second produced good, $g_2$, can be adapted to
the demand for $g_1$, albeit with an additional cost, $t$.

Whether to produce $g_1$ or $g_2$, then, is determined by values for $r$, $t$,
$c_1$, $c_2$, $n_1$ and $n_2$, as well as the number of $g_2$ demanded ($Z_d$).

In a deterministic scenario, it makes sense to build $g_2$ instead of $g_1$
if and only if the cost of building and adapting the $g_2$ is less than the cost
of building the $g_1$.  I.e., if and only if
\[
    (c_1 + t - r)Z_d + n_1 < (c_2+t-r)Z_d + n2.
\]

\subsection{Uncertainty Affects Optimal Choice of Substitution}

Consider a scenario in which two different demanded goods exist, $d_1, d_2$,
and in which three different produced goods exist, $p_1, p_2, p_3$.  The
demand goods $d_1$ and $d_2$ can be satisfied \textit{directly} by an instance
of $p_1$ or $p_2$, respectively, or they can be satisfied by an instance of
$p_3$ with an additional cost of $t$.\footnote{This is the `magical goop'
scenario.}

Suppose that the production costs of all of the $p$ goods are the equal,
as are the unit benefits of the two demand goods.  Suppose that salvage value
is negligble\footnote{sandwhiches go bad at the end of the day, and cannot be
sold the next day}, and that the unit shortage cost, $g$, is very high.

First, suppose that there is no uncertainty in either supply or demand. In this
case, the optimal solution is to $x = (Z_d^1, Z_d^2, 0)$, i.e., we build
exactly as many $d_1$ and $d_2$ as are demanded, and build no $d_3$, since
converting a $d_3$ to a $p_1$ or $p_2$ has an addional cost of $t$.

Next, suppose that there is demand uncertainty modeled as follows: both $Z_d^1$
and $Z_d^2$ are uniformally distrubted over the natural numbers $\leq k$ (where
$k$ is some known consant), and $Z_d^1 + Z_d^2 = k$.  That is, we know with
certainty the demand for the sum of the products, but we have zero knowledge
about the demand for the individual products.

If $g$, the shortage cost is sufficiently high relative to $t$, the cost 
of transforming a $p_3$ into a demand good, then the cost minimizing solution
is $n = (0, 0, k)$.  That is, if $gt \leq k$, then we will \textit{only} build
$p_3$.

\subsection{It is Important to Pick the `Correct' Substitution}

Consider a scenario in which two different produced goods, $p_1, p_2$, can
both be used to produce a single demand good, $d$.  Further, suppose that
$t_1=t_2=0$, i.e., there is no cost associated with transforming either of
the produced goods into the demand good.  However, the NRE costs and unit
costs for the two goods differ, with $n_1 > n_2$, but $c_1 < c_2$.
Further, suppose that there is no uncertainty in either supply or demand.
Then the choice of producing $p_1$ or $p_2$ is dependent on $Z_d$, the
quantity of $d$ demanded.
Thus, the profit of producing $p_i$ to satisfy $d$ is given by
\[
    Z_d(r-c_i) - n_i.
\]
The quantity for $Z_d$ at which $p_1 = p_2$, then, is
\begin{align*}
    Z_d^= &= \frac{n_1-n_2}{c_2-c_1}.
\end{align*}
Thus, if $Z_d < Z_d^=$, it is optimal to subsitute $p_2$ for $d$, while if
$Z_d> Z_d^=$, it is optimal to subsitute $p_1$ for $d$.


\subsection{How Do We Solve the Optimization Problem?}

The optimization problem has some interesting nuance.  On the one hand,
the decision variable, $x$, has to be decided a priori without knowledge
of the realization of supply uncertainty.  On the other hand, the mappings
of the produced goods into the demanded goods may be done a posteriori,
\textit{after} the realization of the produced goods, $\bar{x}$.

This enables problem to be solved using the following function which
evaluates $E[TC|x]$:

\begin{enumerate}
    \item For an input value of $x$.
    \item Compute the probability distributions for $\bar{x}$, as well as for
            $z_d$ (the probability distribution for the demanded goods).
    \item \label{item:joint_pdf}
        Compute the joint pdf for $(\bar{x}, z_d)$.
          Note that this is a discrete distribution.
    \item \label{item:optimal_P}
          Compute optimal $P$, quantities of each mapping to take, for each
          possible value of $(\bar{x}, z_d)$.
    \item Using \ref{item:joint_pdf} and \ref{item:optimal_P}, compute
          $E[TC|x]$.
\end{enumerate}

With this function, we can then perform optimization using standard techniques
such as simulated annealing.
Note that step~\ref{item:optimal_P} can be performed quickly for a given
point in the probability space using a linear program. Further, if the
probability space is prohibitively large (e.g., large quantities of demanded
or produced goods), we can break the probability space into equi-probable
neighborhoods, and use the centroid values of those neighborhoods as
samples, enabling fine-grained control over optimization latency.

\subsection{Programmability Helps}
Consider the case where there is demand for $k$ ASICs, except the demand
has very high variance of the form $m_iX_i$ where the $m_i$ are constants
and the $X_i$ are independent random variables
$X_i\sim{}\text{Bernollui}(p_i)$.  This scenario depicts selling ASICs to
start-ups or other volatile purchasers.
The produced goods used to meet this demand could be the $k$ dedicated ASICs,
or it could be a single device which either combines the $k$ accelerators onto
a single die, or is programmable (e.g., a CGRA or FPGA based system).
Suppose supply is deterministic (i.e., there is no supply uncertainty).
Also suppose that shortage costs are negligible.

Consider the case of building individual ASICs.  For each demanded good
expected profit is the sum of the sales and salvage minus per-unit costs and
NRE costs. We assume that $0 \leq x_i \leq m_i$ (i.e., we will never build
more ASICs than for which there is possible demand).

\begin{align*}
    E[P_i|x_i > 0] &= E[P_i~|~X_i=1, x_i > 0]p_i + E[P_i~|~X_i = 0, x_i > 0](1-p_i) \\
    &= \left(x_i(r_i-c_i) - n_i\right)p_i + \left(h_ix_i - n_i\right)(1-p_i) \\
    &= x_i((r_i-c_i)p_i + h_i(1-p_i)) - n_i.
\end{align*}
Thus, expected profit is an affine function of $x_i$. Thus it is maximized
at $x_i = X_i$ if $((r_i-c_i)p_i + h_i(1-p_i))$ is positive.  If this slope
term is negative, or if $E[P_i|x_i = X_i] \leq 0$, then the optimal course
of action is to not build these ASICs.

Expected profit for demand good $i$, then is $E[P_i] = \max{E[P_i|x_i>0], 0}$,
and expected profit is $E[P] = \sum_i E[P_i]$.

Significantly, there are regimes such that $E[P] = 0$.  That is, we make
zero profit because we anticipate losing money if we manufacturing \textit{any}
ASIC.  However, in such regimes, the programmable approach may lead to
positive profit.

Suppose that instead of manufacturing ASICs, we manufacture a chip with a
programmable substrate (or a `Frankencellerator' which can meet the needs of
all of the purchasers).  In this case, we anticipate a lower unit-reward or
higher unit cost, since the programmable hardware will either be significantly
larger or less-performant than a dedicated ASIC.  We also anticipated that its
NRE, $n$ is larger than any individual $n_i$ as it is a larger circuit,
but less than $\sum_i n_i$, as it is only a single circuit, and not $k$ seperate
circuits. Under this regime, our expected profits, assuming $x > 0$, is highly
non-linear. To compute it, first assume that the demand goods are in decreasing
order of profit, i.e., $r_i-c_i > r_{i+1}-c_{i+1}$ for $i \geq 1$.

\begin{align*}
    E[P] &= \min\{x, m_1X_1\}(r_1-c_1) +
    \sum_{j=1}^k\left(
        \max\{0, \min\{x-\sum_{i=1}^{j-1}\left(m_iX_i\right), m_jX_j\}\}(r_j-c_j)\right) \\
        &+ h\max\{0, x-\sum_{j=1}^k m_jX_j\} -
            \min\{n, xn\}.
\end{align*}

Suppose that $(r_i-c_i) = R$ for all $i$.  Further, suppose $m_i = m$ for all
$i$.  Finally, suppose the $X_i$ are i.i.d. with $p_i = p$.  Suppose that for
these parameters are chosen such that, in the ASIC case, $E_A[P] = 0$.  Then,
if $k = 1$, we also know that in the programmable case, $E_P[P] = 0$, since
$n > n_i$ and $c > c_i$.  However, suppose $k >> 1$.  Then $E_A[P] = 0$, since
$E_P[P_i] = 0$ for all $i$.  However, for sufficiently large $k$,
the non-linearities of $E_P[P]$ kick in, causing $E_P[P] > 0$ so long as
$R > 0$, since, in this case, 
\begin{align*}
    E_P[P|x=kpm] &= E[\min\{x, \sum_{i=1}^k m_iX_i\}R +
                      \max\{0, x-\sum m_iX_i\}h - n] \\
                 &= \min\{x, kpm\}R + \max\{0, x-kpm\}h - n \\
                 &= kpmR - n.
\end{align*}
Then, choice of $k > \frac{n}{pmR}$ results in positive expected profit for the
programmable case, while expected profit for the ASIC case is zero. 
Note that a non-negligable shortage cost \textit{strengthens} the case for
programmability, as a non-negligable shortage cost will push $E_A[P] < 0$.

\subsection{Chiplets Helps}
Suppose we want to enter the microprocessor market in both the commodity and
server classes.  We want to decide whether to build monolithic architectures,
or chiplet based architectures, in which a number of chiplets common to both
server and commodity class are combined to generate the two chips.

In the monolithic scenario, all decisions are made in the presence of both
demand and supply uncertainty.  That is, the number of server-class and
commodity-class dies to order is decided at time A.  However, in the chiplet
scenario, the chiplets the number of chiplets to order is decided at time A,
while the number of each chip to build is determined at time B, after the
chiplets have been manufactured, and significantly later than time A.
As supply uncertainty cannot be higher at time B than at time A, and is, in fact
likely less at time B than at time A, building chiplets has a distinct
advantage over building monolithic chips.


==> summary.tex <==
In this paper, we presented the first study on the role of chip architecture in
improving semiconductor supply chain resilience. We observed that supply chains
with one-to-one mapping between produced and demanded chips are fragile. Based
on this observation, we presented composition, adaptation, and dispersion as
architectural techniques to provide supply chain resilience. These techniques
allow multiple paths to achieve a given chip demand. We developed a model that
allows us to analyze the impact of different architectural techniques on supply
chain costs. We used this model to show quantitatively that composition,
adaptation, and dispersion can indeed be effective at providing supply chain
resilience for different kinds of disruptions (Table~\ref{tab:use-cases}). We
provided specific recommendations  for architects for different supply and
demand regimes.
\iffalse
We observed that composition is best at mitigating losses due to supply
uncertainty, while adaptation is best at mitigating losses due to demand or
market uncertainty.  Dispersion is best used when demand outstrips the supply
available from a single foundry or technology process.  In these cases,
dispersion can mitigate losses by enabling the same demanded chip to be
procured at multiple processes and from multiple foundries.  Dispersion can
also be used to reduce \textit{risk} to extreme losses, even when a single
foundry can produce unconstrained quantities, by using redundant supply
channels to reduce supply variance. These recommendations are summarized in .
\fi
These are the first such recommendations for architects to the best of our
knowledge.


\begin{table}[ht]
\caption{ \small
    Summary of key findings. A `{\color[HTML]{6434FC} ✓}' indicates
    the intervention mitigates profit losses due to the supply
    chain and market disruptions. A `{\color[HTML]{009901} ✓}' indicates the
    intervention is mitigates risks of extreme losses due to the
    supply chain and market disruptions. A `{\color[HTML]{FE0000} ✗}' indicates
    the intervention is not useful.
    }
\label{tab:use-cases}
    \resizebox{\columnwidth}{!}{%
        \input{./texFiles/use-cases.tex}
    }
\end{table}


==> themodel.tex <==
% This section details a model for computing the costs and
% revenues the firm incurs, and hence the net earnings for the chip manufacturing
% company with and without disruptions to demand and %supply. 
% \nathan{
%To perform this study, 
To understand the efficacy of different architectural techniques at improving
supply chain resilience, 
we need a model that computes the costs a chip supply
firm incurs with and without disruptions to demand and supply and that can model different architectural techniques. 
We build on the cost model of a generic supply chain developed by
Begen {\em et al.}~\cite{begen_supply_2016}; this model can estimate the impact
of supply and demand uncertainties on supply chain costs. Crucially, the model
was claimed to have been developed in consultation with  industry experts at Intel and
``a large Korean consumer electronics firm". We augmented the model to enable
compatibility with commercial stochastic program solvers, as well the ability
to model different computer architecture techniques. Since we are less
interested in the absolute numbers produced by the model than the (especially
comparative) trends and analyses generated by the model, we believe that this
model has sufficient fidelity for nature of conclusions we derive
(Section~\ref{sec:results}). 

\iffalse
Assume there is a firm which produces computer chips for customers. The
customers have some requirements for the chip, and the firm sells them chips
which will meet or beat these requirements. Note that the firm may manufacture
multiple types of chips that satisfy this requirement, and the set of all the
types chips that satisfy a particular customer requirement is refered to as a
'class' of chips.  The firm’s two goals are to maximize profit and minimize the
amount of variation in the profit in the face of disruptions to the supply and
demand of chips. 
\fi

\subsection{The Certain Case}

To sell chips to the customer, a chip supply firm must  first produce them. To
do this, the firm decides to order various quantities of different input
components. Let $\vec{x}$ denote this ordering decision, where $x_{i}$
represents the number of input components of type `i' the firm ordered. Input
components can be completed chips or components to make a final chip (e.g.\
chiplets). The components each have a  per-unit cost $\vec{c}$ to manufacture
them as well as a non-recurring engineering cost $\vec{n}$ associated  with the
designing and tooling necessary to produce a given input component. The
`ordered' vector, $\vec{o}$, is defined so $o_{i}$ is zero if and only if
$x_{i}$ is zero. Thus, $\vec{o}$ states which components, chip or chiplet, will
be designed and produced for sale.

With these terms, the cost of ordering components is:
\begin{equation}
    TC_{prod} = \dotprod{x}{c} + \dotprod{o}{n}.
\end{equation}
Assuming the ordered input components do not have perfect yield, and modeling the
average yield for each type of input component as $\vec{y}$, the vector of
usable input components one has produced at cost $TC_{prod}$ is
\(\hadprod{x}{y}\), the Hadamard product of the $\vec{x}$ and $\vec{y}$.

\iffalse
The demand for a chip is certain when
\begin{enumerate}[label=(\alph*)]
  \item The number of chips demanded with each of a given set of requirements
      is known at the time chips must be ordered, and
  \item This demand quantity is not subject to change over the period of the
      lead time in manufacturing the chips.
\end{enumerate}
\fi

%This quantity of chips demanded is given by $\vec{Z_{d}}$ and is a constant.
When not considering any uncertainty in demand, $\vec{B}$
represents the units of each demanded chip type that can be sold, and $\vec{r}$
denotes the per-chip benefit the firm receives for each type of chip.  If the
firm produces more of any kind of chips than its corresponding value in
$\vec{B}$, those chips are salvaged for a reduced price (this could be
through scrapping, re-purposing, etc.);  $\vec{h}$ gives the per-chip salvage
value for each type of chip. On the other hand, if the firm produces a type of
chip in a quantity less than what was demanded (as specified in its
corresponding entry in $\vec{B}$),  it incurs costs. In addition to the
opportunity cost of the missed potential sales, there is an additional shortage
cost to the firm for each chip it didn't deliver because it didn't satisfy the
customer's requirement (this could be in the form of lost back-orders, lower
future order quantities etc.). $\vec{h}$ gives the per-chip shortage cost for
each type of chip.

Assuming the firm sells $\vec{\alpha}$ chips with a shortage of $\vec{\beta}$
units and overage of $\vec{\gamma}$, the total cost to the firm on the demand
side is given by
\begin{equation}
    TC_{dem} = \dotprod{\beta}{g} - \dotprod{\alpha}{r} - \dotprod{\gamma}{h}
\end{equation}
% \begin{align}
%     \beta_{i} = [B_i-p_{i}]^{+} \\
%     \gamma_{i} = [p_{i}-B_i]^{+}
% \end{align}
where $p_{i} = \hadprod{x}{y}$. Note that $TC_{dem}$ will be negative as long
as the firm receives a net cash inflow solely as a result of selling (or not
selling) its chips.  Hence, the quantity of the $i$'th demanded chip assembled
is given by \(\alpha_i = \sum_{j} 1_{M^o_j = i}\cdot M^q_j\),
% \begin{equation}
%     \alpha_i = \sum_{j} 1_{M^o_j = i}\cdot M^q_j,
% \end{equation}
and $\beta_i = \left[B_i - \alpha_i \right]^+$ and
$\gamma_i = \left[\alpha_i - B_i\right]^+$.
As of this point, there are two decoupled cost functions for $TC_{dem}$ and
$TC_{prod}$. To link these two, the mapping function $M$ is used. Given $n$
produced goods and $m$ demanded goods, and $k$ mappings $M$.  Consider mappings
to be parameterized as follows: the $j$'th mapping, $M_j = (M^i_j, M^o_j, \Gamma_j)$
where $M^i_j$ is a vector of length $n$ where the $k$'th index corresponds to
the number of the $k$'th produced good needed to perform the mapping,
$M^o_j$ represents the demand good which the mapping produces, and
\(\Gamma_j\) is the cost of creating an $M^o_j$ using $M_j$.  The 
quantity of the usage of $M_j$ is labeled $M^q_j$.
Thus,
\begin{equation}
    TC_{map} = \sum_{j} M^q_j \cdot \Gamma_j.
\end{equation}

Additionally, there is a cost function associated with the selected mapping
function, denoted by $\Gamma$. $\Gamma$ gives the cost the firm incurs every
time a particular mapping is made, i.e, if $\Gamma_k$ denotes the cost of the
$k$'th mapping, then ${\Gamma_k}\cdot{M^q_j}$ is the total cost associated with
using the mapping $M_j$.

Thus the total cost is given by the sum of the cost of ordering components,
mapping these components into processors and selling these processors:
\begin{equation}
    TC = TC_{prod} + TC_{dem} + TC_{map}. \label{eq:tc}
\end{equation}
\iffalse
Table 1 summarizes all the parameters of the model


\begin{table}
\tiny
    \centering
    \begin{tabular}{|c|c|c|} \hline
        Parameters & Description & Dimension  \\ 
        \hline
        $r$ & Unit Benefit & Saleable Products\\
        $g$ & Shortage Cost & Demand Requirements\\
        $h$ & Salvage Value & Saleable Products\\
        $y$ & Yield Rate & Input Components\\
        $p$ & Saleable Products & Saleable Products\\
        $c$ & Per-Unit Cost & Input Components\\
        $n$ & NRE Cost & Input Components\\
        $Z_s$ & Supply & Input Components\\
        $Z_d$ & Demand & Demand Requirements\\
        $\Gamma_x$ & Mapping Cost Functions & N.A \\ \hline
        Decision Variables & & \\ 
        $x$ & Order Quantity & Input Components\\ 
         $M_x$ & Family of Mapping Functions & N.A\\ \hline
        Calculated Values & & \\
        $o$ & Indicator for $x>0$ & Input Components\\
        $TC_{prod}$ & Cost of ordering components & 0 (Scalar)\\
        $TC_{prod}$ & Cost of selling goods to customer & 0 (Scalar\\ 
        \hline
    \end{tabular}
    \caption{Complete Parameters}
    \label{tab:ComPar}
\end{table}
\fi

\iffalse
Figure ~\ref{fig:Model_diag} depicts the overall model as described till now.
Total Product Cost $TC_{prod}$ depends on the number of goods ordered and which
goods were ordered, which are multiplied by the unit cost of each good, and the
NRE of a particular good if it was ordered respectively. The input component
quantity depends on the order quantity, but there are yield losses and changes
in the quantity due to supply uncertainty. These input components are then
mapped to saleable product $\vec{p}$, which carries a mapping cost. The number
of goods sold depends on both the demand and the quantity of goods produced,
and this is multiplied with the benefit of selling each good to get the total
product sales. Overage and shortage quantities can be found from $\vec{Z_{d}}$
and $\vec{p}$, and using the salvage value or shortage cost, is sufficient to
determine the cost of overage/shortage to the firm. The product sales and the
overage/shortage together make up $TC_{dem}$, and the total cost, $TC$ is the
some of Product Cost, Mapping cost and $TC_{dem}$. 


While the choice of order quantities and sales figures are largely outside of
the architect's hands, the mapping function and its subsequent cost function
are directly controlled by the architect's decisions. A different choice in
terms of tech node, memory sizing, chiplet use, or usability of the chip for
multiple classes of customer demands (such as multi-ISA chips) can affect the
ways input components can be mapped to satisfy various customer demands.
Additionally, the architect's decisions also inform what to do when supply and
demand are not as certain as they are here.
\fi


\subsection{The Uncertain Case}

\iffalse
In the certain case, pre-existing knowledge of supply and demand allows the
firm to plan out its chip production exactly. However, in the real world
neither production or demand are certain, and so the model must capture
uncertainties in both supply and demand of chips. 
\fi

Modeling supply and demand uncertainty requires additional parameters,
$\vec{Z_{s}}$, and $\vec{Z_d}$, which are random vectors whose components scale
the components of $\vec{p}$ and $\vec{B}$, respectively. I.e, the vector of
manufactured input components goes from \(\hadprod{x}{y}\) to
\(\hadprod{x}{y}\circ\vec{Z_s}\). After updating $\beta_i$ and $\gamma_i$ to
account for the introduction of $Z_d$, the expected total cost now becomes
\begin{equation}
    \E{TC} = TC_{prod} + \E{TC_{map}} + \E{TC_{dem}},
\end{equation}
since both $TC_{map}$ and $TC_{prod}$ are functions of $Z_s$ and $Z_d$.
%Here both the mapping cost to assemble the chips and the demand costs
%associated with sales are dependent on $Z_{s}$ and $Z_d$, thus the
%expectation over all of its possible values is relevant.

\iffalse
\begin{figure}
    \centering
    \includegraphics[width=0.65\linewidth]{./images/newfigures/model_eqn_diagram.png}
    \caption{Graphical Depiction of the Cost Model}
    \label{fig:Model_diag}
\end{figure}


As the sales terms are taken
under the joint expectation of both uncertainties, there are many possibilities
to consider. This makes determining the best architectural choices nontrivial
with respect to supply and demand. It may render the best choices in the
certain case inferior in the uncertain case.
\fi

\subsection{Modeling architectures for supply chain resilience}

The above model is capable of expressing adaptation, composition, and disruption by
using a variety of `mappings' and replications of supply goods.
Consider two
produced chips --- 16-core and 8-core CPUs, which are used to meet a
demand for 16-core and 8-core CPUs.  To model a scenario without
the proposed architectural interventions (i.e., when the produced good is the same as the demanded good), two `identity' mappings are used.  The first maps produced
16-core chips to demanded 16-core chips, the second maps produced 8-core chips to
demanded 16-core chips.  To model the ability to adapt the produced 16-core
chip to an 8-core chip demand, an additional mapping is used which consumes one
produced 16-core chip and creates a single 8-core chip.  To model the ability
to compose two 8-core chips into a 16-core chip, a different additional mapping is used
which consumes two produced 8-core chips and creates a single 16-core chip.
This mapping is also paired with a non-zero $\Gamma$ value, indicating
integration cost (e.g., interposer and bonding costs).\footnote{Alternatively,
the interposer can be modeled as a third produced chip, and the mapping
consumes one interposer and two eight-core chips.}
To model dispersion, additional produced goods are modeled (e.g., 16-core A
and 16-core B), with each having their own (independent or dependent) supply
factors and mappings to the related demand good(s).  
%Compositions of these three interventions can be modeled by generating the
%relevant additional mappings and supply good replications.



\iffalse
\nathan{As depicted in
Figure~\ref{fig:opt_stages},}~in stage 1, the program decides on $x$ with no knowledge
about supply and demand uncertainty beyond the shape of their distribution.
Since the constraints require that the quantities of each produced good built
are known before the quantities of each mapping can be determined, $M^q$ is
determined in stage 2 with recourse to supply uncertainty. Depending on the
specifics of the modeling scenario, it may make sense to give the $M^q$
decision recourse to demand uncertainty, as well. For example, the decision to
sell a 16-core processor as an 8-core processor can be made very late in the
production process, as disabling cores can be done via firmware.
Table~\ref{tab:recourse} sumarizes the staging of the decision variables and
recourse parameters.

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\centering
\begin{tabular}{@{}ccc@{}}
\toprule
\multicolumn{1}{l}{\textbf{Variable}} & \multicolumn{1}{l}{\textbf{Decision Stage}} & \multicolumn{1}{l}{\textbf{Recourse Stage}} \\ \midrule
$x$   & 1 & -      \\
$M^q$ & 2 & -      \\
$Z_s$ & - & 2      \\
$Z_d$ & - & 2 or 3 \\ \bottomrule
\end{tabular}
\caption{Staging for Decision Variables and Recourse Parameters}
\label{tab:recourse}
\end{table}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{./images/newfigures/Optimization_Sequence.png}
    \caption{Description of each stage of optimization}
    \label{fig:opt_stages}
\end{figure}

\fi


==> use-cases.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{tabular}{rccccc}
\multicolumn{1}{l}{} & \multicolumn{2}{c}{Uncertainty}                     & \multicolumn{2}{c}{Shocks}                          & Constraints              \\
\multicolumn{1}{l}{} & Supply                   & Demand                   & Supply                   & Demand                   & Supply                   \\
Composition & {\color[HTML]{6434FC} ✓} & {\color[HTML]{FE0000} ✗} & {\color[HTML]{6434FC} ✓} & {\color[HTML]{FE0000} ✗} & {\color[HTML]{6434FC} ✓} \\
Adaptation           & {\color[HTML]{FE0000} ✗} & {\color[HTML]{6434FC} ✓} & {\color[HTML]{FE0000} ✗} & {\color[HTML]{6434FC} ✓} & {\color[HTML]{6434FC} ✓} \\
Dispersion           & {\color[HTML]{009901} ✓} & {\color[HTML]{FE0000} ✗} & {\color[HTML]{009901} ✓} & {\color[HTML]{FE0000} ✗} & {\color[HTML]{6434FC} ✓}
\end{tabular}

